Learning Audio-guided Video Representation with Gated Attention for Video-Text Retrieval

Video-text retrieval, the task of retrieving videos based on a textual query or vice versa, is of paramount importance for video understanding and multimodal information retrieval. Recent methods in this area rely primarily on visual and textual features and often ignore audio, although it helps enhance overall comprehension of video content. Moreover, traditional models that incorporate audio blindly utilize the audio input regardless of whether it is useful or not, resulting in suboptimal video representation. To address these limitations, we propose a novel video-text retrieval framework, Audio-guided VIdeo representation learning with GATEd attention (AVIGATE), that effectively leverages audio cues through a gated attention mechanism that selectively filters out uninformative audio signals. In addition, we propose an adaptive margin-based contrastive loss to deal with the inherently unclear positive-negative relationship between video and text, which facilitates learning better video-text alignment. Our extensive experiments demonstrate that AVIGATE achieves state-of-the-art performance on all the public benchmarks.

==> Sections/_1_introduction_backup_0304.tex <==
\section{Introduction}
\label{sec:intro}
% -----------%
% - Motivation & Challenges
%     - 기존의 VTR methods들은 괄목할만한 improvement를 보여왔지만, video 내에 들어 있는 정보인 audio 정보를 무시함. 하지만 video 내엔 ‘invisible’ 하지만 ‘audible’ 한 정보들이 있고 이는 text-video retrieval을 하는데 중요한 clue가 될 수 있음. 이를 모두 활용해서 video를 표현한다면 더 나은 video representation을 얻을 수 있음.
%         - 모든 audio가 항상 video representation을 강화 하는 것은 아님. such as noisy background sound.
%     - Audio 정보를 활용하는 사전 연구도 있지만, 이는 audible 정보와 visible 정보를 각각 text와의 cross-attention networks 통해 explicit 하게 text와의 relations을 각각 추론하는데, 이는 large computational burden을 요구함. 덧붙여 global text-video alignment 만을 수행하기 때문에 fine-detail을 잡기 어려움.
%     - 대부분의 recent work은 loss function에 대해 무시하고 있으나, 이는 더 큰 성능 향상을 기대할 수 있는 여지가 있음.
% - Our method
%     - Audio-guided video representation을 얻기 위한 새로운 framework 제안.
%         - 이 framework은 audio-visual modalities들을 효과적으로 bridging and fusion하여 video representation을 얻음.
%         - 먼저, audio와 visual frame을 위한 pre-trained audio encoder와 vision encoder가 각각 있고, audio encoder는 dense-sampled audio를 encoding 하고, vision encoder는 sparse-sampled frame을 encoding 한다.
%         - 이러한 dense audio embedding을 direct하게 sparse frame embedding과 fusion하게 되면 풍부하고 informative 한 dense information이 훼손될 수 있음. 이를 방지하고자 fixed number의 embedding을 resampling 함.
%         - Cross-attention mechanism을 통해 resampled audio embedding과 frame embedding을 fusion 하게 되는데, 모든 audio가 informative 하진 않을 수도 있으니 (e.g., noise) 이에 대해 fusion 결과를 얼만큼 반영할 지에 대한 score를 바탕으로 gating 해준다.
%     - Global-Local video-text alignment
%         - 상보적인 역할을 할 수 있는 fused 된 video embedding을 바탕으로 fine-detail을 capture할 수 있는 local video-text alignment과, global context를 capture할 수 있는 global video-text alignment을 통해 matching capability를 강화 함.
%     - Adaptive Margin-based Contrastive loss
%         - 대부분의 previous work은 conventional한 contrastive loss만을 사용 해왔다. 이는 비슷한 context를 담고 있는 negative pair를 embedding space 상에서 강제로 멀게하여 poor generalization capability를 갖게 할 수도 있다.
%         - 이를 방지하고자 adaptive margin-based contrastive loss를 제안하며, 이 때 margin은 negative pair간의 relevance를 고려하여 계산된다.
% - Contribution
%     - An effective audio-video fusion module for Text-Video retrieval
%     - A new loss function for boosting the performance
%     - We achieve the state of the art performance
% -----------%

Video-text retrieval, the task of finding videos relevant to text query or vice versa, has gained significant interest due to its diverse applications in video understanding and multi-modal information retrieval. 
% It leverages a joint latent space to facilitate effective cross-modal alignment by aligning textual descriptions with corresponding video content.
\begin{figure}[t!]
    % \vspace{-1mm}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/teaser_v8.pdf}
    %\caption{Comparative illustration of different scenarios using visual-only, audio-video fusion, and our proposed gated fusion approach. (a) In cases where the audio signal provides valuable information (\eg, the sound of people singing), the audio-video fusion and our gated fusion achieve high similarity scores. (b) When the audio signal is misleading (\eg, background noise), traditional fusion methods degrade performance. In contrast, our gated fusion mechanism successfully filters irrelevant audio cues, maintaining a high similarity score like the visual-only case.}\
    \vspace{-2mm}
    \caption{Comparative illustration of different scenarios using visual-only, audio-video fusion, and our proposed gated fusion approach. (a) In cases where the audio signal provides valuable information, the audio-video fusion and our gated fusion achieve high similarity scores. (b) When the audio signal is misleading, traditional fusion methods degrade performance. In contrast, our gated fusion mechanism successfully filters irrelevant audio cues, maintaining a high similarity score like the visual-only case.}
    \label{fig: teaser}
    \vspace{-3mm}
\end{figure}
Most existing methods in this field have primarily focused on leveraging visual information from videos and textual information from accompanying metadata or captions~\cite{clip4clip,clip2video,camoe,xclip,xpool,ts2,uatvr,prost,ucofia}. 
While these methods have greatly advanced video-text retrieval, they still have a significant limitation: they neglect audio information of video that conveys `\textit{invisible but audible}' cues providing essential context such as speaker identity, background noises, or emotional nuances, which are crucial for a comprehensive understanding of video.
% Existing approaches fail to fully exploit the multi-modal nature of videos, leading to suboptimal retrieval performance.
Leveraging the audio information in video representation learning has potential to substantially improve retrieval performance by offering a richer multi-modal representation of video, as shown in Figure~\ref{fig: teaser}(a).

Nevertheless, only a few recent studies~\cite{eclipse,tefal} have explored the use of audio information in video-text retrieval tasks. ECLIPSE~\cite{eclipse} employs a cross-modal attention mechanism to fuse audio and visual modalities, creating a unified representation. TEFAL~\cite{tefal}, on the other hand, proposes text-conditioned feature alignment based on the cross-attention mechanism for audio and textual modalities as well as for visual and textual modalities.
These methods commonly assume that audio contributes positively to enhancing the video representation, but this is not always the case.
% However, not all videos contain audio that contributes positively to enhancing their representation. 
% In particular, background noise can be detrimental and may degrade the representation rather than improve it. 
When irrelevant audio is processed jointly with visual information~(\eg, irrelevant background music and noise), it could impair the video representation and negatively affect cross-modal alignment, as shown in Figure~\ref{fig: teaser}(b). 
% This degradation may ultimately hinder successful video-text retrieval by negatively affecting the overall cross-modal alignment.
ECLIPSE and TEFAL do not address this issue and blindly exploit the audio modality.
% TEFAL~\cite{tefal} has mitigated this issue by extracting text-conditioned representation of visual frame and audio separately.
Moreover, TEFAL introduces substantial computational demands on retrieval systems since both the video (also audio) and text description must be processed together to generate the representation of both video frame and audio, necessitating reprocessing of the entire database each time a new query is received.


% To address these issues, we introduce a new framework that dynamically determines whether the audio inputs are important, where the text encoder is separated from the audio encoder and visual encoder; its overall architecture is illustrated in Figure~\ref{fig: arch}.
To address these issues, we introduce a novel framework, \textbf{A}udio-guided \textbf{VI}deo representation learning with \textbf{GATE}d attention~(\textbf{AVIGATE}), that dynamically determines whether audio input is useful and enables efficient retrieval by processing video (including audio) and text description independently; its overall architecture is illustrated in Figure~\ref{fig: arch}.
% The proposed framework 
AVIGATE is built on three encoders for each modality: Audio Spectrogram Transformer (AST)~\cite{ast} for the audio input and two CLIP encoders~\cite{clip}, one for visual input and the other for textual input.
The model begins by encoding audio using AST to produce dense audio embeddings. 
These embeddings are then processed by an audio resampler to preserve rich audio information while reducing redundancy by resampling to a fixed number of embeddings. 
Video is represented by frame embeddings given by the CLIP image encoder, while the text is encoded by the CLIP text encoder. 

Audio and frame embeddings are then fused by a gated fusion transformer. \iffalse, which consists of a gated fusion block and a gating function. 
The gated fusion block produces the fused audio-visual embeddings by a cross-attention mechanism to capture complementary information between the two modalities. 
The gating function predicts gating scores given audio and frame embeddings and thus selectively filters out the fused embeddings to mitigate the effect of noisy signals while maintaining the frame embeddings.
\fi
This module integrates audio and frame embeddings by employing an adaptive gating function that regulates the influence of each modality. 
To be specific, the gate function dynamically determines the contribution of audio embeddings, allowing the transformer to leverage complementary audio information when relevant while maintaining the frame embeddings by minimizing the effect of potentially noisy audio.
\iffalse
The output of the gated fusion transformer, \ie, the final video representation, is aligned with the text embedding with a global-local alignment scheme~\cite{xclip,prost,ucofia,uatvr} that combines both global alignment between the entire video and the text, and local alignment between each video frame and the text.
This alignment scheme enables capturing both the overall semantic context and fine details, leading to more accurate retrieval.


In addition, we propose an adaptive margin-based contrastive loss that extends the traditional contrastive loss by incorporating an adaptive margin term for each negative pair. 
The margin is determined based on the intra-modal dissimilarity within both the textual and visual modalities, allowing for implicit exploration of the semantic relationship of the negative pair. 
Meanwhile, conventional contrastive loss, \ie, InfoNCE~\cite{Sohn_nips2016,oord2018representation}, treats all negative pairs equally, ignoring the semantic relationships between them. 
It may lead to suboptimal representations, especially when negative pairs vary significantly in their semantic similarities. 
We address this limitation thanks to the adaptive margins between the negative pairs according to their semantic dissimilarities.
As a consequence, the proposed loss function leads to a better video-text alignment.
\fi
The output of the gated fusion transformer, \ie, the final video representation, is then aligned with the text embedding.

To improve the discriminative capability of video-text alignment, we propose an adaptive margin-based contrastive learning approach that extends the traditional contrastive loss~\cite{Sohn_nips2016,oord2018representation} by incorporating an additional margin for each negative pair.
The margin is determined based on the intra-modal dissimilarity within both the textual and visual modalities, allowing for implicit exploration of inherent relationships among semantically similar pairs.
The input similarity score between the video representation and the text embedding used in the proposed loss is computed through a multi-grained alignment scheme~\cite{xclip,prost,ucofia,uatvr} that enables capturing both the overall semantic context and fine details.
Consequently, the proposed loss with the multi-grained alignment scheme encourages learning a more discriminative and generalizable cross-modal embedding space, leading to a better video-text alignment. 

Our method was evaluated and compared with prior work on two public benchmarks~\cite{msrvtt,vatex} where it outperformed all existing methods while enabling an efficient retrieval.
The main contribution of this paper is three-fold:
\begin{itemize}[leftmargin=*, topsep=1mm]
\item We propose AVIGATE, an effective audio-video fusion framework that fuses audio and visual information while dynamically determining whether the audio is valuable. 
\iffalse with a gated attention mechanism that determines whether the audio signal is valuable. \fi  
\item We propose a new adaptive margin-based contrastive loss, considering inherent relationships between semantically similar pairs so that the cross-modal embedding space becomes more discriminative and better generalizes. 
\item  Our method achieves the best performance on two public benchmarks for video-text retrieval and ensures a high retrieval efficiency during testing.
\end{itemize}


==> Sections/_1_introduction_backup_1110.tex <==
\section{Introduction}
\label{sec:intro}
% -----------%
% - Motivation & Challenges
%     - 기존의 VTR methods들은 괄목할만한 improvement를 보여왔지만, video 내에 들어 있는 정보인 audio 정보를 무시함. 하지만 video 내엔 ‘invisible’ 하지만 ‘audible’ 한 정보들이 있고 이는 text-video retrieval을 하는데 중요한 clue가 될 수 있음. 이를 모두 활용해서 video를 표현한다면 더 나은 video representation을 얻을 수 있음.
%         - 모든 audio가 항상 video representation을 강화 하는 것은 아님. such as noisy background sound.
%     - Audio 정보를 활용하는 사전 연구도 있지만, 이는 audible 정보와 visible 정보를 각각 text와의 cross-attention networks 통해 explicit 하게 text와의 relations을 각각 추론하는데, 이는 large computational burden을 요구함. 덧붙여 global text-video alignment 만을 수행하기 때문에 fine-detail을 잡기 어려움.
%     - 대부분의 recent work은 loss function에 대해 무시하고 있으나, 이는 더 큰 성능 향상을 기대할 수 있는 여지가 있음.
% - Our method
%     - Audio-guided video representation을 얻기 위한 새로운 framework 제안.
%         - 이 framework은 audio-visual modalities들을 효과적으로 bridging and fusion하여 video representation을 얻음.
%         - 먼저, audio와 visual frame을 위한 pre-trained audio encoder와 vision encoder가 각각 있고, audio encoder는 dense-sampled audio를 encoding 하고, vision encoder는 sparse-sampled frame을 encoding 한다.
%         - 이러한 dense audio embedding을 direct하게 sparse frame embedding과 fusion하게 되면 풍부하고 informative 한 dense information이 훼손될 수 있음. 이를 방지하고자 fixed number의 embedding을 resampling 함.
%         - Cross-attention mechanism을 통해 resampled audio embedding과 frame embedding을 fusion 하게 되는데, 모든 audio가 informative 하진 않을 수도 있으니 (e.g., noise) 이에 대해 fusion 결과를 얼만큼 반영할 지에 대한 score를 바탕으로 gating 해준다.
%     - Global-Local video-text alignment
%         - 상보적인 역할을 할 수 있는 fused 된 video embedding을 바탕으로 fine-detail을 capture할 수 있는 local video-text alignment과, global context를 capture할 수 있는 global video-text alignment을 통해 matching capability를 강화 함.
%     - Adaptive Margin-based Contrastive loss
%         - 대부분의 previous work은 conventional한 contrastive loss만을 사용 해왔다. 이는 비슷한 context를 담고 있는 negative pair를 embedding space 상에서 강제로 멀게하여 poor generalization capability를 갖게 할 수도 있다.
%         - 이를 방지하고자 adaptive margin-based contrastive loss를 제안하며, 이 때 margin은 negative pair간의 relevance를 고려하여 계산된다.
% - Contribution
%     - An effective audio-video fusion module for Text-Video retrieval
%     - A new loss function for boosting the performance
%     - We achieve the state of the art performance
% -----------%

Video-text retrieval, which involves retrieving videos from textual queries or vice versa, has gained significant interest due to its applications in video understanding and multi-modal information retrieval. 
The rapid growth of multimedia content necessitates effective alignment between visual and textual modalities to achieve accurate retrieval results. 
Video-text retrieval leverages a joint latent space to facilitate cross-modal alignment, linking text descriptions with corresponding video content. 

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/teaser_v2.pdf}
    %\caption{Comparative illustration of different scenarios using visual-only, audio-video fusion, and our proposed gated fusion approach. (a) In cases where the audio signal provides valuable information (\eg, the sound of people singing), the audio-video fusion and our gated fusion achieve high similarity scores. (b) When the audio signal is misleading (\eg, background noise), traditional fusion methods degrade performance. In contrast, our gated fusion mechanism successfully filters irrelevant audio cues, maintaining a high similarity score like the visual-only case.}\
    \caption{Comparative illustration of different scenarios using visual-only, audio-video fusion, and our proposed gated fusion approach. (a) In cases where the audio signal provides valuable information, the audio-video fusion and our gated fusion achieve high similarity scores. (b) When the audio signal is misleading, traditional fusion methods degrade performance. In contrast, our gated fusion mechanism successfully filters irrelevant audio cues, maintaining a high similarity score like the visual-only case.}
    \label{fig: teaser}
    \vspace{-5mm}
\end{figure}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/arch_v4.pdf}
    \caption{Overall architecture (place-hold)}
    \label{fig: arch}
    \vspace{-3mm}
\end{figure*}

In recent years, many methods~\cite{clip4clip,clip2video,camoe,xclip,xpool,ts2,uatvr,prost,ucofia} in this field have primarily focused on leveraging visual information from videos and textual information from accompanying metadata or captions to perform retrieval tasks. 
Despite these strides, a considerable limitation persists in many existing methods; they often neglect the valuable audio information in videos, which conveys `\textit{invisible but audible}' cues that often serve as essential context, such as speaker identity, background sounds, or emotional nuances, which are crucial for a comprehensive understanding of video content.
% Existing approaches fail to fully exploit the multi-modal nature of videos, leading to suboptimal retrieval performance.
Leveraging the audio information in video representation learning has the potential to substantially improve retrieval performance by offering a richer multi-modal understanding of video data, as shown in Figure~\ref{fig: teaser}(a).
Recent studies~\cite{eclipse,tefal} have explored the incorporation of audio information in video-text retrieval tasks. ECLIPSE~\cite{eclipse} employs a cross-attention mechanism to fuse audio and visual modalities, creating a unified representation. TEFAL~\cite{tefal}, on the other hand, proposes a method for text-conditioned feature alignment by utilizing the cross-attention mechanism for audio and textual modalities as well as for visual and textual modalities.


However, not all videos contain audio that contributes positively to enhancing their representation. 
% In particular, background noise can be detrimental and may degrade the representation rather than improve it. 
When such disruptive audio is processed jointly with visual information, it may impair the representation of the video, even in cases where visual information alone is sufficient, as shown in Figure~\ref{fig: teaser}(b). 
This degradation may ultimately hinder successful video-text retrieval by negatively affecting the overall cross-modal alignment.
ECLIPSE~\cite{eclipse} and TEFAL~\cite{tefal}, for instance, do not adequately address this issue and merely exploit the audio modality.
% TEFAL~\cite{tefal} has mitigated this issue by extracting text-conditioned representation of visual frame and audio separately.
Moreover, TEFAL is not suitable for the real-world retrieval system since it inevitably introduces substantial computational demands on retrieval systems, as both the video (also audio) and text description must be processed together to generate the representation of both video frame and audio, necessitating reprocessing of the entire database each time a new query is received.


% To address these issues, we introduce a new framework that dynamically determines whether the audio inputs are important, where the text encoder is separated from the audio encoder and visual encoder; its overall architecture is illustrated in Figure~\ref{fig: arch}.
To address these issues, we introduce a novel framework, \textbf{A}udio-guided \textbf{V}ideo repres\textbf{EN}tation learning with \textbf{G}ated att\textbf{E}ntion for video-text \textbf{R}etrieval (\textbf{AVENGER}), that dynamically determines whether the audio inputs are important while enabling an efficient retrieval system by processing video (including audio) and text descriptions independently; its overall architecture is illustrated in Figure~\ref{fig: arch}.
% The proposed framework 
AVENGER is built on three encoders for each modality: the AST~\cite{ast} model for the audio input and two CLIP encoders~\cite{clip}, one for visual input and the other for textual input.
The model begins by encoding the audio modality using the AST model, which generates dense audio embeddings. 
These embeddings are then processed through the audio resampler to preserve rich audio information while reducing redundancy by resampling to a fixed number of embeddings. 
The visual modality is represented by frame embeddings obtained from the CLIP image encoder, while the text is encoded by the CLIP text encoder. 
These audio and frame embeddings are then fused within a gated fusion module, which consists of a fusion block and a gating block. The fusion block produces the fused audio-visual embeddings by adopting a cross-attention mechanism to capture complementary information between modalities. 
The gating block predicts gating scores given audio and frame embeddings and thus selectively filters out the audio-visual embeddings, thus mitigating the effect of noisy signals.
The output of the gated fusion module, video representation, is aligned with text embedding with global-local alignment scheme that is a widely explored approach in~\cite{xclip,prost,ucofia,uatvr}. 
It combines both global alignment between the entire video and the text, and local alignment between the video frame and the text.
This alignment scheme enables the capture of both the overall semantic context and fine details, leading to a more accurate retrieval.
% ultimately improves retrieval accuracy.

Meanwhile, most existing methods rely on conventional contrastive loss, \ie, InfoNCE~\cite{Sohn_nips2016,oord2018representation}, which may lead to poor generalization by treating all the negative pairs equally since it neglects the potential semantic relations in the negative pairs. 
To tackle this issue, we propose an adaptive margin-based contrastive loss that extends the traditional contrastive loss by incorporating an adaptive margin term for each negative pair. 
The margin is determined based on the intra-modal dissimilarity within both the textual and visual modalities, allowing for implicit exploration of the semantic relationship of the negative pair. As a consequence, the proposed loss function facilitates a better video-text alignment.

Our method was evaluated and compared with prior work on public benchmarks~\cite{msrvtt,vatex}.
Our method outperforms all existing methods thanks to the audio-guided video representation based on gated attention.
The main contribution of this paper is three-fold:
\begin{itemize}[leftmargin=*, topsep=1mm]
\item We propose AVENGER, an effective audio-video fusion framework with a gated attention mechanism that determines whether the audio signal is valuable.  
\item We propose a new adaptive margin-based contrastive loss that reflects the semantic relationships of video-text pairs. 
\item  Our method achieves the best on all the public benchmarks for video-text retrieval.
\end{itemize}


==> Sections/_1_introduction_backup_1113.tex <==
\section{Introduction}
\label{sec:intro}
% -----------%
% - Motivation & Challenges
%     - 기존의 VTR methods들은 괄목할만한 improvement를 보여왔지만, video 내에 들어 있는 정보인 audio 정보를 무시함. 하지만 video 내엔 ‘invisible’ 하지만 ‘audible’ 한 정보들이 있고 이는 text-video retrieval을 하는데 중요한 clue가 될 수 있음. 이를 모두 활용해서 video를 표현한다면 더 나은 video representation을 얻을 수 있음.
%         - 모든 audio가 항상 video representation을 강화 하는 것은 아님. such as noisy background sound.
%     - Audio 정보를 활용하는 사전 연구도 있지만, 이는 audible 정보와 visible 정보를 각각 text와의 cross-attention networks 통해 explicit 하게 text와의 relations을 각각 추론하는데, 이는 large computational burden을 요구함. 덧붙여 global text-video alignment 만을 수행하기 때문에 fine-detail을 잡기 어려움.
%     - 대부분의 recent work은 loss function에 대해 무시하고 있으나, 이는 더 큰 성능 향상을 기대할 수 있는 여지가 있음.
% - Our method
%     - Audio-guided video representation을 얻기 위한 새로운 framework 제안.
%         - 이 framework은 audio-visual modalities들을 효과적으로 bridging and fusion하여 video representation을 얻음.
%         - 먼저, audio와 visual frame을 위한 pre-trained audio encoder와 vision encoder가 각각 있고, audio encoder는 dense-sampled audio를 encoding 하고, vision encoder는 sparse-sampled frame을 encoding 한다.
%         - 이러한 dense audio embedding을 direct하게 sparse frame embedding과 fusion하게 되면 풍부하고 informative 한 dense information이 훼손될 수 있음. 이를 방지하고자 fixed number의 embedding을 resampling 함.
%         - Cross-attention mechanism을 통해 resampled audio embedding과 frame embedding을 fusion 하게 되는데, 모든 audio가 informative 하진 않을 수도 있으니 (e.g., noise) 이에 대해 fusion 결과를 얼만큼 반영할 지에 대한 score를 바탕으로 gating 해준다.
%     - Global-Local video-text alignment
%         - 상보적인 역할을 할 수 있는 fused 된 video embedding을 바탕으로 fine-detail을 capture할 수 있는 local video-text alignment과, global context를 capture할 수 있는 global video-text alignment을 통해 matching capability를 강화 함.
%     - Adaptive Margin-based Contrastive loss
%         - 대부분의 previous work은 conventional한 contrastive loss만을 사용 해왔다. 이는 비슷한 context를 담고 있는 negative pair를 embedding space 상에서 강제로 멀게하여 poor generalization capability를 갖게 할 수도 있다.
%         - 이를 방지하고자 adaptive margin-based contrastive loss를 제안하며, 이 때 margin은 negative pair간의 relevance를 고려하여 계산된다.
% - Contribution
%     - An effective audio-video fusion module for Text-Video retrieval
%     - A new loss function for boosting the performance
%     - We achieve the state of the art performance
% -----------%

Video-text retrieval, the task of finding videos relevant to text query or vice versa, has gained significant interest due to its diverse applications in video understanding and multi-modal information retrieval. 
It leverages a joint latent space to facilitate effective cross-modal alignment by aligning textual descriptions with corresponding video content.
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/teaser_v4.pdf}
    %\caption{Comparative illustration of different scenarios using visual-only, audio-video fusion, and our proposed gated fusion approach. (a) In cases where the audio signal provides valuable information (\eg, the sound of people singing), the audio-video fusion and our gated fusion achieve high similarity scores. (b) When the audio signal is misleading (\eg, background noise), traditional fusion methods degrade performance. In contrast, our gated fusion mechanism successfully filters irrelevant audio cues, maintaining a high similarity score like the visual-only case.}\
    \caption{Comparative illustration of different scenarios using visual-only, audio-video fusion, and our proposed gated fusion approach. (a) In cases where the audio signal provides valuable information, the audio-video fusion and our gated fusion achieve high similarity scores. (b) When the audio signal is misleading, traditional fusion methods degrade performance. In contrast, our gated fusion mechanism successfully filters irrelevant audio cues, maintaining a high similarity score like the visual-only case.}
    \label{fig: teaser}
    \vspace{-5mm}
\end{figure}

Most of the existing methods in this field have primarily focused on leveraging visual information from videos and textual information from accompanying metadata or captions~\cite{clip4clip,clip2video,camoe,xclip,xpool,ts2,uatvr,prost,ucofia}. 
While these methods have greatly advanced video-text retrieval, they still have a significant limitation: they neglect audio information of video that conveys `\textit{invisible but audible}' cues providing essential context such as speaker identity, background sounds, or emotional nuances, which are crucial for a comprehensive understanding of video content.
% Existing approaches fail to fully exploit the multi-modal nature of videos, leading to suboptimal retrieval performance.
Leveraging the audio information in video representation learning has the potential to substantially improve retrieval performance by offering a richer multi-modal understanding of video data, as shown in Figure~\ref{fig: teaser}(a).

Only a few recent studies~\cite{eclipse,tefal} have explored the use of audio information in video-text retrieval tasks. ECLIPSE~\cite{eclipse} employs a cross-modal attention mechanism to fuse audio and visual modalities, creating a unified representation. TEFAL~\cite{tefal}, on the other hand, proposes a method for text-conditioned feature alignment by utilizing the cross-attention mechanism for audio and textual modalities as well as for visual and textual modalities.
These methods commonly assume that audio contributes positively to enhancing the video representation, but this is not always the case.
% However, not all videos contain audio that contributes positively to enhancing their representation. 
% In particular, background noise can be detrimental and may degrade the representation rather than improve it. 
When irrelevant audio is processed jointly with visual information~(\eg, irrelevant background music and noise), it could impair the video representation and negatively affect cross-modal alignment, as shown in Figure~\ref{fig: teaser}(b). 
% This degradation may ultimately hinder successful video-text retrieval by negatively affecting the overall cross-modal alignment.
ECLIPSE and TEFAL, for instance, do not address this issue and blindly exploit the audio modality.
% TEFAL~\cite{tefal} has mitigated this issue by extracting text-conditioned representation of visual frame and audio separately.
Moreover, TEFAL introduces substantial computational demands on retrieval systems since both the video (also audio) and text description must be processed together to generate the representation of both video frame and audio, necessitating reprocessing of the entire database each time a new query is received.


% To address these issues, we introduce a new framework that dynamically determines whether the audio inputs are important, where the text encoder is separated from the audio encoder and visual encoder; its overall architecture is illustrated in Figure~\ref{fig: arch}.
To address these issues, we introduce a novel framework, \textbf{A}udio-guided \textbf{VI}deo representation learning with \textbf{GATE}d attention~(\textbf{AVIGATE}), that dynamically determines whether audio input is useful and enables an efficient retrieval system by processing video (including audio) and text description independently; its overall architecture is illustrated in Figure~\ref{fig: arch}.
% The proposed framework 
AVIGATE is built on three encoders for each modality: Audio Spectrogram Transformer (AST)~\cite{ast} for the audio input and two CLIP encoders~\cite{clip}, one for visual input and the other for textual input.
The model begins by encoding audio modality using AST, which generates dense audio embeddings. 
These embeddings are then processed by an audio resampler to preserve rich audio information while reducing redundancy by resampling to a fixed number of embeddings. 
Video is represented by frame embeddings obtained from the CLIP image encoder, while the text is encoded by the CLIP text encoder. 

Audio and frame embeddings are then fused by a gated fusion transformer. \iffalse, which consists of a gated fusion block and a gating function. 
The gated fusion block produces the fused audio-visual embeddings by a cross-attention mechanism to capture complementary information between the two modalities. 
The gating function predicts gating scores given audio and frame embeddings and thus selectively filters out the fused embeddings to mitigate the effect of noisy signals while maintaining the frame embeddings.
\fi
Specifically, the gated fusion transformer integrates audio and frame embeddings by employing an adaptive gating function that assigns scores to regulate the influence of each modality. 
These gating scores dynamically determine the contribution of audio embeddings, allowing the transformer to leverage complementary audio information when relevant while maintaining the frame embeddings by minimizing the effect of potentially noisy audio.
\iffalse
The output of the gated fusion transformer, \ie, the final video representation, is aligned with the text embedding with a global-local alignment scheme~\cite{xclip,prost,ucofia,uatvr} that combines both global alignment between the entire video and the text, and local alignment between each video frame and the text.
This alignment scheme enables capturing both the overall semantic context and fine details, leading to more accurate retrieval.


In addition, we propose an adaptive margin-based contrastive loss that extends the traditional contrastive loss by incorporating an adaptive margin term for each negative pair. 
The margin is determined based on the intra-modal dissimilarity within both the textual and visual modalities, allowing for implicit exploration of the semantic relationship of the negative pair. 
Meanwhile, conventional contrastive loss, \ie, InfoNCE~\cite{Sohn_nips2016,oord2018representation}, treats all negative pairs equally, ignoring the semantic relationships between them. 
It may lead to suboptimal representations, especially when negative pairs vary significantly in their semantic similarities. 
We address this limitation thanks to the adaptive margins between the negative pairs according to their semantic dissimilarities.
As a consequence, the proposed loss function leads to a better video-text alignment.
\fi
The output of the gated fusion transformer, \ie, the final video representation, is then aligned with the text embedding.

To improve the discriminative capability of video-text alignment, we propose an adaptive margin-based contrastive learning approach that extends the traditional contrastive loss~\cite{Sohn_nips2016,oord2018representation} by incorporating an additional margin for each negative pair.
The margin is determined based on the intra-modal dissimilarity within both the textual and visual modalities, allowing for implicit exploration of inherent relationships among semantically similar pairs.
Furthermore, the input similarity score between the video representation and the text embedding used in the proposed loss is computed through a multi-grained alignment scheme~\cite{xclip,prost,ucofia,uatvr} that enables capturing both the overall semantic context and fine details.
Consequently, the proposed loss with the multi-grained alignment scheme encourages learning a more discriminative and generalizable cross-modal embedding space, leading to a better video-text alignment. 

Our method was evaluated and compared with prior work on two public benchmarks~\cite{msrvtt,vatex}.
Our method outperformed all existing methods thanks to the audio-guided video representation based on gated attention.
The main contribution of this paper is three-fold:
\begin{itemize}[leftmargin=*, topsep=1mm]
\item We propose AVIGATE, an effective audio-video fusion framework that fuses audio and visual information while dynamically determining whether the audio signal is valuable. 
\iffalse with a gated attention mechanism that determines whether the audio signal is valuable. \fi  
\item We propose a new adaptive margin-based contrastive loss, considering inherent relationships among semantically similar pairs so that the cross-modal embedding space becomes more discriminative and better generalizes. 
\item  Our method achieves the best on two public benchmarks for video-text retrieval.
\end{itemize}


==> Sections/_3_method_backup1112.tex <==

\section{Proposed Method}
\label{sec:method}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/arch_v6.pdf}
    \caption{The overall architecture of AVIGATE. (\bs{Need caption.})}
    \label{fig: arch}
    \vspace{-3mm}
\end{figure*}
% In this section, we describe our novel framework, AVIGATE.
% Firstly, we present embedding extraction for each modality with its encoder~(\cref{sec:extraction}). Then, the gated fusion transformer~(\cref{sec:gate}) and the global-local alignment scheme~(\cref{sec:align}) are introduced. 
% The overall architecture of our framework is depicted in Figure~\ref{fig: arch}.
% Lastly, we describe the adaptive margin-based contrastive loss~(\cref{sec:margin_loss}).
In this section, we describe our novel framework, AVIGATE.
Firstly, we present embedding extraction for each modality with its encoder~(\cref{sec:extraction}). 
Then, the gated fusion transformer is introduced~(\cref{sec:gate}). 
Lastly, we describe the adaptive margin-based contrastive learning strategy~(\cref{sec:margin_loss}).
The overall architecture of our framework is depicted in Figure~\ref{fig: arch}.

\subsection{Embedding Extraction}
\label{sec:extraction}

The proposed framework, AVIGATE, utilizes three pre-trained encoders to process each modality: Two CLIP encoders~\cite{clip} for the video frames and the text descriptions, respectively, and Audio Spectrogram Transformer (AST)~\cite{ast} for the audio signals.

\noindent\textbf{Frame Embeddings:} Following~\cite{clip4clip}, we utilize the pre-trained CLIP image encoder~\cite{clip} to extract the frame embeddings of each video.
Given an input video $V$, the video is uniformly sampled to obtain $N$ frames, denoted as $V=[F^1, F^2, \dots, F^N]$. 
Each frame is divided into non-overlapping patches, which are then transformed using a linear projection. 
A [\texttt{CLS}] token is prepended to this sequence of patches, and the combined sequence is fed through the CLIP image encoder. 
The output corresponding to the [\texttt{CLS}] token is taken as the frame embedding.
Finally, these frame embeddings are concatenated to form a sequence of frame embeddings, $\mathbf{f}=[\mathbf{f}^1, \mathbf{f}^2, \dots, \mathbf{f}^N]\in\mathbb{R}^{N\times D}$, where $D$ denotes the dimension of the frame embedding. 

\noindent\textbf{Text Embeddings:} The text embedding extraction process is carried out using the CLIP text encoder~\cite{clip}, akin to the procedure for extracting frame embeddings. 
Given a text input $T$, all words in the text are tokenized, and special tokens [\texttt{SOS}] and [\texttt{EOS}] are enclosed to designate the start and the end of the sentence, respectively. 
This complete sequence is then passed through the CLIP text encoder.
Then, the output corresponding to the [\texttt{EOS}] token is regarded as the text embedding, $\mathbf{t} \in \mathbb{R}^{D}$, capturing the overall semantics of the input text.

% \noindent\textbf{Audio Embeddings:} Following~\cite{ast, tefal}, we adopt the AST~\cite{ast} model as the audio encoder. 
% Given an audio input $A_i$ from the video $V_i$, it is converted into a Mel-spectrogram, capturing essential auditory features in both time and frequency domains. 
% The AST model treats this spectrogram as a sequence of patches with length $N_a$ and applies transformer encoder layers to extract audio embeddings. %, $\mathbf{a}_i=[\mathbf{a}^1_i, \mathbf{a}^2_i, \dots, \mathbf{a}^{N_a}_i]\in\mathbb{R}^{N_a\times D}$.
% \bs{It is worth noting that the audio signals are densely sampled compared to the frame sampling; thus, the AST model outputs a large number of embeddings per audio input (\ie, $N_a \gg N$). 
% Directly fusing this large number of audio embeddings with frame embeddings would lead to excessive computational overhead. 
% To address this, we introduce an audio resampler inspired by Perceiver~\cite{perceiver}, DETR~\cite{detr}, and Flamingo~\cite{flamingo}, which efficiently reduces the number of audio embeddings by employing a cross-attention mechanism with $M$ learnable query embeddings to generate a fixed length of $M$ audio embeddings $\mathbf{a}_i=[\mathbf{a}^1_i, \mathbf{a}^2_i, \dots, \mathbf{a}^{M}_i]\in\mathbb{R}^{M\times D}$.
% The audio resampler maintains the essential auditory information while significantly lowering the computational cost of subsequent fusion with visual modalities. 
% Additionally, we freeze the AST model during training to prevent the high computational demands associated with fine-tuning its parameters. 
% More architectural details are presented in the supplementary material.}

\noindent\textbf{Audio Embeddings:} We utilize the AST model~\cite{ast} as our audio encoder, following the approach in prior work~\cite{ast, tefal}. Given an audio input $A$ from video $V$, the signal is first converted into a Mel-spectrogram, capturing key auditory features across time and frequency. The AST model processes this spectrogram as a sequence of $N_a$ patches, using transformer layers to generate a detailed set of audio embeddings.
However, since audio signals are densely sampled compared to video frames, directly fusing all $N_a$ audio embeddings with frame embeddings would be computationally expensive. To address this, we employ an additional query-based transformer~(\ie, audio resampler)~\cite{perceiver, detr, flamingo} that uses a cross-attention mechanism with $M$ learnable query embeddings. This design reduces the number of audio embeddings to a fixed length of $M$, $\mathbf{a}=[\mathbf{a}^1, \mathbf{a}^2, \dots, \mathbf{a}^{M}] \in \mathbb{R}^{M \times D}$, maintaining essential auditory information while significantly lowering computational load for subsequent fusion with visual modalities. We freeze the AST model parameters during training, avoiding the high computational cost of fine-tuning. More architectural details are provided in the supplementary material.

\subsection{Gated Fusion Transformer}
\label{sec:gate}

% To achieve effective fusion between the audio embedding $\mathbf{a}$ and the frame embedding $\mathbf{f}$, we introduce a gated fusion transformer consisting of $L$ layers, which dynamically assesses the importance of the audio signal.  
% By employing a gating mechanism, the gated fusion transformer ensures that only informative audio content contributes to the final video representation. 
% This method mitigates the impact of detrimental audio signals and enables the video representation to contain salient multimodal features while preserving frame information under unfavorable audio signals.
% In the following, we provide an in-depth discussion of the two core components of the gated fusion transformer: the fusion block and the gating block.
% \bs{To achieve effective fusion between the audio embedding $\mathbf{a}$ and the frame embedding $\mathbf{f}$, we introduce a gated fusion transformer, which is the core of the AVIGATE framework and the key contribution of our approach. 
% The gated fusion transformer employs a sophisticated fusion mechanism to extract an enhanced video representation. 
% It consists of $L$ layers with a gated fusion block, each block with Multi-Head Attention (MHA) and Feed-Forward Network (FFN) to fuse the audio embeddings with frame embeddings and refine the fused embeddings~(\ie, fusion process), followed by Multi-Head Self-Attention (MHSA) and another FFN to refine the representation~(\ie, refining process). 
% Crucially, the gating function plays a pivotal role by producing adaptive gating scores ($g_{mha}$ and $g_{ffn}$) that regulate the contribution of audio embeddings in the fusion process. 
% When the gating score is high, it allows more information from the audio to influence the output, effectively capturing complementary audio cues; when the gating score is low, the model preserves more of the original visual content, mitigating the risk of noisy or irrelevant audio signals disrupting the video representation. 
% Consequently, the adaptive gating ensures that the fusion process is dynamic and context-sensitive, leading to a more discriminative and robust representation that improves video-text retrieval performance.
% In the following, we provide in-depth architectural details of two core components of the gated fusion transformer: the gated fusion block and the gating function.}

To effectively fuse the audio embedding $\mathbf{a}$ and frame embedding $\mathbf{f}$, the gated fusion transformer in the AVIGATE is designed to dynamically adjust the contribution of audio based on its relevance to the video. This transformer achieves adaptive fusion by using gating scores that modulate the impact of audio features on the video representation, ensuring that irrelevant audio signals have a reduced influence, thus preserving the integrity of the visual content.

The gated fusion transformer consists of $L$ layers, each containing a gated fusion block that applies gating scores to control the fusion process. Within each block, Multi-Head Attention (MHA) and a Feed-Forward Network (FFN) blend the audio and frame embeddings, with the adaptive gating function providing scores ($g_{\textrm{mha}}$ and $g_{\textrm{ffn}}$) to regulate their influence. 
These gating scores control the contribution of audio embeddings, enabling the transformer to integrate complementary audio cues when relevant while minimizing the effect of potentially noisy audio. This is followed by Multi-Head Self-Attention (MHSA) and a Feed-Forward Network (FFN) to refine the representation.

When the gating scores are high, audio cues are emphasized, enhancing the representation by capturing complementary audio details. Conversely, when low gating scores, the visual content is prioritized, maintaining robustness against irrelevant audio interference. This selective fusion leads to a more context-sensitive and discriminative video representation, which improves video-text retrieval performance. In the following, we provide in-depth architectural details of two core components of the gated fusion transformer: the gated fusion block and the gating function.

\subsubsection{Gated Fusion Block}
\label{sec:fusion}
\bs{The gated fusion block takes the audio embedding $\mathbf{a}$ and the frame embedding $\mathbf{f}$ as inputs and outputs video representation through the fusion process followed by the refining process.
Specifically, with a series of $L$ layers, the frame embedding $\mathbf{f}$ evolves into refined $\mathbf{f}^{(L)}$ by capturing cross-modal interactions between audio embedding $\mathbf{a}$, where the frame embedding $\mathbf{f}$ from the CLIP image encoder is regarded as initial input $\mathbf{f}^{(0)}$.
The refined $\mathbf{f}^{(L)}$ serves as the final video representation $\mathbf{v}=[\mathbf{v}^1, \mathbf{v}^2, \dots, \mathbf{v}^N]\in\mathbb{R}^{N\times D}$.

% The gated fusion block can be formulated by:
% \begin{equation}
%     \mathbf{v} := \mathbf{f}^{(L)},~\text{where}~ \mathbf{f}^{(l)} =\texttt{GatedFusionBlock}(\mathbf{f}^{(l-1)}, \mathbf{a}).
% \end{equation}

In the fusion process, the frame embedding $\mathbf{f}^{(l-1)}$ is fused with the audio embedding $\mathbf{a}$ by the MHA mechanism with a residual connection.
%, where the frame embedding serves as the query, while the audio embedding acts as the key and value. 
The output is modulated by a gating score $g_{\textrm{mha}}$ generated from the gating function~(\cref{sec:gating_function}) to determine the contribution of the audio embedding in the fusion.
Then, the output is fed into an FFN with a residual connection, which is also modulated by a gating score $g_{\textrm{ffn}}$, ensuring selective enhancement based on the gating mechanism.
% When these gating scores are high, it emphasizes the audio features in the fusion, while a low score limits the audio contribution, thereby preserving the visual information.
The fusion process can be formulated as follows:
\begin{equation}
\begin{aligned}
    \mathbf{z}^{(l)} &=  g_{\textrm{mha}}^{(l)} \cdot \textrm{MHA}(\textrm{LN}(\mathbf{f}^{(l-1)}), \textrm{LN}(\mathbf{a})) +\mathbf{f}^{(l-1)} , \\
    \bar{\mathbf{z}}^{(l)} &= g_{\textrm{ffn}}^{(l)} \cdot \textrm{FFN}_1(\textrm{LN}(\mathbf{z}^{(l)})) + \mathbf{z}^{(l)}  , \\
    \label{eq:fusion_process}
\end{aligned}
\end{equation}
where LN denotes the layer normalization.
MHA involves $n$-head attention operations; it is formulated by
\begin{equation}
\begin{aligned}
    \textrm{MHA}(\mathbf{X},\mathbf{Y}) &= [\textrm{Attn}^1(\mathbf{X},\mathbf{Y}), ..., \textrm{Attn}^n(\mathbf{X},\mathbf{Y})]\mathbf{W}_o,\\ 
    \textrm{Attn}^i(\mathbf{X},\mathbf{Y}) &= \text{softmax}\left( \frac{(\mathbf{X}\mathbf{W}_{q}^{i}) (\mathbf{Y}\mathbf{W}_k^{i})^\top}{\sqrt{D_h}} \right) (\mathbf{Y}\mathbf{W}_v^{i})
    \label{eq:MHA}
\end{aligned}
\end{equation}
where $[\cdot,\cdot]$ denotes concatenation, and $D_h$ is set to $D/n$. 
$\mathbf{W}_{q}^{i}, \mathbf{W}_{k}^{i}, \mathbf{W}_{v}^{i}\in\mathbb{R}^{D\times D_h}$ and $\mathbf{W}_{o}\in\mathbb{R}^{D\times D}$ are linear projection matrices.

The fused representation $\bar{\mathbf{z}}^{(l)}$ undergoes the refining process to enhance the overall video representation.
Specifically, $\bar{\mathbf{z}}^{(l)}$ is fed into the Multi-Head Self-Attention (MHSA) mechanism with a residual connection.
Then, the second FFN with a residual connection is applied to the output of MHSA to produce the refined frame embedding $\mathbf{f}^{(l)}$. 
The refining process is formulated as follows:
\begin{equation}
\begin{aligned}
    \Tilde{\mathbf{z}}^{(l)} &= \textrm{MHSA}(\textrm{LN}(\bar{\mathbf{z}}^{(l)})) + \bar{\mathbf{z}}^{(l)} , \\
    \mathbf{f}^{(l)} &= \textrm{FFN}_2(\textrm{LN}(\Tilde{\mathbf{z}}^{(l)})) + \Tilde{\mathbf{z}}^{(l)}.
    \label{eq:refining_process}
\end{aligned}
\end{equation}
}
Similar to MHA, MHSA involves $n$-head self-attention operations, where $\textbf{X}=\textbf{Y}$ in~\cref{eq:MHA}.

% The gated fusion block takes the audio embedding $\mathbf{a}$ and the frame embedding $\mathbf{f}$ as inputs. 
% Then, through a series of $L$ layers, the frame embedding $\mathbf{f}$ evolves into refined $\mathbf{f}^{(L)}$ by capturing cross-modal interactions.
% Note that the frame embedding $\mathbf{f}$ from the CLIP image encoder is regarded as initial input $\mathbf{f}^{(0)}$.
% The refined $\mathbf{f}^{(L)}$ serves as the final video representation $\mathbf{v}\in \mathbb{R}^{N \times D}$.
% The fusion block can be formulated by:
% \begin{equation}
%     \mathbf{v} := \mathbf{f}^{(L)},~\text{where}~ \mathbf{f}^{(l)} =\texttt{FusionBlock}(\mathbf{f}^{(l-1)}, \mathbf{a}).
% \end{equation}

% The fusion block in each layer $l$ consists of Multi-Head Attention (MHA), Layer normalization (LN), two different Feed-Forward Networks (FFN), Multi-Head Self-Attention (MHSA), and gating scores.
% Specifically, the $l$-th fusion block is formulated as follows:
% \begin{equation}
% \begin{aligned}
%     \mathbf{z}^{(l)} &= \mathbf{f}^{(l-1)} + \textrm{MHA}(\textrm{LN}(\mathbf{f}^{(l-1)}), \textrm{LN}(\mathbf{a})) \cdot g_{\textrm{mha}}^{(l)}, \\
%     \bar{\mathbf{z}}^{(l)} &= \mathbf{z}^{(l)} + \textrm{FFN}_1(\textrm{LN}(\mathbf{z}^{(l)})) \cdot g_{\textrm{ffn}}^{(l)}, \\
%     \Tilde{\mathbf{z}}^{(l)} &= \bar{\mathbf{z}}^{(l)} + \textrm{MHSA}(\textrm{LN}(\bar{\mathbf{z}}^{(l)})), \\
%     \mathbf{f}^{(l)} &= \Tilde{\mathbf{z}}^{(l)} + \textrm{FFN}_2(\textrm{LN}(\Tilde{\mathbf{z}}^{(l)})).
%     \label{eq:fusion}
% \end{aligned}
% \end{equation}
% MHA involves $n$-head attention operations; it is formulated by
% \begin{equation}
% \begin{aligned}
%     \textrm{MHA}(\mathbf{X},\mathbf{Y}) &= [\textrm{Attn}^1(\mathbf{X},\mathbf{Y}), ..., \textrm{Attn}^n(\mathbf{X},\mathbf{Y})]\mathbf{W}_o,\\ 
%     \textrm{Attn}^i(\mathbf{X},\mathbf{Y}) &= \text{softmax}\left( \frac{(\mathbf{X}\mathbf{W}_{q}^{i}) (\mathbf{Y}\mathbf{W}_k^{i})^\top}{\sqrt{D_h}} \right) (\mathbf{Y}\mathbf{W}_v^{i})
%     \label{eq:MHA}
% \end{aligned}
% \end{equation}
% where $[\cdot,\cdot]$ denotes concatenation, and $D_h$ is set to $D/n$. 
% $\mathbf{W}_{q}^{i}, \mathbf{W}_{k}^{i}, \mathbf{W}_{v}^{i}\in\mathbb{R}^{D\times D_h}$ and $\mathbf{W}_{o}\in\mathbb{R}^{D\times D}$ are linear projection matrices.
% Similar to MHA, MHSA involves $n$-head self-attention operations, where $\textbf{X}=\textbf{Y}$ in Eq~\ref{eq:MHA}.
% Both FFN$_1$ and FFN$_2$ consist of two linear layers with a non-linear function in between:
% \begin{equation}
%     \textrm{FFN}(\mathbf{X}) = \sigma(\mathbf{X}\mathbf{W}_1+\mathbf{b}_1)\mathbf{W}_2 + \mathbf{b}_2,
%     \label{eq:FFN}
% \end{equation}
% where $\mathbf{W}_1\in\mathbb{R}^{D\times4D}$ and $\mathbf{W}_2\in\mathbb{R}^{4D\times D}$ are linear projection weights, and $b_1 \in \mathbb{R}^{4D}$ and $b_2 \in \mathbb{R}^D$ are biases.
% $\sigma(\cdot)$ denotes the non-linear function (\eg, GELU).
% Meanwhile, $g_{\text{mha}}^{(l)}$ and $g_{\text{ffn}}^{(l)}$ are the gating scores derived from the gating block (Sec.~\ref{sec:gating_block}), which modulate the outputs of MHA and FFN$_1$ layers, thereby ensuring that only relevant auditory information is incorporated into the video representation.




\subsubsection{Gating Function}
\label{sec:gating_function}
\bs{
The gating function, $G(\mathbf{a}, \mathbf{f}^{(l-1)})$, at each layer $l$ produces two gating scores~($g_\text{mha}^{(l)}$ and $g_\text{ffn}^{(l)}$) that modulate the outputs of MHA and FFN$_1$ in the gated fusion block, respectively. 
% This gating function is designed to adaptively assess whether audio embeddings are useful to improve video representation, playing the role of a filter to enhance or suppress audio information.
To this end, the audio embedding $\mathbf{a}$ and the frame embedding $\mathbf{f}^{(l)}$ are first aggregated using average pooling, resulting in aggregated embeddings $\bar{\mathbf{a}} \in \mathbb{R}^D$ and $\bar{\mathbf{f}}^{(l-1)} \in \mathbb{R}^D$, respectively. 
These aggregated embeddings are then concatenated to form a joint representation, $\mathbf{u}^{(l)} = [\bar{\mathbf{a}}, \bar{\mathbf{f}}^{(l-1)}] \in \mathbb{R}^{2D}$.
The joint embedding $\mathbf{u}^{(l-1)}$ is passed through two distinct Multi-Layer Perceptrons (MLPs) followed by the non-linear function to compute the gating scores for the outputs of MHA and FFN$_1$. 
The gating function, $G(\mathbf{a}, \mathbf{f}^{(l-1)})$ can be formulated as follows:

\begin{equation}
\begin{aligned}
    [g_{\text{mha}}^{(l)},\ g_{\text{ffn}}^{(l)}] &= G(\mathbf{a}, \mathbf{f}^{(l-1)}) \\
    &=\sigma\Big[\left( \textrm{MLP}_{\textrm{mha}}(\mathbf{u}^{(l-1)})\right), \left( \textrm{MLP}_{\textrm{ffn}}(\mathbf{u}^{(l-1)})\right)\Big],
    % &= \tanh\left( \mathbf{W}_2\, \sigma\left( \mathbf{W}_1\, \mathbf{u}^{(l)} \right) \right),
\label{eq:gates}    
\end{aligned}
\end{equation} 
where $\sigma$ is a non-linear function (\ie, tanh).}
% \begin{equation}
% \begin{aligned}
% g_\text{mha}^{(l)} &= \tanh\left( \mathbf{W}_2^{\text{MHA}} \sigma\left( \mathbf{W}_1^{\text{MHA}} \mathbf{u}^{(l)} \right) \right), \\
% g_\text{ffn}^{(l)} &= \tanh\left( \mathbf{W}_2^{\text{FFN}} \sigma\left( \mathbf{W}_1^{\text{FFN}} \mathbf{u}^{(l)} \right) \right), \\
% \label{eq:gates}
% \end{aligned}
% \end{equation} 
% where $\mathbf{W}_1^{\text{MHA}} \in \mathbb{R}^{D \times 2D}$, $\mathbf{W}_2^{\text{MHA}} \in \mathbb{R}^{1 \times D}$, $\mathbf{W}_1^{\text{FFN}} \in \mathbb{R}^{D \times 2D}$, and $\mathbf{W}_2^{\text{FFN}} \in \mathbb{R}^{1 \times D}$ are linear projection weights; $\sigma$ denotes the activation function (\eg, GELU). 
% The $\tanh$ function bounds the gating scores up to 1, allowing the model to either enhance or suppress the influence of the audio information.}

% These gating scores $g_{\text{mha}}^{(l)}$ and $g_{\text{ffn}}^{(l)}$ are then multiplied by the outputs of the multi-head attention and the first feed-forward network in the fusion block, respectively, as previously described in~\cref{eq:fusion_process}. 
% By producing these gating scores based on the content of both modalities, the gating block ensures that only informative audio content contributes to the final video representation.
% The gating function at each layer $l$ produces scalar gating scores that modulate the outputs of MHA and FFN$_1$ in the gated fusion block. 
% This gating mechanism is designed to adaptively assess whether audio embeddings help improve the video representation, acting as a filter to enhance or suppress audio information as needed.
% To compute gating scores, the audio embedding $\mathbf{a}$ and the frame embedding $\mathbf{f}^{(l)}$ are first aggregated using average pooling, resulting in aggregated embeddings $\bar{\mathbf{a}} \in \mathbb{R}^D$ and $\bar{\mathbf{f}}^{(l)} \in \mathbb{R}^D$, respectively. 
% These aggregated embeddings are then concatenated to form a joint representation:
% \begin{equation} 
%     \mathbf{u} = [\bar{\mathbf{a}}; \bar{\mathbf{f}}^{(l)}] \in \mathbb{R}^{2D}.
%     \label{eq:concat}
% \end{equation}
% The joint embedding $\mathbf{u}^{(l)}$ is then passed through two separate Multi-Layer Perceptrons (MLPs) and tanh function to compute the gating scores for the outputs of MHA and FFN$_1$:

% \begin{align}  
% g_\text{mha}^{(l)} &= \tanh\left( \mathbf{W}_2^{\text{MHA}} \sigma\left( \mathbf{W}_1^{\text{MHA}} \mathbf{u}^{(l)} \right) \right), \\
% g_\text{ffn}^{(l)} &= \tanh\left( \mathbf{W}_2^{\text{FFN}} \sigma\left( \mathbf{W}_1^{\text{FFN}} \mathbf{u}^{(l)} \right) \right),
% \label{eq:gates}
% \end{align}
% where $\mathbf{W}_1^{\text{MHA}} \in \mathbb{R}^{D \times 2D}$, $\mathbf{W}_2^{\text{MHA}} \in \mathbb{R}^{1 \times D}$, $\mathbf{W}_1^{\text{FFN}} \in \mathbb{R}^{D \times 2D}$, and $\mathbf{W}_2^{\text{FFN}} \in \mathbb{R}^{1 \times D}$ are linear projection weights; $\sigma$ denotes the activation function (\eg, GELU). 
% The $\tanh$ function bounds the gating scores up to 1, allowing the model to either enhance or suppress the influence of the audio information.

% These gating scores $g_{\text{mha}}^{(l)}$ and $g_{\text{ffn}}^{(l)}$ are then multiplied by the outputs of the multi-head attention and the first feed-forward network in the fusion block, respectively, as previously described in~\cref{eq:fusion}. 
% By producing these gating scores based on the content of both modalities, the gating block ensures that only informative audio content contributes to the final video representation.

\bs{
\subsection{Adaptive Margin-based Contrastive Learning}
\label{sec:margin_loss}
% The output of the gated fusion transformer, video representation $\mathbf{v}\in\mathbb{R}^{N\times D}$, is aligned with text embedding $\mathbf{t}\in\mathbb{R}^D$.
% Conventionally, this video-text alignment is achieved by the cross-modal contrastive learning objective~\cite{clip,clip4clip,xpool,xclip} designed to maximize similarity scores (\eg, cosine similarity) of positive pairs and minimize the scores of negative pairs.
% These frameworks are based on binary relationships, where all cross-modal pairs that are not the matching pair (\ie, the pair of a video and its corresponding text) in a batch are treated as negative pairs. 
% % This binary labeling assumes that all negatives are equally dissimilar to the positives.
% % However, this assumption neglects the fact that some negative pairs can be semantically similar.
% % Regarding all non-matching pairs as negatives can restrict supervisory information, introducing potentially
% % poor supervisory signals during training.
% However, this binary labeling introduces potentially poor supervisory signals since it neglects the fact that some negative pairs can be semantically similar.

% discriminative representations, as it forces the model to push apart embeddings that are semantically close. 


The output of the gated fusion transformer, video representation $\mathbf{v} \in \mathbb{R}^{N \times D}$, is aligned with text embedding $\mathbf{t} \in \mathbb{R}^{D}$. Conventionally, this video-text alignment is achieved by the cross-modal contrastive learning objective~\cite{clip,clip4clip,xpool,xclip}, designed to maximize similarity scores (e.g., cosine similarity) of positive pairs and minimize the scores of negative pairs. To further enhance discriminative ability in contrastive learning, we introduce an additional margin between positive and negative pairs. While this margin enhances discriminability, applying a fixed margin uniformly across all pairs presents an issue.
A fixed margin may excessively push apart negative pairs that still share some level of semantic similarity. This rigid margin risks creating overly strict separations, potentially leading to poor generalization by disregarding inherent relationships among semantically similar pairs. 

To address this limitation, we propose an adaptive margin-based contrastive loss that dynamically adjusts margins for each negative pair, informed by their intra-modal semantic similarities. The core insight behind our approach is that semantic relationships within the visual and textual modalities provide implicit cues that can be leveraged for richer supervision. For instance, if two videos are visually similar or if two texts have high textual similarity, their cross-modal counterparts are also likely to share some level of semantic relatedness. 



% To address this limitation, we propose an adaptive margin-based contrastive loss that extends the traditional contrastive loss by incorporating an adaptive margin term for each negative pair.
% To address this limitation, we propose an adaptive margin-based contrastive loss that dynamically controls margins for each negative pair based on their intra-modal semantic similarities. %, thereby enabling the implicit exploration for more accurate supervisory signals.
% % Specifically, the proposed loss controls the margin between a negative pair according to their semantic dissimilarity within intra-modalities.
% The key intuition is that intra-modal similarities within the visual and textual modalities provide important clues for the implicit exploration of rich supervisory signals.
% Specifically, if two videos are similar in the visual space or two texts are similar in the textual space, it is likely that their cross-modal counterparts are also semantically related to some extent.  

Following this nature, given a batch with $B$ video-text pairs $\mathcal{B} =\big\{(V_i,T_i)\big\}_{i=1}^{B}$, we define the adaptive margin $m_{ij}$ for each negative pair ($V_i$,$T_j$) according to the average of their intra-modal similarities in both the visual and textual modalities. 
First of all, the frame embedding $\mathbf{f}_i$ is average pooled to obtain holistic embedding of the visual modality denoted by $\bar{\mathbf{f}_i}$.
Let $c_{ij}^{v}$ denotes the cosine similarity between $\bar{\mathbf{f}_i}$ and $\bar{\mathbf{f}_j}$, and $c_{ij}^{t}$ denotes the cosine similarity between $\mathbf{t}_i$ and $\mathbf{t}_j$. The adaptive margin is obtained by:
\begin{equation}
    m_{ij} = \min\left(\lambda \left( 1 - \frac{c_{ij}^{v} + c_{ij}^{t}}{2} \right),\ \delta \right),
    \label{eq:margin}
\end{equation}
where $\lambda$ is a scaling factor, and $\delta$ is the maximum margin to prevent excessively large margins. The operation $\min(\cdot,\cdot)$ ensures that the margin does not exceed $\delta$.
The adaptive margin $m_{ij}$ is then added to the similarity score of the negative pair in the contrastive loss function as follows:
\begin{equation}
\begin{aligned}
    \mathcal{L}(\mathcal{B}) = &-\sum_{i=1}^{B}\Bigg(\log\frac{e^{s_{ii}/\tau }}{e^{s_{ii}/\tau}+\sum_{j=1, j\neq i}^{B}e^{(s_{ij}+m_{ij})/\tau }} \Bigg) \\
    &-\sum_{i=1}^{B}\Bigg(\log\frac{e^{s_{ii}/\tau }}{e^{s_{ii}/\tau}+\sum_{j=1, j\neq i}^{B}e^{(s_{ji}+m_{ji})/\tau }} \Bigg).
    \label{eq:Margin_loss}
\end{aligned}
\end{equation}
By incorporating the adaptive margin into the contrastive loss, our method promotes a more discriminative and generalizable cross-modal embedding space that considers inherent intra-modality relationships, which leads to improved retrieval performance.

Rather than relying on simple cosine similarity, we compute an enhanced similarity score \( s \) that captures both global and local relationships between video and text representations. This combination captures complementary information, enhancing the retrieval performance as observed in the previous arts~\cite{xclip,ucofia,uatvr,prost}. 
First, for global alignment, we derive a comprehensive video representation by applying average pooling to the final video embedding, \( \mathbf{v} \in \mathbb{R}^{N \times D} \), where \( N \) represents the number of frame segments. This pooled representation, \( \mathbf{v}_g = \sum_{i=1}^{N} \mathbf{v}^i / N \in \mathbb{R}^{D} \), captures the overall content of the video. The global similarity score \( s_g \) between the video’s global representation \( \mathbf{v}_g \) and the text embedding \( \mathbf{t} \in \mathbb{R}^{D} \) is then computed as:
\begin{equation}
    s_g = \frac{\mathbf{v}_g^\top \mathbf{t}}{|| \mathbf{v}_g ||_2 || \mathbf{t} ||_2}.
\end{equation}
Next, for local alignment, we match each frame segment’s embedding \( \mathbf{v}^i \in \mathbb{R}^{D} \) with the text embedding \( \mathbf{t} \), computing segment-level similarities \( s^i = \frac{\mathbf{v}^{i\top} \mathbf{t}}{|| \mathbf{v}^i ||_2 || \mathbf{t} ||_2} \). These frame-level similarities are aggregated using the log-sum-exp (LSE) function:
\begin{equation}
    s_l = \underset{{i\in[1,N]}}{\text{LSE}}(s^i) = \log\left( \sum_{i=1}^{N} e^{\alpha s^i} \right),
\end{equation}
where \( \alpha \) is a scaling parameter that controls the smoothness of the maximum operation.
The final similarity score \( s \), which combines both global and local perspectives, is calculated by averaging \( s_g \) and \( s_l \):
\begin{equation}
    s = \frac{s_g + s_l}{2}.
    \label{eq:final_score}
\end{equation}
The final similarity score $s$ is utilized for the adaptive margin-based contrastive loss in~\cref{eq:Margin_loss}.
% Note that the final similarity scores of pairs of video and text are utilized for the retrieval system during inference.
This multi-grained alignment scheme enables the model to capture both holistic and fine-grained details, thereby enhancing video-text retrieval accuracy.
}

% Finally, the proposed learning framework ensures that the model penalizes negative pairs according to their semantic dissimilarities.
% It assigns smaller margins to semantically similar negative pairs and larger margins to semantically dissimilar ones.
% Consequently, the adaptive margin-based contrastive loss encourages the model to learn more discriminative embeddings, leading to improved performance in the video-text retrieval task.


% To obtain the alignment score $s$, used in the loss function, we employ a na\"ive multi-grained alignment scheme that is prevalent scheme across the previous arts~\cite{xclip,ucofia,uatvr,prost}.
% It combines both global alignment between the entire video and the text, and local alignment between the video frame and the text.
% To derive a global video representation, average pooling is applied to the final video representation $\mathbf{v} \in \mathbb{R}^{N \times D}$, yielding a global video representation $\mathbf{v}_g =\sum_{i=1}^{N} \mathbf{v}^i/N \in \mathbb{R}^{D}$. The global alignment score $s_g$ between the global video representation $\mathbf{v}_g$ and text embedding $\mathbf{t} \in \mathbb{R}^{D}$ is computed as $s_g = \mathbf{v}_g^\top \mathbf{t}/{|| \mathbf{v}_g ||_2 || \mathbf{t}||_2}$.
% The video representation, $\mathbf{v} \in \mathbb{R}^{N \times D}$, where $N$ is the number of frame segments, is used for local alignment by calculating the similarity between each frame segment embedding $\mathbf{v}^i \in \mathbb{R}^{D}$ and the text embedding $\mathbf{t} \in \mathbb{R}^{D}$ is denoted by $s^i = \mathbf{v}^{i\top} \mathbf{t}/{|| \mathbf{v}^i ||_2 || \mathbf{t}||_2}$.
% The local alignment score $s_l$ is then obtained by aggregating these segment-level similarities using the log-sum-exp (LSE) function, which serves as a smooth approximation of the maximum operation:
% \begin{equation}
%     s_l = \underset{{i\in[1,N]}}{\text{LSE}}(s^i) = \log\left( \sum_{i=1}^{N} e^{\alpha s^i}   \right),
%     \label{eq:local_alignment}
% \end{equation}corresponding
% where $\alpha$ is a scaling parameter.
% The final alignment score $s$ is computed by averaging the global and local alignment scores:
% \begin{equation}
%     s = \frac{s_g +  s_l}{2}.
%     \label{eq:final}
% \end{equation}
% Note that the final alignment scores of pairs of video and text are utilized for the retrieval system during inference. 

% Finally, the proposed learning framework ensures that the model penalizes negative pairs according to their semantic dissimilarities.
% It assigns smaller margins to semantically similar negative pairs and larger margins to semantically dissimilar ones.
% Consequently, the adaptive margin-based contrastive loss encourages the model to learn more discriminative embeddings, leading to improved performance in the video-text retrieval task.


% Rather than relying on simple cosine similarity, we compute an enhanced alignment score \( s \) that captures both global and local relationships between video and text representations. This combination captures complementary information, enhancing the retrieval performance as observed in the previous arts~\cite{xclip,ucofia,uatvr,prost}. 
% First, for global alignment, we derive a comprehensive video representation by applying average pooling to the final video embedding, \( \mathbf{v} \in \mathbb{R}^{N \times D} \), where \( N \) represents the number of frame segments. This pooled representation, \( \mathbf{v}_g = \sum_{i=1}^{N} \mathbf{v}^i / N \in \mathbb{R}^{D} \), captures the overall content of the video. The global alignment score \( s_g \) between the video’s global representation \( \mathbf{v}_g \) and the text embedding \( \mathbf{t} \in \mathbb{R}^{D} \) is then computed as:
% \begin{equation}
%     s_g = \frac{\mathbf{v}_g^\top \mathbf{t}}{|| \mathbf{v}_g ||_2 || \mathbf{t} ||_2}.
% \end{equation}
% Next, for local alignment, we match each frame segment’s embedding \( \mathbf{v}^i \in \mathbb{R}^{D} \) with the text embedding \( \mathbf{t} \), computing segment-level similarities \( s^i = \frac{\mathbf{v}^{i\top} \mathbf{t}}{|| \mathbf{v}^i ||_2 || \mathbf{t} ||_2} \). These frame-level similarities are aggregated using the log-sum-exp (LSE) function:
% \begin{equation}
%     s_l = \underset{{i\in[1,N]}}{\text{LSE}}(s^i) = \log\left( \sum_{i=1}^{N} e^{\alpha s^i} \right),
% \end{equation}
% where \( \alpha \) is a scaling parameter that controls the smoothness of the maximum operation.
% The final alignment score \( s \), which combines both global and local perspectives, is calculated by averaging \( s_g \) and \( s_l \):
% \begin{equation}
%     s = \frac{s_g + s_l}{2}.
% \end{equation}

% This multi-grained alignment scheme enables the model to capture both holistic and fine-grained details, thereby enhancing video-text retrieval accuracy.


% \subsection{Global-Local Alignment}
% \label{sec:align}
% The output of the gated fusion transformer, video representation $\mathbf{v}=[\mathbf{v}^1, \mathbf{v}^2, \dots, \mathbf{v}^N]\in\mathbb{R}^{N\times D}$, is aligned with text embedding with a global-local alignment scheme~\cite{xclip,ucofia,uatvr,prost}. 
% The global-local alignment scheme combines both global alignment between the entire video and the text, and local alignment between the video frame and the text.
% Below, we describe each of these alignments in more detail.

% \noindent\textbf{Global Alignment:}
% To derive a global video representation, average pooling is applied to the final video representation $\mathbf{v} \in \mathbb{R}^{N \times D}$, yielding a global video representation $\mathbf{v}_g =\sum_{i=1}^{N} \mathbf{v}^i/N \in \mathbb{R}^{D}$. The global alignment score $s_g$ between the global video representation $\mathbf{v}_g$ and text embedding $\mathbf{t} \in \mathbb{R}^{D}$ is computed as $s_g = \mathbf{v}_g^\top \mathbf{t}/{|| \mathbf{v}_g ||_2 || \mathbf{t}||_2}$.

% \noindent\textbf{Local Alignment:}
% The video representation, $\mathbf{v} \in \mathbb{R}^{N \times D}$, where $N$ is the number of frame segments, is used for local alignment by calculating the similarity between each frame segment embedding $\mathbf{v}^i \in \mathbb{R}^{D}$ and the text embedding $\mathbf{t} \in \mathbb{R}^{D}$ is denoted by $s^i = \mathbf{v}^{i\top} \mathbf{t}/{|| \mathbf{v}^i ||_2 || \mathbf{t}||_2}$.
% The local alignment score $s_l$ is then obtained by aggregating these segment-level similarities using the log-sum-exp (LSE) function, which serves as a smooth approximation of the maximum operation:
% \begin{equation}
%     s_l = \underset{{i\in[1,N]}}{\text{LSE}}(s^i) = \log\left( \sum_{i=1}^{N} e^{\alpha s^i}   \right),
%     \label{eq:local_alignment}
% \end{equation}
% where $\alpha$ is a scaling parameter.

% The final alignment score $s$ is computed by averaging the global and local alignment scores:
% \begin{equation}
%     s = \frac{s_g +  s_l}{2}.
%     \label{eq:final}
% \end{equation}
% Finally, the global-local alignment is achieved through cross-modal contrastive learning~\cite{clip} using the InfoNCE loss~\cite{oord2018representation}. 
% Given a batch with $B$ video-text pairs $\mathcal{B} =\big\{(V_i,T_i)\big\}_{i=1}^{B}$, the loss function $\mathcal{L}_{NCE}(\mathcal{B})$ is formulated by:
% \begin{equation}
%     \mathcal{L}_{NCE}(\mathcal{B}) = -\sum_{i=1}^{B}\Bigg(\log\frac{e^{s_{ii}/\tau }}{\sum_{j=1}^{B}e^{s_{ij}/\tau }} 
%     +\log\frac{e^{s_{ii}/\tau }}{\sum_{j=1}^{B}e^{s_{ji}/\tau}}\Bigg),
%     \label{eq:NCE}
% \end{equation}
% where $s_{ij}$ denotes the final alignment score between $i$-th video (\ie, $V_i$) and $j$-th text (\ie, $T_j$), and $\tau$ denotes a temperature parameter.


% \subsection{Global-Local Alignment}
% \label{sec:align}
% The output of the gated fusion transformer, video representation, is aligned with text embedding with a global-local alignment scheme~\cite{xclip,ucofia,uatvr,prost}. 
% % The primary objective of this alignment scheme is to capture both holistic semantic context and fine details.
% The global-local alignment scheme combines both global alignment between the entire video and the text, and local alignment between the video frame and the text.
% Below, we describe each of these alignments in more detail.

% \noindent\textbf{Global Alignment:}
% To derive a global video representation, average pooling is applied to the final video representation $\mathbf{v} \in \mathbb{R}^{N \times D}$, yielding a global video representation $\mathbf{v}_g =\sum_{i=1}^{N} \mathbf{v}_i/N \in \mathbb{R}^{D}$. The global alignment score $s_g$ between the global video representation $\mathbf{v}_g$ and text embedding $\mathbf{t} \in \mathbb{R}^{D}$ is computed as follows:
% \begin{equation}
%     s_g = \frac{\mathbf{v}_g^\top \mathbf{t}}{|| \mathbf{v}_g ||_2 || \mathbf{t}||_2}.
%     \label{eq:global_alignment}
% \end{equation}
% \noindent\textbf{Local Alignment:}
% The video representation, $\mathbf{v} \in \mathbb{R}^{N \times D}$, where $N$ is the number of frame segments, is used to compute local similarities. 
% Each frame segment embedding $\mathbf{v}_i \in \mathbb{R}^{D}$ is compared with the text embedding $\mathbf{t} \in \mathbb{R}^{D}$ using cosine similarity:
% \begin{equation}
%     s_i  = \frac{\mathbf{v}_i^\top \mathbf{t}}{|| \mathbf{v}_i ||_2 || \mathbf{t} ||_2}, \quad i \in [1,N].
%     \label{eq:local_sim}
% \end{equation}
% The local alignment score $s_l$ is then obtained by aggregating these segment-level similarities using the log-sum-exp (LSE) function, which serves as a smooth approximation of the maximum operation:
% \begin{equation}
%     % s_l = \text{LSE}(s_1, s_2, \dots, s_N) = \log\left( \sum_{i=1}^{N} \exp(s_i / \tau) \right),
%     s_l = \underset{{i\in[1,N]}}{\text{LSE}}(s_i) = \log\left( \sum_{i=1}^{N} e^{\alpha s_i}   \right),
%     \label{eq:local_alignment}
% \end{equation}
% where $\alpha$ is a scaling parameter.

% The final alignment score $s$ is computed by combining the global and local alignment scores:
% \begin{equation}
%     s = s_g +  s_l.
%     \label{eq:final}
% \end{equation}
% Finally, the global-local alignment for the video and text is achieved through cross-modal contrastive learning~\cite{clip} using the InfoNCE loss~\cite{oord2018representation}. 
% Given a batch with $B$ video-text pairs $\mathcal{B} =\big\{(V_i,T_i)\big\}_{i=1}^{B}$, the loss function $\mathcal{L}_{C}(\mathcal{B})$ is formulated by:
% \begin{equation}
%     \mathcal{L}_{C}(\mathcal{B}) = -\sum_{i=1}^{B}\Bigg(\log\frac{e^{s_{ii}/\tau }}{\sum_{j=1}^{B}e^{s_{ij}/\tau }} 
%     +\log\frac{e^{s_{ii}/\tau }}{\sum_{j=1}^{B}e^{s_{ji}/\tau}}\Bigg),
%     \label{eq:NCE}
% \end{equation}
% where $s_{ij}$ denotes the final alignment score between $i$-th video (\ie, $V_i$) and $j$-th text (\ie, $T_j$), and $\tau$ denotes a temperature parameter.


% \subsection{Adaptive Margin-based Contrastive Learning}
% \label{sec:margin_loss}
% In conventional contrastive learning frameworks, such as the InfoNCE loss~\cite{Sohn_nips2016, oord2018representation}, all negative pairs are treated equally while neglecting the semantic relationships of the negative pairs. 
% However, negative pairs can vary significantly in their semantic relationships. 
% For instance, a video of a ``soccer match'' is more semantically similar to a video of a ``basketball game'' than a video of ``cooking pasta''.
% Contrastive learning that ignores these relationships may lead to suboptimal representations.  

% To address this limitation, we propose an adaptive margin-based contrastive loss designed to enhance the discrimination of learned embeddings by reflecting these semantic relationships. 
% The key intuition is that intra-modal similarities within the visual and textual modalities provide important clues about the semantic relationships between samples. 
% Specifically, if two videos are similar in the visual space or two texts are similar in the textual space, it is likely that their cross-modal counterparts are also semantically related to some extent.  

% Following this nature, we define the adaptive margin $m_{ij}$ for each negative pair ($V_i$,$T_j$) according to the average of their intra-modal similarities in both the visual and textual modalities. 
% First of all, the frame embedding $\mathbf{f}_i$ is average pooled to obtain holistic embedding of the visual modality denoted by $\bar{\mathbf{f}_i}$.
% Let $s_{ij}^{v}$ denotes the cosine similarity between $\bar{\mathbf{f}_i}$ and $\bar{\mathbf{f}_j}$, and $s_{ij}^{t}$ denotes the cosine similarity between $\mathbf{t}_i$ and $\mathbf{t}_j$. The adaptive margin is obtained by:
% \begin{equation}
%     m_{ij} = \min\left(\lambda \left( 1 - \frac{s_{ij}^{v} + s_{ij}^{t}}{2} \right),\ \delta \right),
%     \label{eq:margin}
% \end{equation}
% where $\lambda$ is a scaling factor, and $\delta$ is the maximum margin to prevent excessively large margins. The operation $\min(\cdot,\cdot)$ ensures that the margin does not exceed $\delta$.
% The adaptive margin $m_{ij}$ is then added to the similarity score of the negative pair in the contrastive loss function~(\cref{eq:NCE}) as follows:
% \begin{equation}
% \begin{aligned}
%     \mathcal{L}(\mathcal{B}) = &-\sum_{i=1}^{B}\Bigg(\log\frac{e^{s_{ii}/\tau }}{e^{s_{ii}/\tau}+\sum_{j=1, j\neq i}^{B}e^{(s_{ij}+m_{ij})/\tau }} \Bigg) \\
%     &-\sum_{i=1}^{B}\Bigg(\log\frac{e^{s_{ii}/\tau }}{e^{s_{ii}/\tau}+\sum_{j=1, j\neq i}^{B}e^{(s_{ji}+m_{ji})/\tau }} \Bigg).
%     \label{eq:Margin_loss}
% \end{aligned}
% \end{equation}

% This adaptive approach ensures that the model penalizes negative pairs proportionally according to their semantic dissimilarities.
% It assigns smaller margins to semantically similar negative pairs and larger margins to semantically dissimilar ones.
% Consequently, the adaptive margin-based contrastive loss encourages the model to learn more discriminative embeddings, leading to improved performance in the video-text retrieval task.

==> Sections/_3_method_backup_0304.tex <==

\section{Proposed Method}
\label{sec:method}

\begin{figure*}[t!]
    \centering
    \vspace{-1mm}
    \includegraphics[width=0.99\linewidth]{figs/arch_v8.pdf}
    \vspace{-2mm}
    \caption{($Left$) The overall architecture of AVIGATE. Audio input is processed through an Audio Spectrogram Transformer (AST) and further refined by an audio resampler to generate fixed-size audio embeddings. Frame embeddings are derived from the video using a CLIP Image Encoder, while the text embedding is extracted by the CLIP Text Encoder. These audio and frame embeddings are fused by a gated fusion transformer, which dynamically determines the contribution of audio. 
    The final video representation is aligned with the text embedding using a multi-grained alignment scheme, facilitating an effective video-text retrieval process.
    ($Right$) The gated fusion transformer consists of a gated fusion block and a gating function.
    }
    \label{fig: arch}
    \vspace{-2.5mm}
\end{figure*}
\iffalse
In this section, we describe our novel framework, AVIGATE.
Firstly, we present embedding extraction for each modality with its encoder~(\cref{sec:extraction}). 
Then, the gated fusion transformer is introduced~(\cref{sec:gate}). 
Lastly, we describe the adaptive margin-based contrastive learning strategy~(\cref{sec:margin_loss}).
The overall architecture of our framework is depicted in Figure~\ref{fig: arch}.
\fi
This section presents details of our video-text retrieval framework, dubbed AVIGATE; its overall architecture is depicted in Figure~\ref{fig: arch}. 
We first describe the embedding extraction process for each modality in ~\cref{sec:extraction}, and then elaborate on the gated fusion transformer in~\cref{sec:gate}. 
Finally, the adaptive margin-based contrastive learning strategy is introduced in~\cref{sec:margin_loss}.
\subsection{Embedding Extraction}
\label{sec:extraction}

AVIGATE utilizes three pre-trained encoders to process each modality: Two CLIP encoders~\cite{clip} for the video frames and the text descriptions, respectively, and Audio Spectrogram Transformer (AST)~\cite{ast} for the audio signals.

\noindent\textbf{Frame Embeddings:} We utilize the pre-trained CLIP image encoder~\cite{clip} to extract the frame embeddings of each video.
Given an input video $V$, $N$ frames are first uniformly sampled denoted as $V=[F^1, F^2, \dots, F^N]$. 
Each frame is divided into non-overlapping patches, which are then transformed using a linear projection. 
A [\texttt{CLS}] token is prepended to this sequence of patches, and the combined sequence is fed to the CLIP image encoder. 
The output corresponding to the [\texttt{CLS}] token is taken as the frame embedding.
Finally, these frame embeddings are concatenated to form a sequence of frame embeddings, $\mathbf{f}=[\mathbf{f}^1, \mathbf{f}^2, \dots, \mathbf{f}^N]\in\mathbb{R}^{N\times D}$, where $D$ denotes the dimension of the embeddings. 

\noindent\textbf{Text Embeddings:} The text embedding extraction is carried out by the CLIP text encoder~\cite{clip}, as in the frame embedding extraction. 
Given a text input $T$, all words in the text are tokenized and enclosed with special tokens [\texttt{SOS}] and [\texttt{EOS}], indicating the start and the end of the sentence, respectively. 
This complete sequence is then passed through the CLIP text encoder.
Then, the output corresponding to the [\texttt{EOS}] token is regarded as the text embedding, $\mathbf{t} \in \mathbb{R}^{D}$, capturing the overall semantics of the input text.


\noindent\textbf{Audio Embeddings:} We employ AST~\cite{ast} as our audio encoder following prior work~\cite{ast, tefal}. The audio input $A$ from the video $V$ is first converted into a Mel-spectrogram, capturing key audio features across time and frequency. 
AST processes this spectrogram as a sequence of $N_a$ patches, using transformer layers to generate a detailed set of audio embeddings.
However, since audio signals are much more densely sampled compared to video frames, directly fusing all $N_a$ audio embeddings with frame embeddings would be computationally expensive. 
To address this, we employ an additional query-based transformer~(\ie, audio resampler)~\cite{perceiver, detr, flamingo} that uses a cross-attention mechanism with $M$ learnable query embeddings. 
This design reduces the number of audio embeddings to a fixed length of $M$, $\mathbf{a}=[\mathbf{a}^1, \mathbf{a}^2, \dots, \mathbf{a}^{M}] \in \mathbb{R}^{M \times D}$, maintaining essential audio information while significantly lowering computational load for subsequent fusion with visual modalities. We freeze the pretrained AST parameters during training, avoiding the high computational cost of fine-tuning. Architectural details are provided in the supplementary material.

\subsection{Gated Fusion Transformer}
\label{sec:gate}


To effectively fuse the audio embeddings $\mathbf{a}$ and frame embedding $\mathbf{f}$, the gated fusion transformer is designed to dynamically adjust the contribution of audio based on its relevance to the video. This transformer achieves adaptive fusion by using gating scores that modulate the impact of audio features on the video representation, ensuring that irrelevant audio signals have a reduced influence, thus preserving the integrity of the visual content.

The gated fusion transformer consists of $L$ layers, each containing a gated fusion block that applies gating scores to control the fusion process. Within each block, Multi-Head Attention (MHA) and a Feed-Forward Network (FFN) blend the audio and frame embeddings, with the adaptive gating function providing scores ($g_{\textrm{mha}}$ and $g_{\textrm{ffn}}$) to regulate their influence. These gating scores control the contribution of audio embeddings, enabling the transformer to integrate complementary audio cues when relevant while minimizing the effect of potentially noisy audio. This is followed by Multi-Head Self-Attention (MHSA) and a Feed-Forward Network (FFN) to refine the representation.

When the gating scores are high, audio cues are emphasized, enhancing the representation by capturing complementary audio details. Conversely, low gating scores prioritize the robustness of the visual content against irrelevant audio interference. This selective fusion leads to a more context-sensitive and discriminative video representation, which improves video-text retrieval performance. In the following, we provide architectural details of the two core components of the gated fusion transformer: the gated fusion block and the gating function.

\subsubsection{Gated Fusion Block}
\label{sec:fusion}
The gated fusion block takes the audio embeddings $\mathbf{a}$ and the frame embeddings $\mathbf{f}$ as inputs and outputs video representation through the fusion process followed by the refining process.
Specifically, with a series of $L$ layers, the frame embeddings $\mathbf{f}$ evolve into refined $\mathbf{f}^{(L)}$ by capturing cross-modal interactions with the audio embeddings $\mathbf{a}$, where $\mathbf{f}$ directly from the CLIP image encoder is regarded as initial input $\mathbf{f}^{(0)}$.
The refined $\mathbf{f}^{(L)}$ serves as the final video representation $\mathbf{v}=[\mathbf{v}^1, \mathbf{v}^2, \dots, \mathbf{v}^N]\in\mathbb{R}^{N\times D}$.



In the fusion process, $\mathbf{f}^{(l-1)}$ is fused with $\mathbf{a}$ by MHA with a residual connection.
The output is modulated by a gating score $g_{\textrm{mha}}$ generated by the gating function~(\cref{sec:gating_function}) to determine the contribution of the audio embedding in the fusion.
Then, the output is fed into an FFN with a residual connection, which is also modulated by a gating score $g_{\textrm{ffn}}$, ensuring selective enhancement based on the gating mechanism.
The fusion process is formulated as follows:
\begin{equation}
    \begin{aligned}
    \mathbf{z}^{(l)} &=  g_{\textrm{mha}}^{(l)} \cdot \textrm{MHA}(\textrm{LN}(\mathbf{f}^{(l-1)}), \textrm{LN}(\mathbf{a})) +\mathbf{f}^{(l-1)} , \\
    \bar{\mathbf{z}}^{(l)} &= g_{\textrm{ffn}}^{(l)} \cdot \textrm{FFN}_1(\textrm{LN}(\mathbf{z}^{(l)})) + \mathbf{z}^{(l)},
    \label{eq:fusion_process}
    \end{aligned}
\end{equation}
where LN denotes the layer normalization.
MHA involves $n$-head attention operations; it is formulated by
\begin{equation}
\begin{aligned}
    \textrm{MHA}(\mathbf{X},\mathbf{Y}) &= [\textrm{Attn}^1(\mathbf{X},\mathbf{Y}), ..., \textrm{Attn}^n(\mathbf{X},\mathbf{Y})]\mathbf{W}_o,\\ 
    \textrm{Attn}^i(\mathbf{X},\mathbf{Y}) &= \text{softmax}\left( \frac{(\mathbf{X}\mathbf{W}_{q}^{i}) (\mathbf{Y}\mathbf{W}_k^{i})^\top}{\sqrt{D_h}} \right) (\mathbf{Y}\mathbf{W}_v^{i})
    \label{eq:MHA}
\end{aligned}
\end{equation}
where $[\cdot,\cdot]$ denotes concatenation, and $D_h$ is set to $D/n$. 
$\mathbf{W}_{q}^{i}, \mathbf{W}_{k}^{i}, \mathbf{W}_{v}^{i}\in\mathbb{R}^{D\times D_h}$ and $\mathbf{W}_{o}\in\mathbb{R}^{D\times D}$ are linear projection matrices.

The fused representation $\bar{\mathbf{z}}^{(l)}$ undergoes the refining process to enhance the overall video representation.
Specifically, $\bar{\mathbf{z}}^{(l)}$ is fed into a Multi-Head Self-Attention (MHSA) module with a residual connection.
Then, the second FFN with a residual connection is applied to the output of MHSA to produce the refined frame embeddings $\mathbf{f}^{(l)}$. 
The refining process is formulated as follows:
\begin{equation}
\begin{aligned}
    \Tilde{\mathbf{z}}^{(l)} &= \textrm{MHSA}(\textrm{LN}(\bar{\mathbf{z}}^{(l)})) + \bar{\mathbf{z}}^{(l)} , \\
    \mathbf{f}^{(l)} &= \textrm{FFN}_2(\textrm{LN}(\Tilde{\mathbf{z}}^{(l)})) + \Tilde{\mathbf{z}}^{(l)}.
    \label{eq:refining_process}
\end{aligned}
\end{equation}
Similar to MHA, MHSA involves $n$-head self-attention operations, where $\textrm{MHSA}(\textrm{X})=\textrm{MHSA}(\textrm{X},\textrm{X})$.% in~\cref{eq:MHA}.



\subsubsection{Gating Function}
\label{sec:gating_function}
The gating function, $G(\mathbf{a}, \mathbf{f}^{(l-1)})$ at each layer $l$ produces two gating scores, $g_\text{mha}^{(l)}$ and $g_\text{ffn}^{(l)}$, that modulate the outputs of MHA and FFN$_1$ in the gated fusion block, respectively. 
To this end, the audio embeddings $\mathbf{a}$ and the frame embeddings $\mathbf{f}^{(l-1)}$ are first aggregated using average pooling, resulting in $\bar{\mathbf{a}} \in \mathbb{R}^D$ and $\bar{\mathbf{f}}^{(l-1)} \in \mathbb{R}^D$, respectively. 
These aggregated embeddings are then concatenated to form a joint representation, $\mathbf{u}^{(l)} = [\bar{\mathbf{a}}; \bar{\mathbf{f}}^{(l-1)}] \in \mathbb{R}^{2D}$.
The joint embedding $\mathbf{u}^{(l)}$ is passed through two distinct Multi-Layer Perceptrons (MLPs) followed by a non-linear function to compute the gating scores for the outputs of MHA and FFN$_1$. 
The gating function, $G(\mathbf{a}, \mathbf{f}^{(l-1)})$ is formulated as follows:
\begin{equation}
\begin{aligned}
    [g_{\text{mha}}^{(l)},\ g_{\text{ffn}}^{(l)}] &= G(\mathbf{a}, \mathbf{f}^{(l-1)}) \\
    &=\sigma\Big[\left( \textrm{MLP}_{\textrm{mha}}(\mathbf{u}^{(l-1)})\right), \left( \textrm{MLP}_{\textrm{ffn}}(\mathbf{u}^{(l-1)})\right)\Big],
\label{eq:gates}    
\end{aligned}
\end{equation} 
where $\sigma$ is a non-linear function (\ie, tanh).


\subsection{Adaptive Margin-based Contrastive Learning}
\label{sec:margin_loss}

The output of the gated fusion transformer, video representation $\mathbf{v} \in \mathbb{R}^{N \times D}$, is aligned with text embedding $\mathbf{t} \in \mathbb{R}^{D}$. 
This video-text alignment has been, in general, achieved by the cross-modal contrastive learning~\cite{clip,clip4clip,xpool,xclip}, which maximizes similarity scores (e.g., cosine similarity) of positive pairs and minimizes the those of negative pairs.
\iffalse
To further enhance discriminative ability in contrastive learning, we introduce an additional margin between a pair of negative data. 
The concept of margins has been widely explored in prior works on metric learning~\cite{kim2020proxy,deng2019arcface, kim2024efficient}, showing their effectiveness in enforcing clear separation between a negative pair.
\iffalse
% However, applying a fixed margin across all negative pairs presents an issue.
% A fixed margin may excessively push apart negative pairs that still share some level of semantic similarity. This rigid margin risks creating overly strict separations, potentially leading to poor generalization by disregarding inherent relationships among semantically similar pairs. 
To address this limitation,\fi
% However, a fixed margin may not account for varying degrees of semantic similarity among negative pairs.

Motivated by this, we propose an adaptive margin-based contrastive loss that dynamically adjusts margins for each negative pair, informed by their intra-modal semantic similarities. 
\fi

To further enhance the discriminative ability of contrastive learning, we introduce an adaptive margin-based contrastive loss that dynamically adjusts margins for each negative pair based on their intra-modal semantic similarities. The key idea of our method is that semantic relationships within each visual and textual modality provide implicit cues for determining appropriate margins. For instance, if two videos are visually similar or if two texts have high textual similarity, their cross-modal counterparts are also likely to have some level of semantic relatedness. 
In contrast to fixed-margin contrastive loss~\cite{kim2020proxy,deng2019arcface, kim2024efficient}, which applies the same margin to all negative pairs, our method accounts for varying degrees of semantic similarity between negative pairs. This adaptability enables the model to learn discriminative features while maintaining strong generalization by considering the inherent relationships between semantically similar pairs.

\iffalse
The core insight behind our method is that semantic relationships within each visual and textual modality provide implicit cues that can be leveraged for richer supervision. 
For instance, if two videos are visually similar or if two texts have high textual similarity, their cross-modal counterparts are also likely to have some level of semantic relatedness. 
\fi


Following this nature, given a batch with $B$ video-text pairs $\mathcal{B} =\big\{(V_i,T_i)\big\}_{i=1}^{B}$, we define the adaptive margin $m_{ij}$ for each negative pair ($V_i$,$T_j$) according to the average of their intra-modal similarities in both the visual and textual modalities. 
First of all, the frame embedding $\mathbf{f}_i$ is average pooled to obtain holistic embedding of the visual modality denoted by $\bar{\mathbf{f}_i}$.
Let $c_{ij}^{v}$ denotes the cosine similarity between $\bar{\mathbf{f}_i}$ and $\bar{\mathbf{f}_j}$, and $c_{ij}^{t}$ denotes the cosine similarity between $\mathbf{t}_i$ and $\mathbf{t}_j$. The adaptive margin is obtained by:
\begin{equation}
    m_{ij} = \min\left(\lambda \left( 1 - \frac{c_{ij}^{v} + c_{ij}^{t}}{2} \right),\ \delta \right),
    \label{eq:margin}
\end{equation}
where $\lambda$ is a scaling factor, and $\delta$ is the maximum margin to prevent excessively large margins. The operation $\min(\cdot,\cdot)$ ensures that the margin does not exceed $\delta$.
The adaptive margin $m_{ij}$ is then added to the similarity score of the negative pair in the contrastive loss function as follows:
\begin{equation}
\begin{aligned}
    \mathcal{L}(\mathcal{B}) = &-\sum_{i=1}^{B}\Bigg(\log\frac{e^{s_{ii}/\tau }}{e^{s_{ii}/\tau}+\sum_{j=1, j\neq i}^{B}e^{(s_{ij}+m_{ij})/\tau }} \Bigg) \\
    &-\sum_{i=1}^{B}\Bigg(\log\frac{e^{s_{ii}/\tau }}{e^{s_{ii}/\tau}+\sum_{j=1, j\neq i}^{B}e^{(s_{ji}+m_{ji})/\tau }} \Bigg).
    \label{eq:Margin_loss}
\end{aligned}
\end{equation}
By incorporating the adaptive margin into the contrastive loss, our method promotes a more discriminative and generalizable cross-modal embedding space that considers inherent intra-modality relationships, which leads to improved retrieval performance.
\input{tabs/table1}

To compute a similarity score, rather than simply leveraging cosine similarity, we employ an enhanced method that captures both global and local relationships between video and text representations. This combination captures complementary information, enhancing the retrieval performance as observed in the previous arts~\cite{xclip,ucofia,uatvr,prost}. 
First, for global alignment, we derive a comprehensive video representation by applying average pooling to the final video embedding, $\mathbf{v}=[\mathbf{v}^1, \mathbf{v}^2, \dots, \mathbf{v}^N]\in\mathbb{R}^{N\times D}$, where $N$ represents the number of frame segments. This pooled representation,  $\mathbf{v}_g = \sum_{i=1}^{N} \mathbf{v}^i / N \in \mathbb{R}^{D}$, captures the overall content of the video. The video-text similarity score $s_g$ between the global representation of the video $\mathbf{v}_g$ and the text embedding $\mathbf{t} \in \mathbb{R}^{D}$ is then computed as:
\begin{equation}
    s_g = \frac{\mathbf{v}_g^\top \mathbf{t}}{|| \mathbf{v}_g ||_2 || \mathbf{t} ||_2}.
\end{equation}
Next, for local alignment, we match each frame segment embedding $\mathbf{v}^i \in \mathbb{R}^{D}$ with the text embedding $\mathbf{t}$, computing frame-text similarities $s^i = \frac{\mathbf{v}^{i\top} \mathbf{t}}{|| \mathbf{v}^i ||_2 || \mathbf{t} ||_2}$. These frame-text similarities are aggregated using the log-sum-exp (LSE) function:
\begin{equation}
    s_l = \underset{{i\in[1,N]}}{\text{LSE}}(s^i) = \log\left( \sum_{i=1}^{N} e^{\alpha s^i} \right),
    \label{eq:local_alignment}
\end{equation}
where $\alpha$ is a scaling parameter that controls the smoothness of the maximum operation.
The final similarity score $s$, which combines both global and local perspectives, is calculated by averaging $s_g$ and $s_l$:
\begin{equation}
    s = \frac{s_g + s_l}{2}. 
    \label{eq:final_score}
\end{equation}
The final similarity score $s$ is utilized for the adaptive margin-based contrastive loss in~\cref{eq:Margin_loss}.
This multi-grained alignment scheme enables the model to capture both holistic and fine-grained details, thereby enhancing video-text retrieval accuracy.


==> Sections/_4_experiments_backup_0304.tex <==
%\input{tabs/table1.tex}



\section{Experiments}
\label{sec:experiments}
In this section, we present a comprehensive evaluation of the proposed framework, \textit{AVIGATE}. 
We first describe the experimental setup, including the datasets, evaluation metric, and implementation details in~\cref{sec:setup}. 
We then provide quantitative results to show the effectiveness of AVIGATE compared to state-of-the-art methods in~\cref{sec:quan}. 
Next, we include the qualitative results of AVIGATE in~\cref{sec:qual}. 
Moreover, we conduct ablation studies to analyze the impact of components of AVIGATE in~\cref{sec:ablation}.
Lastly, we demonstrate the efficiency of AVIGATE compared to previous arts by analyzing the computational costs in~\cref{sec:complexity}.
\subsection{Experimental Setup}
\label{sec:setup}
\noindent\textbf{Datasets:}
% Audio 있는 dataset만 사용
On two public benchmarks, MSR-VTT~\cite{msrvtt} and VATEX~\cite{vatex}, we evaluate and compare the performance of our method against previous methods.
MSR-VTT, the most common dataset for video-text retrieval, contains 10,000 videos collected from the web, including audio signals. Each video is 10 to 32 seconds long and has 20 corresponding text descriptions. Following the data split from~\cite{mmt,clip4clip}, we train AVIGATE on 9,000 videos (180,000 video-text pairs) and evaluate it on 1,000 selected video-text pairs. Out of the 10,000 videos, 9,582 have audio, which we utilize in our method.
VATEX contains 34,991 videos with multiple text descriptions for each video.  We follow the split protocol of~\cite{hgr} with 25,991 videos for training, 1,500 videos for validation, and 1,500 for testing, respectively.

\noindent \textbf{Evaluation Metric:} 
We employ the standard metric of recall at $K$ (R@$K$, with $K$ = 1, 5, 10) to evaluate retrieval performance for both text-to-video and video-to-text retrieval tasks. In both cases, samples are ranked based on their similarities to the query (in~\cref{eq:final_score}). 
We also report the RSUM, which is the sum of all R@$K$ metrics.
Retrieval is considered successful if at least one relevant item appears within the Top-K positions.


\begin{figure*}[t!]
    \vspace{-1mm}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/Qual_v2.pdf}
    \vspace{-3.5mm}
    \caption{ Top-1 text-to-video retrieval results of our method on MSR-VTT, where they are true matches. 
    $g_{mha}^{(l)}$ and $g_{ffn}^{(l)}$ denote the gating scores for $l$-th layers of the gated fusion transformer. 
    The audio provides informative cues for accurate retrieval, where ``a man is talking'' in the query text is not visible (a). The irrelevant audio is filtered by the gated fusion transformer, leading to an accurate retrieval result (b).   
    }
    \label{fig: qual}
    \vspace{-4.5mm}
\end{figure*}

\noindent\textbf{Implementation Details:}
%audio 없는 instance는 zero input 들어가는거 꼭 넣어주기
We adopt the pre-trained CLIP models from OpenAI~\cite{clip} with two different sizes of image encoder, \ie, ViT-B/32 and ViT-B/16. Moreover, we adopt AST pre-trained on ImageNet~\cite{imagenet} and AudioSet~\cite{audioset} with DeiT~\cite{DeiT} backbone.
Note that we set the audio input as zero vector for the videos that do not include audio signals. 
The dimension $D$ of audio, frame, and text embeddings is set to 512. Our model is optimized using the Adam optimizer~\cite{Adamsolver} for five epochs with a batch size of 128 for all experiments.
The initial learning rate is set to $\expnum{1}{7}$ for the CLIP encoders and $\expnum{1}{4}$ for other modules, using a cosine warm-up strategy~\cite{warmup}, while AST is frozen. 
Following~\cite{clip4clip}, the number of frames $N$ is set to 12, and the max length of the text description is set to 32.
The fixed length of resampled audio embedding $M$ is set to 12. 
The number of layers of the gated fusion module $L$ is set to 4. We use the scaling parameter $\alpha$ in~\cref{eq:local_alignment} of 100. 
$\lambda$ in~\cref{eq:margin} is set to 0.2.
Except for $\delta$ in~\cref{eq:margin}, the same hyperparameter settings are used in both MSR-VTT and VATEX.
$\delta$ is set to 0.1 and 0.05 for MSR-VTT and VATEX, respectively.
\input{tabs/table2}

\subsection{Quantitative Results}
\label{sec:quan}
%Table~\ref{tab:main_results} presents the quantitative results of video-text retrieval on MSR-VTT 9k split~\cite{msrvtt}. 
% Our proposed approach demonstrates superior performance compared to existing methods, including both text-to-video and video-to-text retrieval tasks. 
% % We evaluate retrieval performance using recall metrics at ranks 1, 5, and 10 (R@1, R@5, R@10), which are widely adopted to measure the effectiveness of retrieval systems.
% For the CLIP ViT-B/32~\cite{clip} backbone, our method outperforms state-of-the-art models such as TEFAL~\cite{tefal} and UCoFiA~\cite{ucofia}, achieving R@1 of 50.2\% for text-to-video retrieval, surpassing TEFAL by 0.8\%. Similarly, our approach obtains a substantial gain in video-to-text retrieval, achieving R@1 of 49.7\%. 
% The improvement is consistent across higher recall metrics, highlighting the effectiveness of our audio-guided video representation framework.

% When evaluated with a large size backbone (\ie, CLIP ViT-B/16~\cite{clip}), our method further shows its robustness by achieving R@1 scores of 52.1\% and 51.2\% for text-to-video and video-to-text retrieval, respectively. 
% This performance surpasses other approaches, including UCoFiA and TEFAL, demonstrating the efficacy of incorporating audio modality alongside visual and textual information.
% The consistent improvements across different backbones and retrieval tasks underscore the benefits of our approach in bridging the modality gap and effectively fusing audio-visual information. 
% These quantitative results affirm the advantage of our method in achieving state-of-the-art retrieval performance.
We compare AVIGATE with previous video-text retrieval methods on the MSR-VTT 9k split~\cite{msrvtt} and VATEX~\cite{vatex} datasets, with results presented in Table~\ref{tab:main_results} and Table~\ref{tab:vatex}, respectively.
Each table shows the modalities used by the methods for video-text retrieval, indicated as visual (V), textual (T), and audio (A), with results reported separately for each CLIP ViT backbone size.

%As shown in the tables, our method outperforms previous methods.
%We demonstrate superior performance across all datasets and CLIP ViT backbone sizes in terms of R@1.
These tables demonstrate that AVIGATE outperforms all previous methods in R@1 across all datasets and CLIP ViT backbone sizes.
% Specifically, on MSR-VTT, AVIGATE using the CLIP ViT-B/32 backbone achieves improvements over TEFAL~\cite{tefal}, the previous state-of-the-art audio-based model, by 0.8\%p and 2.6\%p in R@1 for text-to-video and video-to-text retrieval tasks, respectively.
% Moreover, AVIGATE surpasses UATVR~\cite{uatvr} by a large margin, 1.8\%p in terms of R@1 for text-to-video retrieval on VATEX.
Specifically, on MSR-VTT, AVIGATE achieves improvements of 0.8\%p and 2.6\%p over TEFAL~\cite{tefal} (w/ audio SOTA) in text-to-video retrieval and video-to-text retrieval, respectively.
Ours also surpasses UATVR~\cite{uatvr} (w/o audio, but SOTA) by a large margin, 1.8\%p in R@1 on VATEX.
\iffalse
As shown in the tables, our method outperforms previous methods across all datasets and CLIP ViT backbone sizes.
We demonstrate superior performance not only in R@1 but also R@5, R@10 and Rsum, indicating consistently strong retrieval results.
%In particular, compared to TEFAL which incurs high computational costs to extract text-guided audio and visual features, we achieve superior performance while requiring lower computational costs by using only audio-guided visual features.
In particular, compared to TEFAL, which hinders the efficiency of the retrieval system by extracting text-guided audio and visual features, we achieve superior performance by using only audio-guided video representation, allowing for a more suitable retrieval process.
\fi
The improvements of AVIGATE become more distinctive when a larger backbone is used.
% For the larger ViT backbone, AVIGATE outperforms prior state-of-the-art methods~\cite{uatvr,ucofia} by a large margin in both R@1 and RSum on both MSR-VTT and VATEX.
Specifically, on MSR-VTT, AVIGATE achieves a 1.3\%p improvement in text-to-video retrieval and a 3.1\%p in video-to-text retrieval while achieving a 3.0\%p improvement in text-to-video retrieval on VATEX.
Furthermore, our method demonstrates significant improvements in RSum, with 6.6\%p improvements on MSR-VTT.
% These quantitative results demonstrate that our method  
The superior performance of AVIGATE is attributed to its ability to selectively integrate informative audio cues while dynamically adjusting the semantic alignment between video and text, leading to a more discriminative and generalizable cross-modal representation.
\subsection{Qualitative Results}
\label{sec:qual}
% To demonstrate the effectiveness of AVIGATE, %we present the Top-1 retrieved video results given a text query, along with gating scores from the gated fusion transformer.
% In Figure~\ref{fig: qual}, we present Top-1 retrieved video results for the given text query, including the paired audio signal and layer-wise gating scores.
Figure~\ref{fig: qual} illustrates the Top-1 retrieved video results from our method for the given text query, including the paired audio signal and layer-wise gating scores.
% In cases where the audio is uninformative, simple audio-video fusion without gating leads to retrieval failure.
% In contrast, our model assigns low gating scores to uninformative audio, effectively filtering out uninformative signals and retrieving the relevant video.
% Figure~\ref{fig: qual}(a) illustrates a scenario where the audio is informative.
% In this case, our model achieves successful retrieval with high gating scores that enable effective audio fusion.
% However, the baseline model that ignores audio information fails in retrieval.
\iffalse
For the query ``a man is talking about a sports car he is driving''~(Figure~\ref{fig: qual}(a)), our model retrieves the correct video, supported by the informative audio cues that match the content of the query. 
\fi
For the query in Figure~\ref{fig: qual}(a), our model retrieves the correct video, supported by the informative audio cues that match the content of the query. 
% In this example, the audio contains meaningful spoken descriptions, which are reflected in high gating scores ($g_{\text{mha}}^{(l)}$ and $g_{\text{ffn}}^{(l)}$) except $g_{\text{mha}}^{(0)}$, emphasizing the relevance of the auditory information. 
In this example, the audio provides valuable information, reflected by relatively high gating scores ($g_{\text{mha}}^{(l)}$ and $g_{\text{ffn}}^{(l)}$) except $g_{\text{mha}}^{(1)}$ across layers, emphasizing the contribution of the audio in the fusion.
\iffalse
Conversely, for the query ``a man with a very red nose''~(Figure~\ref{fig: qual}(b)), the successfully retrieved video includes background music that is irrelevant content. 
\fi
Conversely, for the query in Figure~\ref{fig: qual}(b), the successfully retrieved video includes background music that is irrelevant content.
The gating mechanism responds accordingly, assigning low gating scores to suppress the influence of irrelevant audio signals. 
This behavior shows that the gated fusion transformer successfully filters out irrelevant audio while using the multi-modal nature of videos only when the audio contributes positively. 
% It demonstrates that our gated fusion transformer can adaptively control the integration of audio embeddings, ensuring that only useful cues contribute to the final video representation. 


\subsection{Ablation Studies}
\label{sec:ablation}
%We evaluate the effectiveness of different components in AVIGATE through comprehensive experiments. 
%The default image encoder is CLIP ViT-B/32~\cite{clip}, and the text-to-video retrieval results are reported on the widely-used MSR-VTT dataset~\cite{msrvtt}.
We evaluate the effectiveness of the proposed components in AVIGATE through comprehensive experiments.
For the ablation study, we report text-to-video retrieval results on the MSR-VTT dataset~\cite{msrvtt} with CLIP ViT-B/32~\cite{clip}. %as the image encoder.

\noindent \textbf{Components of AVIGATE:}
In Table~\ref{tab:ablation_components}, we present the results of the ablation study on the main components of our model.
% A baseline model, which utilizes only video-text modalities without additional audio modality, achieves 45.4\%, 72.2\%, and 81.6\% in terms of R@1, R@5 and R@10, respectively.
We first build a baseline that includes only the CLIP encoders for video and text embeddings, which is learned by a conventional cross-modal contrastive loss.
%When the audio modality is added, we observe an overall performance improvement, indicating that audio contributes positively to text-to-video retrieval.
% \iffalse
Then, the baseline is extended by introducing a simplified fusion transformer without the gating mechanism from our gated fusion transformer to exploit audio modality (Baseline + Audio).
The extended baseline improves overall performance, particularly with a notable 1.7\%p improvement in R@1, demonstrating that audio contributes positively to text-to-video retrieval.
% \fi
\iffalse
Additionally, in the baseline model, we introduce a simplified fusion transformer without the gating mechanism from our gated fusion transformer to add the audio modality to the visual modality.
This integration leads to an overall performance improvement, indicating that audio contributes positively to text-to-video retrieval.
\fi
Subsequently, introducing our main components, including the gated fusion transformer and adaptive margin, consistently improves the extended baseline in all metrics when each component is applied individually.
This observation highlights the effectiveness of the gated fusion transformer, which dynamically adjusts the contribution of the audio, and the benefit of contrastive learning with adaptive margin.
The full configuration of our method achieves the best performance in R@1 at 50.2\% while demonstrating consistent improvements and highlighting the complementary synergy between the gated fusion transformer and the adaptive margin-based contrastive loss.
It is worth noting that employing a fixed margin ($m_{ij}$ in Eq.~\ref{eq:margin} is fixed as 0.1) with the gated fusion transformer achieves a moderate performance gain in R@1, but the most significant improvement is presented when the margin is adaptively employed.
% the superiority of our adaptive margin-based contrastive learning, with a 1.2\%p improvement in R@1 compared to using a fixed margin instead.

% \noindent \textbf{Layer Depth of Gated Fusion Transformer:}
% We present the impact of the number of layers of the gated fusion transformer ($L$) in Table~\ref{tab:ablation_hyp}(a)  and observe that the performance gradually improves up to $L$=4.%, where the best performance is achieved.
%best performance is achieved at $L$=4.
\input{tabs/table_ablation}
\input{tabs/table_hyp}
\noindent \textbf{Granularity of Alignment Scheme:}
We analyze alignment schemes in terms of granularity in Table~\ref{tab:ablation_hyp}, demonstrating that the global-local multi-grained alignment scheme improves performance across all metrics due to its ability to capture the overall semantic context and fine details.

% We explore the influence of the number of layers in the gated fusion transformer and the alignment scheme at global and local levels. 
% In Table~\ref{tab:ablation_hyp}(a), we examine various layer configurations of the gated fusion transformer ($L$) and observe that the best performance is achieved at $L$=4. 
% Lastly, we analyze alignment schemes in terms of granularity in Table~\ref{tab:ablation_hyp}(b), demonstrating that the global-local multi-grained alignment scheme achieves superior performance across all metrics due to its ability to capture both the overall semantic context and fine details.
%\bs{Need to define what is baseline, gate, and margin in the table.}



\subsection{Computational Cost Analysis}
\label{sec:complexity}
\input{tabs/table_complexity}
Let $\mathcal{T}$, $\mathcal{V}$, and $\mathcal{A}$ denote the number of text queries, videos, and audios, respectively, where $\mathcal{A} \leq \mathcal{V}$, as each audio is associated with a corresponding video but not all videos include an audio.
% To demonstrate the efficiency of our model during testing, we compare the computational complexity and latency of AVIGATE with previous methods~\cite{clip4clip,xpool,tefal}, as summarized in Table~\ref{tab:complexity}.
Table~\ref{tab:complexity} compares the computational complexity and latency of AVIGATE with previous methods~\cite{clip4clip,xpool,tefal} to demonstrate the efficiency of our model during testing.
% Specifically, we analyze the time complexity in terms of the required operations for text-to-video retrieval and evaluate the latency for computing similarity scores between pairs of video and text.
% Given $\mathcal{T}$ text queries and $\mathcal{V}$ videos including $\mathcal{A}$ audios, 
AVIGATE achieves an efficient retrieval process with a time complexity of $\mathcal{O}(\mathcal{A}+\mathcal{V} + \mathcal{T})$, while TEFAL introduces additional computational burdens with complexity of $\mathcal{O}(\mathcal{AT} + \mathcal{VT})$.
% We further evaluate the latency for text-to-video retrieval, which involves processing a single text query against a large set of video representations. 
We further evaluate the average latency involved in processing a single text query against a large set of pre-extracted video representations for text-to-video retrieval.
Specifically, we utilize the MSR-VTT-9k test split~\cite{msrvtt}, which comprises 1,000 video-text pairs, where the video representations are pre-extracted and stored, eliminating the need for on-the-fly computation during the retrieval process.
When a text query arrives, the system computes similarity scores between the text embedding and the entire set of video representations. 
% The total latency encompasses two primary components: the time required to extract the text query embedding and the time taken to calculate the similarity scores between the text embedding and all video representations.
The total latency encompasses the extraction of the text embedding and calculating similarity scores between the text embedding and all video representations.
AVIGATE is over 14 times faster than TEFAL and over 6 times faster than X-Pool, as they require cross-modal interaction processes repeatedly for all videos with each text query to generate their final representations, resulting in substantial latency overhead.
% since they necessitate additional cross-modal interaction processes for each text query to generate the final video representations, resulting in substantial latency overhead.
Meanwhile, ours incurs only a slight additional cost due to our multi-grained alignment compared to CLIP4Clip.
% Also, it is worth noting that AVIGATE surpasses TEFAL in terms of R@1 and RSum, as shown in Table~\ref{tab:complexity}.

==> Sections/_7_supple_backup_0304.tex <==





\section{More Architectural Details}
\label{supp_sec:archi}
To efficiently fuse audio embeddings with frame embeddings while reducing computational overhead, we introduce an audio resampler using a query-based transformer framework~\cite{perceiver,detr,flamingo} that utilizes a cross-attention mechanism with $M$ learnable query embeddings. 
Specifically, the audio input is fed into Audio Spectrogram Transformer (AST)~\cite{ast}, and the output is then passed to the audio resampler to reduce the number of audio embeddings to a fixed length of $M$ while preserving essential information.
As shown in Figure~\ref{fig:resampler}, the audio resampler comprises $K$ audio resampler blocks, each with multi-head self-attention (MHSA), multi-head cross-attention (MHA), and a feed-forward network (FFN).
We set $K$ as 4 for default. 

MHSA first allows the learnable query embeddings to interact and capture contextual relationships among themselves, refining their initial representations. This is followed by MHA, where the query embeddings attend to the output of AST, extracting audio embeddings with a fixed length of $M$.
The FFN then processes the audio embeddings to refine them.
This sequence of operations enables the audio resampler to reduce the number of audio embeddings efficiently while preserving critical information, facilitating seamless fusion with the frame embeddings in subsequent stages.
\begin{figure}[t!]
    % \vspace{-1mm}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/supp_resampler_v2.pdf}
    \caption{The overall architecture of audio resampler.}
    \label{fig:resampler}
    \vspace{-3mm}
\end{figure}

\bs{The MLP consists of two layers with dimensions $\mathbb{R}^{2D\times D/2}$ and $\mathbb{R}^{D/2 \times 1}$, using a QuickGELU as the non-linearity between them.}

\section{More Quantitative Results}
\label{supp_sec:quan}
\noindent\textbf{Effect of Post-Processing:}
% \bs{About post processing...}
Post-processing techniques have been widely adopted in video-text retrieval to enhance performance by refining similarity scores.
Previous methods~\cite{camoe,ts2,ucofia,uatvr,tefal} adopt the post-processing techniques, including Dual Softmax Loss (DSL)~\cite{camoe}, Querybank Norm (QB-Norm)~\cite{qbnorm}, and the Sinkhorn-Knopp algorithm (SK-Norm), for further improvements in retrieval accuracy.
We also explore the effect of the post-processing technique by adopting DSL that applies inverted softmax~\cite{inverted} during inference.
We report the retrieval performance of AVIGATE with and without post-processing in Table~\ref{tab:supp_postprocessing} compared with existing methods.
Our model, AVIGATE, consistently achieves superior performance across all evaluation metrics for both text-to-video and video-to-text retrieval tasks, outperforming all previous methods by significant margins. 
Specifically, for the CLIP ViT-B/32 backbone, AVIGATE with post-processing achieves R@1 of 53.9\% for text-to-video retrieval.
Furthermore, in video-to-text retrieval, AVIGATE with DSL achieves R@1 of 53.0\%. 
Similarly, for the CLIP ViT-B/16 backbone, AVIGATE achieves substantial gains over existing methods. 
When using post-processing, our method achieves R@1 of 56.3\% for text-to-video retrieval, representing a considerable 2.3\%p improvement over TS2-Net~\cite{ts2}. 
In video-to-text retrieval, AVIGATE also outperforms other methods with R@1 of 57.4\%.

\input{tabs/supp_table_post}
\input{tabs/supp_table_vatex}
\noindent\textbf{Entire Performance on VATEX:}
We present the complete video-text retrieval results on VATEX~\cite{vatex} in Table~\ref{tab:supp_vatex}, including both text-to-video and video-to-text retrieval.
\iffalse
Our method, AVIGATE, is evaluated with two variants of the CLIP ViT backbone (\ie, ViT-B/32 and ViT-B/16).
As shown in Table~\ref{tab:supp_vatex}, AVIGATE achieves notable results in text-to-video retrieval, with R@1 of 63.1\% and 67.5\% for ViT-B/32 and ViT-B/16, respectively. 
In the video-to-text retrieval task, AVIGATE also demonstrates impressive performance, achieving R@1 of 76.6\% and 80.7\% for ViT-B/32 and ViT-B/16, respectively. 
These results highlight the scalability of AVIGATE across different backbone sizes.
% In addition, we demonstrate the effect of post-processing, as detailed in Table~\ref{tab:supp_vatex}.
Furthermore, the use of the post-processing technique, DSL~\cite{camoe}, leads to a significant boost in retrieval accuracy.
% Specifically, RSum increases from 522.0 to 545.2 with ViT-B/32 and from 535.4 to 555.6 with ViT-B/16, indicating a substantial gain in overall retrieval accuracy.
\fi
The results are reported using two variants of the CLIP ViT backbone, CLIP ViT-B/32 and CLIP ViT-B/16.
Moreover, we assess the effect of the post-processing technique, DSL~\cite{camoe}, for further performance boosts.
With the CLIP ViT-B/32 backbone, AVIGATE achieves notable results in text-to-video retrieval, with R@1 of 63.1\% and 76.6\% for text-to-video retrieval and video-to-text retrieval, respectively.
When applying DSL, we observe significant improvements across all metrics.
Specifically, it improves AVIGATE by a large margin, 7.6\%p and 8.7\%p in R@1 for text-to-video retrieval and video-to-text retrieval, respectively.
When employing the larger backbone, CLIP ViT-B/16, our method demonstrates the scalability across different backbone sizes, achieving R@1 of 67.5\% for text-to-video retrieval and 80.7\% for video-to-text retrieval.
Moreover, the use of DSL consistently boosts the retrieval accuracy overall, with 20.2\%p improvements in RSum.


\section{Comparison to Recent Work}
\label{supp_sec:tmass}
\bs{(To be removed?)
T-MASS~\cite{tmass} presents a state-of-the-art performance in video-text retrieval, introducing a stochastic text modeling method.
Although we aimed to conduct a comprehensive evaluation that included comparisons with recent state-of-the-art methods, this was unfortunately not possible due to the unavailability of their official code repository\footnote[1]{\url{https://github.com/Jiamian-Wang/T-MASS-text-video-retrieval}}, which appears to have been removed from GitHub due to technical or unforeseen issues.
Without access to the implementation details or pretrained models, reproducing their results consistently and fairly was not feasible. Considering the critical importance of reproducibility, we opted to exclude T-MASS from our experiments rather than risk an inaccurate and incomplete evaluation.
}
% We appreciate their contributions to the field and would be glad to include such comparisons if the necessary resources become available in the future.


\section{More Ablation Studies}
\label{supp_sec:ablation}
We further conduct ablation studies using varying hyperparameters in AVIGATE.
Similar to the main paper, we report text-to-video retrieval results on the MSR-VTT dataset~\cite{msrvtt} with CLIP ViT-B/32. Table~\ref{tab:supp_ablation_hyp} presents the whole results of the ablation studies.

\noindent \textbf{Layer Depth of Gated Fusion Transformer:}
We present the impact of the number of layers of the gated fusion transformer ($L$) in Table~\ref{tab:supp_ablation_hyp}(a)  and observe that the performance gradually improves up to $L$=4, where the best performance is achieved.

\noindent \textbf{Hyperparameters $\lambda$ and $\delta$ in Eq.~(5):}
We investigate the impact of the scaling factor $\lambda$ and the maximum margin $\delta$ in Eq.~(5) of the manuscript.
It is worth noting that the adaptive margin in Eq.~(5) becomes 0 when $\lambda$ or $\delta$ are set to 0, leading the loss in Eq.~(6) to the conventional contrastive loss.
As shown in Table~\ref{tab:supp_ablation_hyp}(b), when $\lambda$ is set to 0.2, the model yields the best performance. 
Meanwhile, setting $\lambda$ to 0.1 results in a slight decrease in performance, indicating that a smaller scaling factor may not provide sufficient margin adjustment.  
However, increasing $\lambda$ to 0.3 does not lead to further improvements.
Similarly, Table~\ref{tab:supp_ablation_hyp}(c) presents the effect of varying the maximum margin $\delta$. 
We observe that the performance gradually improves up to $\delta = 0.1$.
Increasing $\delta$ beyond 0.1 degrades performance due to excessively large margins pushing negative pairs too far apart.

\noindent \textbf{Gate Mechanism Type:}
Our method employs a soft gate mechanism, which allows for continuous modulation of the contribution of audio during fusion.
To evaluate the effectiveness of the soft gate mechanism, we compare the soft gate with a hard gate mechanism, which assigns a gating score of 1 if it exceeds a predefined threshold and 0 otherwise.
As shown in Table~\ref{tab:supp_ablation_hyp}(d), using the hard gate underperforms our method.
% The performance degradation when using the hard gate is attributed to its binary decision-making.
Unlike using the hard gate mechanism, our method facilitates the effective use of relevant audio cues while minimizing the impact of irrelevant or noisy audio signals; it enables the model to leverage informative audio more precisely, thereby improving retrieval accuracy.

\input{tabs/supp_table_ablation}

\begin{figure*}[t!]
    \vspace{-1mm}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/Supple_Qual.pdf}
    \vspace{-2mm}
    \caption{ Top-1 text-to-video retrieval results of our method on MSR-VTT, where they are true matches.
    The audio provides informative cues for accurate retrieval, where ``a man is talking'' in the query text is not visible (a) and ``talk$\cdots$san diego'' in the query text is not visible but audible (b).
    However, neglecting these informative audio signals (\ie, w/o Audio) fails to retrieve true matches. 
    Meanwhile, The irrelevant audio is filtered by the gated fusion transformer, leading to an accurate retrieval result (c) and (d); without the gating mechanism (\ie, w/o Gate), it leads to retrieving false matches due to the irrelevant audio.    
    }
    \label{fig:supp_qual}
    \vspace{-3.5mm}
\end{figure*}
\section{More Qualitative Results}
\label{supp_sec:qual}
We further present additional qualitative results that illustrate the effectiveness of AVIGATE in leveraging audio information for text-to-video retrieval. 
Figure~\ref{fig:supp_qual} shows the Top-1 retrieved videos from our method, including the corresponding audio signals, to highlight how audio cues influence retrieval outcomes.

In Figure~\ref{fig:supp_qual}(a) and (b), we present a scenario where the audio provides valuable information that enables improving retrieval performance. 
AVIGATE, which incorporates audio through the gated fusion transformer, successfully retrieves the correct video corresponding to the text query. In contrast, the method without audio information (\ie, w/o Audio) fails to retrieve the true matches. This comparison highlights the benefit of utilizing informative audio cues.

Conversely, Figure~\ref{fig:supp_qual}(c) and (d) present another scenario where the audio input contains irrelevant information, such as background noise. AVIGATE effectively filters out the uninformative audio signals through the gating mechanism. The gating function assigns low gating scores, allowing the model to focus only on the visual cues. As a result, AVIGATE successfully retrieves the correct videos. In contrast, the method without the gating function (\ie, w/o Gate) is impacted by the noisy audio and fails to retrieve the true matches.

These qualitative results demonstrate that the gated fusion transformer successfully filters out irrelevant audio while leveraging valuable audio information when the audio contributes positively.

==> Submission_backup_0304/_0_abstract.tex <==
\begin{abstract}
% Video-text retrieval, which involves retrieving videos based on textual queries or vice versa, is of paramount importance for advancing video understanding and multimodal information retrieval. 
% Recent methods predominantly rely on visual and textual features while often disregarding the informative audio modality, which can provide critical semantic context and enhance the overall comprehension of video content. 
% Nonetheless, existing approaches that incorporate audio information tend to inadequately handle noisy or irrelevant audio signals, thereby resulting in suboptimal video representations. 
% To address this issue, we propose a novel framework, \textbfAudio-guided \textbfVIdeo representation learning with \textbfGATEd attention~(\textbfAVIGATE), that effectively leverages audio cues through a gated attention mechanism that selectively filters out uninformative audio signals.
% % To address this issue, we propose a novel framework for video-text retrieval that effectively leverages audio cues through a gated attention mechanism that selectively filters out uninformative audio signals.
% Furthermore, we propose an adaptive margin-based contrastive loss that accounts for intra-modal dissimilarity, facilitating a better video-text alignment.
% Our extensive experiments on public benchmarks demonstrate that the proposed method achieves state-of-the-art performance.
Video-text retrieval, the task of retrieving videos based on a textual query or vice versa, is of paramount importance for video understanding and multimodal information retrieval. 
Recent methods in this area rely primarily on visual and textual features and often ignore audio, although it helps enhance overall comprehension of video content.
Moreover, traditional models that incorporate audio blindly utilize the audio input regardless of whether it is useful or not, resulting in suboptimal video representation. 
To address these limitations, we propose a novel video-text retrieval framework, Audio-guided VIdeo representation learning with GATEd attention (AVIGATE), that effectively leverages audio cues through a gated attention mechanism that selectively filters out uninformative audio signals.
In addition, we propose an adaptive margin-based contrastive loss to deal with the inherently unclear positive-negative relationship between video and text, which facilitates learning better video-text alignment.
Our extensive experiments demonstrate that AVIGATE achieves state-of-the-art performance on all the public benchmarks.
\end{abstract}

\iffalse
TL;DR
Our paper proposes a new framework for video-text retrieval, AVIGATE, using a gated fusion for video and audio, and an adaptive margin-based contrastive loss.
\fi

==> Submission_backup_0304/_1_introduction.tex <==
\section{Introduction}
\label{sec:intro}
% -----------%
% - Motivation & Challenges
%     - 기존의 VTR methods들은 괄목할만한 improvement를 보여왔지만, video 내에 들어 있는 정보인 audio 정보를 무시함. 하지만 video 내엔 ‘invisible’ 하지만 ‘audible’ 한 정보들이 있고 이는 text-video retrieval을 하는데 중요한 clue가 될 수 있음. 이를 모두 활용해서 video를 표현한다면 더 나은 video representation을 얻을 수 있음.
%         - 모든 audio가 항상 video representation을 강화 하는 것은 아님. such as noisy background sound.
%     - Audio 정보를 활용하는 사전 연구도 있지만, 이는 audible 정보와 visible 정보를 각각 text와의 cross-attention networks 통해 explicit 하게 text와의 relations을 각각 추론하는데, 이는 large computational burden을 요구함. 덧붙여 global text-video alignment 만을 수행하기 때문에 fine-detail을 잡기 어려움.
%     - 대부분의 recent work은 loss function에 대해 무시하고 있으나, 이는 더 큰 성능 향상을 기대할 수 있는 여지가 있음.
% - Our method
%     - Audio-guided video representation을 얻기 위한 새로운 framework 제안.
%         - 이 framework은 audio-visual modalities들을 효과적으로 bridging and fusion하여 video representation을 얻음.
%         - 먼저, audio와 visual frame을 위한 pre-trained audio encoder와 vision encoder가 각각 있고, audio encoder는 dense-sampled audio를 encoding 하고, vision encoder는 sparse-sampled frame을 encoding 한다.
%         - 이러한 dense audio embedding을 direct하게 sparse frame embedding과 fusion하게 되면 풍부하고 informative 한 dense information이 훼손될 수 있음. 이를 방지하고자 fixed number의 embedding을 resampling 함.
%         - Cross-attention mechanism을 통해 resampled audio embedding과 frame embedding을 fusion 하게 되는데, 모든 audio가 informative 하진 않을 수도 있으니 (e.g., noise) 이에 대해 fusion 결과를 얼만큼 반영할 지에 대한 score를 바탕으로 gating 해준다.
%     - Global-Local video-text alignment
%         - 상보적인 역할을 할 수 있는 fused 된 video embedding을 바탕으로 fine-detail을 capture할 수 있는 local video-text alignment과, global context를 capture할 수 있는 global video-text alignment을 통해 matching capability를 강화 함.
%     - Adaptive Margin-based Contrastive loss
%         - 대부분의 previous work은 conventional한 contrastive loss만을 사용 해왔다. 이는 비슷한 context를 담고 있는 negative pair를 embedding space 상에서 강제로 멀게하여 poor generalization capability를 갖게 할 수도 있다.
%         - 이를 방지하고자 adaptive margin-based contrastive loss를 제안하며, 이 때 margin은 negative pair간의 relevance를 고려하여 계산된다.
% - Contribution
%     - An effective audio-video fusion module for Text-Video retrieval
%     - A new loss function for boosting the performance
%     - We achieve the state of the art performance
% -----------%

Video-text retrieval, the task of finding videos relevant to text query or vice versa, has gained significant interest due to its diverse applications in video understanding and multi-modal information retrieval. 
% It leverages a joint latent space to facilitate effective cross-modal alignment by aligning textual descriptions with corresponding video content.
\begin{figure}[t!]
    % \vspace{-1mm}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/teaser_v8.pdf}
    %\caption{Comparative illustration of different scenarios using visual-only, audio-video fusion, and our proposed gated fusion approach. (a) In cases where the audio signal provides valuable information (\eg, the sound of people singing), the audio-video fusion and our gated fusion achieve high similarity scores. (b) When the audio signal is misleading (\eg, background noise), traditional fusion methods degrade performance. In contrast, our gated fusion mechanism successfully filters irrelevant audio cues, maintaining a high similarity score like the visual-only case.}\
    \vspace{-2mm}
    \caption{Comparative illustration of different scenarios using visual-only, audio-video fusion, and our proposed gated fusion approach. (a) In cases where the audio signal provides valuable information, the audio-video fusion and our gated fusion achieve high similarity scores. (b) When the audio signal is misleading, traditional fusion methods degrade performance. In contrast, our gated fusion mechanism successfully filters irrelevant audio cues, maintaining a high similarity score like the visual-only case.}
    \label{fig: teaser}
    \vspace{-3mm}
\end{figure}
Most existing methods in this field have primarily focused on leveraging visual information from videos and textual information from accompanying metadata or captions~\cite{clip4clip,clip2video,camoe,xclip,xpool,ts2,uatvr,prost,ucofia}. 
While these methods have greatly advanced video-text retrieval, they still have a significant limitation: they neglect audio information of video that conveys `\textit{invisible but audible}' cues providing essential context such as speaker identity, background noises, or emotional nuances, which are crucial for a comprehensive understanding of video.
% Existing approaches fail to fully exploit the multi-modal nature of videos, leading to suboptimal retrieval performance.
Leveraging the audio information in video representation learning has potential to substantially improve retrieval performance by offering a richer multi-modal representation of video, as shown in Figure~\ref{fig: teaser}(a).

Nevertheless, only a few recent studies~\cite{eclipse,tefal} have explored the use of audio information in video-text retrieval tasks. ECLIPSE~\cite{eclipse} employs a cross-modal attention mechanism to fuse audio and visual modalities, creating a unified representation. TEFAL~\cite{tefal}, on the other hand, proposes text-conditioned feature alignment based on the cross-attention mechanism for audio and textual modalities as well as for visual and textual modalities.
These methods commonly assume that audio contributes positively to enhancing the video representation, but this is not always the case.
% However, not all videos contain audio that contributes positively to enhancing their representation. 
% In particular, background noise can be detrimental and may degrade the representation rather than improve it. 
When irrelevant audio is processed jointly with visual information~(\eg, irrelevant background music and noise), it could impair the video representation and negatively affect cross-modal alignment, as shown in Figure~\ref{fig: teaser}(b). 
% This degradation may ultimately hinder successful video-text retrieval by negatively affecting the overall cross-modal alignment.
ECLIPSE and TEFAL do not address this issue and blindly exploit the audio modality.
% TEFAL~\cite{tefal} has mitigated this issue by extracting text-conditioned representation of visual frame and audio separately.
Moreover, TEFAL introduces substantial computational demands on retrieval systems since both the video (also audio) and text description must be processed together to generate the representation of both video frame and audio, necessitating reprocessing of the entire database each time a new query is received.


% To address these issues, we introduce a new framework that dynamically determines whether the audio inputs are important, where the text encoder is separated from the audio encoder and visual encoder; its overall architecture is illustrated in Figure~\ref{fig: arch}.
To address these issues, we introduce a novel framework, \textbf{A}udio-guided \textbf{VI}deo representation learning with \textbf{GATE}d attention~(\textbf{AVIGATE}), that dynamically determines whether audio input is useful and enables efficient retrieval by processing video (including audio) and text description independently; its overall architecture is illustrated in Figure~\ref{fig: arch}.
% The proposed framework 
AVIGATE is built on three encoders for each modality: Audio Spectrogram Transformer (AST)~\cite{ast} for the audio input and two CLIP encoders~\cite{clip}, one for visual input and the other for textual input.
The model begins by encoding audio using AST to produce dense audio embeddings. 
These embeddings are then processed by an audio resampler to preserve rich audio information while reducing redundancy by resampling to a fixed number of embeddings. 
Video is represented by frame embeddings given by the CLIP image encoder, while the text is encoded by the CLIP text encoder. 

Audio and frame embeddings are then fused by a gated fusion transformer. \iffalse, which consists of a gated fusion block and a gating function. 
The gated fusion block produces the fused audio-visual embeddings by a cross-attention mechanism to capture complementary information between the two modalities. 
The gating function predicts gating scores given audio and frame embeddings and thus selectively filters out the fused embeddings to mitigate the effect of noisy signals while maintaining the frame embeddings.
\fi
This module integrates audio and frame embeddings by employing an adaptive gating function that regulates the influence of each modality. 
To be specific, the gate function dynamically determines the contribution of audio embeddings, allowing the transformer to leverage complementary audio information when relevant while maintaining the frame embeddings by minimizing the effect of potentially noisy audio.
\iffalse
The output of the gated fusion transformer, \ie, the final video representation, is aligned with the text embedding with a global-local alignment scheme~\cite{xclip,prost,ucofia,uatvr} that combines both global alignment between the entire video and the text, and local alignment between each video frame and the text.
This alignment scheme enables capturing both the overall semantic context and fine details, leading to more accurate retrieval.


In addition, we propose an adaptive margin-based contrastive loss that extends the traditional contrastive loss by incorporating an adaptive margin term for each negative pair. 
The margin is determined based on the intra-modal dissimilarity within both the textual and visual modalities, allowing for implicit exploration of the semantic relationship of the negative pair. 
Meanwhile, conventional contrastive loss, \ie, InfoNCE~\cite{Sohn_nips2016,oord2018representation}, treats all negative pairs equally, ignoring the semantic relationships between them. 
It may lead to suboptimal representations, especially when negative pairs vary significantly in their semantic similarities. 
We address this limitation thanks to the adaptive margins between the negative pairs according to their semantic dissimilarities.
As a consequence, the proposed loss function leads to a better video-text alignment.
\fi
The output of the gated fusion transformer, \ie, the final video representation, is then aligned with the text embedding.

To improve the discriminative capability of video-text alignment, we propose an adaptive margin-based contrastive learning approach that extends the traditional contrastive loss~\cite{Sohn_nips2016,oord2018representation} by incorporating an additional margin for each negative pair.
The margin is determined based on the intra-modal dissimilarity within both the textual and visual modalities, allowing for implicit exploration of inherent relationships among semantically similar pairs.
The input similarity score between the video representation and the text embedding used in the proposed loss is computed through a multi-grained alignment scheme~\cite{xclip,prost,ucofia,uatvr} that enables capturing both the overall semantic context and fine details.
Consequently, the proposed loss with the multi-grained alignment scheme encourages learning a more discriminative and generalizable cross-modal embedding space, leading to a better video-text alignment. 

Our method was evaluated and compared with prior work on two public benchmarks~\cite{msrvtt,vatex} where it outperformed all existing methods while enabling an efficient retrieval.
The main contribution of this paper is three-fold:
\begin{itemize}[leftmargin=*, topsep=1mm]
\item We propose AVIGATE, an effective audio-video fusion framework that fuses audio and visual information while dynamically determining whether the audio is valuable. 
\iffalse with a gated attention mechanism that determines whether the audio signal is valuable. \fi  
\item We propose a new adaptive margin-based contrastive loss, considering inherent relationships between semantically similar pairs so that the cross-modal embedding space becomes more discriminative and better generalizes. 
\item  Our method achieves the best performance on two public benchmarks for video-text retrieval and ensures a high retrieval efficiency during testing.
\end{itemize}


==> Submission_backup_0304/_2_relatedwork.tex <==
\section{Related Work}
\subsection{Video-Text Retrieval}
Video-text retrieval is a fundamental topic in the vision-language domain aimed at retrieving the most semantically relevant video for a given text query.
Early work in this field primarily employed dense fusion mechanisms for cross-modal alignment, aiming to tightly integrate features across modalities~\cite{ctsan, jsf}.
However, with the introduction of large-scale text-video datasets, more recent approaches have shifted toward end-to-end pre-training strategies that allow models to learn video and text features jointly.

To further these advancements, notable methods such as ClipBERT~\cite{clipbert} and Frozen~\cite{frozen} have proposed efficient training techniques like sparse sampling and curriculum learning, enhancing the feasibility of handling large datasets.
Additionally, recent methods have leveraged models pre-trained on massive image-text pairs, such as CLIP~\cite{clip}, to benefit from their robust visual-textual alignment capabilities.
CLIP4Clip~\cite{clip4clip} applies frame-level alignment within CLIP’s pre-trained feature space to significantly improve video retrieval performance.

Expanding on CLIP4Clip, recent studies emphasize achieving precise alignment between visual and textual modalities.
X-Pool~\cite{xpool} calculates cross-attention weights between text and video frames to extract text-conditioned video representations, where the video encoding process must involve both modal data, introducing significant computational costs.
% Prompt Switch~\cite{pswitch} introduced a learnable prompt cube for spatial-temporal feature adaptation and a prompt-switching mechanism to capture temporal information efficiently.
Meanwhile, a series of studies~\cite{xclip,ucofia,uatvr,prost} have explored and exploited a multi-grained alignment scheme to achieve more accurate retrieval.  
UCOFiA~\cite{ucofia} employs a hierarchical alignment strategy across patch-word, frame-sentence, and video-sentence levels.
UATVR~\cite{uatvr} that begins with token-wise word-frame matching addresses semantic uncertainty in video-text pairs by introducing a distribution matching method that models modality-specific distributions, enabling more robust and adaptive matching.
% To achieve more accurate retrieval, the above methods have proposed spatial-temporal alignment or cross-attention between text queries and video frame features to extract text-conditioned video representations.
% However, such methods often incur high computational costs that hinder retrieval system efficiency.
% Building on the principles of CLIP4Clip, we propose a framework that pursues an efficient retrieval system through frame-level alignment while delivering accurate retrieval outcomes.
Following this spirit, our method, built on the principles of CLIP4Clip, also exploits a multi-grained alignment scheme in a na\"ive way. 
\subsection{Audio-Enhanced Video-Text Retrieval}
Although video-text retrieval has advanced significantly, there remains room for improvement by incorporating audio, readily available yet often overlooked in video content.
An early study by Liu \etal,~\cite{collaboexperts} uses audio information for video-text retrieval by integrating the pre-trained representation of audio experts with that of other modalities.

More recent studies have focused on learning representations that fuse audio with other modalities.
ECLIPSE~\cite{eclipse} introduces a fusion method using cross-attention between audio and video to generate audio-guided video representations.
On the other hand, TEFAL~\cite{tefal} applies cross-attention between text and audio, as well as between text and video, to produce text-guided audio and video representations.
% However, extracting text-guided representations for both audio and visual modalities leads to computational overhead, hindering retrieval system efficiency.
This process requires a large burden of computational costs, hindering efficient retrieval.

Furthermore, the prior fusion methods have limitations, as they fail to handle irrelevant audio, like background noises, which can degrade video representations and hinder cross-modal alignment.
To tackle these issues, we present a new fusion method that dynamically assesses the relevance of audio input and enables an efficient retrieval system by independently processing video and text descriptions.
\label{sec:relate}


==> Submission_backup_0304/_3_method.tex <==

\section{Proposed Method}
\label{sec:method}

\begin{figure*}[t!]
    \centering
    \vspace{-1mm}
    \includegraphics[width=0.99\linewidth]{figs/arch_v8.pdf}
    \vspace{-2mm}
    \caption{($Left$) The overall architecture of AVIGATE. Audio input is processed through an Audio Spectrogram Transformer (AST) and further refined by an audio resampler to generate fixed-size audio embeddings. Frame embeddings are derived from the video using a CLIP Image Encoder, while the text embedding is extracted by the CLIP Text Encoder. These audio and frame embeddings are fused by a gated fusion transformer, which dynamically determines the contribution of audio. 
    The final video representation is aligned with the text embedding using a multi-grained alignment scheme, facilitating an effective video-text retrieval process.
    ($Right$) The gated fusion transformer consists of a gated fusion block and a gating function.
    }
    \label{fig: arch}
    \vspace{-2.5mm}
\end{figure*}
\iffalse
In this section, we describe our novel framework, AVIGATE.
Firstly, we present embedding extraction for each modality with its encoder~(\cref{sec:extraction}). 
Then, the gated fusion transformer is introduced~(\cref{sec:gate}). 
Lastly, we describe the adaptive margin-based contrastive learning strategy~(\cref{sec:margin_loss}).
The overall architecture of our framework is depicted in Figure~\ref{fig: arch}.
\fi
This section presents details of our video-text retrieval framework, dubbed AVIGATE; its overall architecture is depicted in Figure~\ref{fig: arch}. 
We first describe the embedding extraction process for each modality in ~\cref{sec:extraction}, and then elaborate on the gated fusion transformer in~\cref{sec:gate}. 
Finally, the adaptive margin-based contrastive learning strategy is introduced in~\cref{sec:margin_loss}.
\subsection{Embedding Extraction}
\label{sec:extraction}

AVIGATE utilizes three pre-trained encoders to process each modality: Two CLIP encoders~\cite{clip} for the video frames and the text descriptions, respectively, and Audio Spectrogram Transformer (AST)~\cite{ast} for the audio signals.

\noindent\textbf{Frame Embeddings:} We utilize the pre-trained CLIP image encoder~\cite{clip} to extract the frame embeddings of each video.
Given an input video $V$, $N$ frames are first uniformly sampled denoted as $V=[F^1, F^2, \dots, F^N]$. 
Each frame is divided into non-overlapping patches, which are then transformed using a linear projection. 
A [\texttt{CLS}] token is prepended to this sequence of patches, and the combined sequence is fed to the CLIP image encoder. 
The output corresponding to the [\texttt{CLS}] token is taken as the frame embedding.
Finally, these frame embeddings are concatenated to form a sequence of frame embeddings, $\mathbf{f}=[\mathbf{f}^1, \mathbf{f}^2, \dots, \mathbf{f}^N]\in\mathbb{R}^{N\times D}$, where $D$ denotes the dimension of the embeddings. 

\noindent\textbf{Text Embeddings:} The text embedding extraction is carried out by the CLIP text encoder~\cite{clip}, as in the frame embedding extraction. 
Given a text input $T$, all words in the text are tokenized and enclosed with special tokens [\texttt{SOS}] and [\texttt{EOS}], indicating the start and the end of the sentence, respectively. 
This complete sequence is then passed through the CLIP text encoder.
Then, the output corresponding to the [\texttt{EOS}] token is regarded as the text embedding, $\mathbf{t} \in \mathbb{R}^{D}$, capturing the overall semantics of the input text.


\noindent\textbf{Audio Embeddings:} We employ AST~\cite{ast} as our audio encoder following prior work~\cite{ast, tefal}. The audio input $A$ from the video $V$ is first converted into a Mel-spectrogram, capturing key audio features across time and frequency. 
AST processes this spectrogram as a sequence of $N_a$ patches, using transformer layers to generate a detailed set of audio embeddings.
However, since audio signals are much more densely sampled compared to video frames, directly fusing all $N_a$ audio embeddings with frame embeddings would be computationally expensive. 
To address this, we employ an additional query-based transformer~(\ie, audio resampler)~\cite{perceiver, detr, flamingo} that uses a cross-attention mechanism with $M$ learnable query embeddings. 
This design reduces the number of audio embeddings to a fixed length of $M$, $\mathbf{a}=[\mathbf{a}^1, \mathbf{a}^2, \dots, \mathbf{a}^{M}] \in \mathbb{R}^{M \times D}$, maintaining essential audio information while significantly lowering computational load for subsequent fusion with visual modalities. We freeze the pretrained AST parameters during training, avoiding the high computational cost of fine-tuning. Architectural details are provided in the supplementary material.

\subsection{Gated Fusion Transformer}
\label{sec:gate}


To effectively fuse the audio embeddings $\mathbf{a}$ and frame embedding $\mathbf{f}$, the gated fusion transformer is designed to dynamically adjust the contribution of audio based on its relevance to the video. This transformer achieves adaptive fusion by using gating scores that modulate the impact of audio features on the video representation, ensuring that irrelevant audio signals have a reduced influence, thus preserving the integrity of the visual content.

The gated fusion transformer consists of $L$ layers, each containing a gated fusion block that applies gating scores to control the fusion process. Within each block, Multi-Head Attention (MHA) and a Feed-Forward Network (FFN) blend the audio and frame embeddings, with the adaptive gating function providing scores ($g_{\textrm{mha}}$ and $g_{\textrm{ffn}}$) to regulate their influence. These gating scores control the contribution of audio embeddings, enabling the transformer to integrate complementary audio cues when relevant while minimizing the effect of potentially noisy audio. This is followed by Multi-Head Self-Attention (MHSA) and a Feed-Forward Network (FFN) to refine the representation.

When the gating scores are high, audio cues are emphasized, enhancing the representation by capturing complementary audio details. Conversely, low gating scores prioritize the robustness of the visual content against irrelevant audio interference. This selective fusion leads to a more context-sensitive and discriminative video representation, which improves video-text retrieval performance. In the following, we provide architectural details of the two core components of the gated fusion transformer: the gated fusion block and the gating function.

\subsubsection{Gated Fusion Block}
\label{sec:fusion}
The gated fusion block takes the audio embeddings $\mathbf{a}$ and the frame embeddings $\mathbf{f}$ as inputs and outputs video representation through the fusion process followed by the refining process.
Specifically, with a series of $L$ layers, the frame embeddings $\mathbf{f}$ evolve into refined $\mathbf{f}^{(L)}$ by capturing cross-modal interactions with the audio embeddings $\mathbf{a}$, where $\mathbf{f}$ directly from the CLIP image encoder is regarded as initial input $\mathbf{f}^{(0)}$.
The refined $\mathbf{f}^{(L)}$ serves as the final video representation $\mathbf{v}=[\mathbf{v}^1, \mathbf{v}^2, \dots, \mathbf{v}^N]\in\mathbb{R}^{N\times D}$.



In the fusion process, $\mathbf{f}^{(l-1)}$ is fused with $\mathbf{a}$ by MHA with a residual connection.
The output is modulated by a gating score $g_{\textrm{mha}}$ generated by the gating function~(\cref{sec:gating_function}) to determine the contribution of the audio embedding in the fusion.
Then, the output is fed into an FFN with a residual connection, which is also modulated by a gating score $g_{\textrm{ffn}}$, ensuring selective enhancement based on the gating mechanism.
The fusion process is formulated as follows:
\begin{equation}
    \begin{aligned}
    \mathbf{z}^{(l)} &=  g_{\textrm{mha}}^{(l)} \cdot \textrm{MHA}(\textrm{LN}(\mathbf{f}^{(l-1)}), \textrm{LN}(\mathbf{a})) +\mathbf{f}^{(l-1)} , \\
    \bar{\mathbf{z}}^{(l)} &= g_{\textrm{ffn}}^{(l)} \cdot \textrm{FFN}_1(\textrm{LN}(\mathbf{z}^{(l)})) + \mathbf{z}^{(l)},
    \label{eq:fusion_process}
    \end{aligned}
\end{equation}
where LN denotes the layer normalization.
MHA involves $n$-head attention operations; it is formulated by
\begin{equation}
\begin{aligned}
    \textrm{MHA}(\mathbf{X},\mathbf{Y}) &= [\textrm{Attn}^1(\mathbf{X},\mathbf{Y}), ..., \textrm{Attn}^n(\mathbf{X},\mathbf{Y})]\mathbf{W}_o,\\ 
    \textrm{Attn}^i(\mathbf{X},\mathbf{Y}) &= \text{softmax}\left( \frac{(\mathbf{X}\mathbf{W}_{q}^{i}) (\mathbf{Y}\mathbf{W}_k^{i})^\top}{\sqrt{D_h}} \right) (\mathbf{Y}\mathbf{W}_v^{i})
    \label{eq:MHA}
\end{aligned}
\end{equation}
where $[\cdot,\cdot]$ denotes concatenation, and $D_h$ is set to $D/n$. 
$\mathbf{W}_{q}^{i}, \mathbf{W}_{k}^{i}, \mathbf{W}_{v}^{i}\in\mathbb{R}^{D\times D_h}$ and $\mathbf{W}_{o}\in\mathbb{R}^{D\times D}$ are linear projection matrices.

The fused representation $\bar{\mathbf{z}}^{(l)}$ undergoes the refining process to enhance the overall video representation.
Specifically, $\bar{\mathbf{z}}^{(l)}$ is fed into a Multi-Head Self-Attention (MHSA) module with a residual connection.
Then, the second FFN with a residual connection is applied to the output of MHSA to produce the refined frame embeddings $\mathbf{f}^{(l)}$. 
The refining process is formulated as follows:
\begin{equation}
\begin{aligned}
    \Tilde{\mathbf{z}}^{(l)} &= \textrm{MHSA}(\textrm{LN}(\bar{\mathbf{z}}^{(l)})) + \bar{\mathbf{z}}^{(l)} , \\
    \mathbf{f}^{(l)} &= \textrm{FFN}_2(\textrm{LN}(\Tilde{\mathbf{z}}^{(l)})) + \Tilde{\mathbf{z}}^{(l)}.
    \label{eq:refining_process}
\end{aligned}
\end{equation}
Similar to MHA, MHSA involves $n$-head self-attention operations, where $\textrm{MHSA}(\textrm{X})=\textrm{MHSA}(\textrm{X},\textrm{X})$.% in~\cref{eq:MHA}.



\subsubsection{Gating Function}
\label{sec:gating_function}
The gating function, $G(\mathbf{a}, \mathbf{f}^{(l-1)})$ at each layer $l$ produces two gating scores, $g_\text{mha}^{(l)}$ and $g_\text{ffn}^{(l)}$, that modulate the outputs of MHA and FFN$_1$ in the gated fusion block, respectively. 
To this end, the audio embeddings $\mathbf{a}$ and the frame embeddings $\mathbf{f}^{(l-1)}$ are first aggregated using average pooling, resulting in $\bar{\mathbf{a}} \in \mathbb{R}^D$ and $\bar{\mathbf{f}}^{(l-1)} \in \mathbb{R}^D$, respectively. 
These aggregated embeddings are then concatenated to form a joint representation, $\mathbf{u}^{(l)} = [\bar{\mathbf{a}}; \bar{\mathbf{f}}^{(l-1)}] \in \mathbb{R}^{2D}$.
The joint embedding $\mathbf{u}^{(l)}$ is passed through two distinct Multi-Layer Perceptrons (MLPs) followed by a non-linear function to compute the gating scores for the outputs of MHA and FFN$_1$. 
The gating function, $G(\mathbf{a}, \mathbf{f}^{(l-1)})$ is formulated as follows:
\begin{equation}
\begin{aligned}
    [g_{\text{mha}}^{(l)},\ g_{\text{ffn}}^{(l)}] &= G(\mathbf{a}, \mathbf{f}^{(l-1)}) \\
    &=\sigma\Big[\left( \textrm{MLP}_{\textrm{mha}}(\mathbf{u}^{(l-1)})\right), \left( \textrm{MLP}_{\textrm{ffn}}(\mathbf{u}^{(l-1)})\right)\Big],
\label{eq:gates}    
\end{aligned}
\end{equation} 
where $\sigma$ is a non-linear function (\ie, tanh).


\subsection{Adaptive Margin-based Contrastive Learning}
\label{sec:margin_loss}

The output of the gated fusion transformer, video representation $\mathbf{v} \in \mathbb{R}^{N \times D}$, is aligned with text embedding $\mathbf{t} \in \mathbb{R}^{D}$. 
This video-text alignment has been, in general, achieved by the cross-modal contrastive learning~\cite{clip,clip4clip,xpool,xclip}, which maximizes similarity scores (e.g., cosine similarity) of positive pairs and minimizes the those of negative pairs.
\iffalse
To further enhance discriminative ability in contrastive learning, we introduce an additional margin between a pair of negative data. 
The concept of margins has been widely explored in prior works on metric learning~\cite{kim2020proxy,deng2019arcface, kim2024efficient}, showing their effectiveness in enforcing clear separation between a negative pair.
\iffalse
% However, applying a fixed margin across all negative pairs presents an issue.
% A fixed margin may excessively push apart negative pairs that still share some level of semantic similarity. This rigid margin risks creating overly strict separations, potentially leading to poor generalization by disregarding inherent relationships among semantically similar pairs. 
To address this limitation,\fi
% However, a fixed margin may not account for varying degrees of semantic similarity among negative pairs.

Motivated by this, we propose an adaptive margin-based contrastive loss that dynamically adjusts margins for each negative pair, informed by their intra-modal semantic similarities. 
\fi

To further enhance the discriminative ability of contrastive learning, we introduce an adaptive margin-based contrastive loss that dynamically adjusts margins for each negative pair based on their intra-modal semantic similarities. The key idea of our method is that semantic relationships within each visual and textual modality provide implicit cues for determining appropriate margins. For instance, if two videos are visually similar or if two texts have high textual similarity, their cross-modal counterparts are also likely to have some level of semantic relatedness. 
In contrast to fixed-margin contrastive loss~\cite{kim2020proxy,deng2019arcface, kim2024efficient}, which applies the same margin to all negative pairs, our method accounts for varying degrees of semantic similarity between negative pairs. This adaptability enables the model to learn discriminative features while maintaining strong generalization by considering the inherent relationships between semantically similar pairs.

\iffalse
The core insight behind our method is that semantic relationships within each visual and textual modality provide implicit cues that can be leveraged for richer supervision. 
For instance, if two videos are visually similar or if two texts have high textual similarity, their cross-modal counterparts are also likely to have some level of semantic relatedness. 
\fi


Following this nature, given a batch with $B$ video-text pairs $\mathcal{B} =\big\{(V_i,T_i)\big\}_{i=1}^{B}$, we define the adaptive margin $m_{ij}$ for each negative pair ($V_i$,$T_j$) according to the average of their intra-modal similarities in both the visual and textual modalities. 
First of all, the frame embedding $\mathbf{f}_i$ is average pooled to obtain holistic embedding of the visual modality denoted by $\bar{\mathbf{f}_i}$.
Let $c_{ij}^{v}$ denotes the cosine similarity between $\bar{\mathbf{f}_i}$ and $\bar{\mathbf{f}_j}$, and $c_{ij}^{t}$ denotes the cosine similarity between $\mathbf{t}_i$ and $\mathbf{t}_j$. The adaptive margin is obtained by:
\begin{equation}
    m_{ij} = \min\left(\lambda \left( 1 - \frac{c_{ij}^{v} + c_{ij}^{t}}{2} \right),\ \delta \right),
    \label{eq:margin}
\end{equation}
where $\lambda$ is a scaling factor, and $\delta$ is the maximum margin to prevent excessively large margins. The operation $\min(\cdot,\cdot)$ ensures that the margin does not exceed $\delta$.
The adaptive margin $m_{ij}$ is then added to the similarity score of the negative pair in the contrastive loss function as follows:
\begin{equation}
\begin{aligned}
    \mathcal{L}(\mathcal{B}) = &-\sum_{i=1}^{B}\Bigg(\log\frac{e^{s_{ii}/\tau }}{e^{s_{ii}/\tau}+\sum_{j=1, j\neq i}^{B}e^{(s_{ij}+m_{ij})/\tau }} \Bigg) \\
    &-\sum_{i=1}^{B}\Bigg(\log\frac{e^{s_{ii}/\tau }}{e^{s_{ii}/\tau}+\sum_{j=1, j\neq i}^{B}e^{(s_{ji}+m_{ji})/\tau }} \Bigg).
    \label{eq:Margin_loss}
\end{aligned}
\end{equation}
By incorporating the adaptive margin into the contrastive loss, our method promotes a more discriminative and generalizable cross-modal embedding space that considers inherent intra-modality relationships, which leads to improved retrieval performance.
\input{tabs/table1}

To compute a similarity score, rather than simply leveraging cosine similarity, we employ an enhanced method that captures both global and local relationships between video and text representations. This combination captures complementary information, enhancing the retrieval performance as observed in the previous arts~\cite{xclip,ucofia,uatvr,prost}. 
First, for global alignment, we derive a comprehensive video representation by applying average pooling to the final video embedding, $\mathbf{v}=[\mathbf{v}^1, \mathbf{v}^2, \dots, \mathbf{v}^N]\in\mathbb{R}^{N\times D}$, where $N$ represents the number of frame segments. This pooled representation,  $\mathbf{v}_g = \sum_{i=1}^{N} \mathbf{v}^i / N \in \mathbb{R}^{D}$, captures the overall content of the video. The video-text similarity score $s_g$ between the global representation of the video $\mathbf{v}_g$ and the text embedding $\mathbf{t} \in \mathbb{R}^{D}$ is then computed as:
\begin{equation}
    s_g = \frac{\mathbf{v}_g^\top \mathbf{t}}{|| \mathbf{v}_g ||_2 || \mathbf{t} ||_2}.
\end{equation}
Next, for local alignment, we match each frame segment embedding $\mathbf{v}^i \in \mathbb{R}^{D}$ with the text embedding $\mathbf{t}$, computing frame-text similarities $s^i = \frac{\mathbf{v}^{i\top} \mathbf{t}}{|| \mathbf{v}^i ||_2 || \mathbf{t} ||_2}$. These frame-text similarities are aggregated using the log-sum-exp (LSE) function:
\begin{equation}
    s_l = \underset{{i\in[1,N]}}{\text{LSE}}(s^i) = \log\left( \sum_{i=1}^{N} e^{\alpha s^i} \right),
    \label{eq:local_alignment}
\end{equation}
where $\alpha$ is a scaling parameter that controls the smoothness of the maximum operation.
The final similarity score $s$, which combines both global and local perspectives, is calculated by averaging $s_g$ and $s_l$:
\begin{equation}
    s = \frac{s_g + s_l}{2}. 
    \label{eq:final_score}
\end{equation}
The final similarity score $s$ is utilized for the adaptive margin-based contrastive loss in~\cref{eq:Margin_loss}.
This multi-grained alignment scheme enables the model to capture both holistic and fine-grained details, thereby enhancing video-text retrieval accuracy.


==> Submission_backup_0304/_4_experiments.tex <==
%\input{tabs/table1.tex}



\section{Experiments}
\label{sec:experiments}
In this section, we present a comprehensive evaluation of the proposed framework, \textit{AVIGATE}. 
We first describe the experimental setup, including the datasets, evaluation metric, and implementation details in~\cref{sec:setup}. 
We then provide quantitative results to show the effectiveness of AVIGATE compared to state-of-the-art methods in~\cref{sec:quan}. 
Next, we include the qualitative results of AVIGATE in~\cref{sec:qual}. 
Moreover, we conduct ablation studies to analyze the impact of components of AVIGATE in~\cref{sec:ablation}.
Lastly, we demonstrate the efficiency of AVIGATE compared to previous arts by analyzing the computational costs in~\cref{sec:complexity}.
\subsection{Experimental Setup}
\label{sec:setup}
\noindent\textbf{Datasets:}
% Audio 있는 dataset만 사용
On two public benchmarks, MSR-VTT~\cite{msrvtt} and VATEX~\cite{vatex}, we evaluate and compare the performance of our method against previous methods.
MSR-VTT, the most common dataset for video-text retrieval, contains 10,000 videos collected from the web, including audio signals. Each video is 10 to 32 seconds long and has 20 corresponding text descriptions. Following the data split from~\cite{mmt,clip4clip}, we train AVIGATE on 9,000 videos (180,000 video-text pairs) and evaluate it on 1,000 selected video-text pairs. Out of the 10,000 videos, 9,582 have audio, which we utilize in our method.
VATEX contains 34,991 videos with multiple text descriptions for each video.  We follow the split protocol of~\cite{hgr} with 25,991 videos for training, 1,500 videos for validation, and 1,500 for testing, respectively.

\noindent \textbf{Evaluation Metric:} 
We employ the standard metric of recall at $K$ (R@$K$, with $K$ = 1, 5, 10) to evaluate retrieval performance for both text-to-video and video-to-text retrieval tasks. In both cases, samples are ranked based on their similarities to the query (in~\cref{eq:final_score}). 
We also report the RSUM, which is the sum of all R@$K$ metrics.
Retrieval is considered successful if at least one relevant item appears within the Top-K positions.


\begin{figure*}[t!]
    \vspace{-1mm}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/Qual_v2.pdf}
    \vspace{-3.5mm}
    \caption{ Top-1 text-to-video retrieval results of our method on MSR-VTT, where they are true matches. 
    $g_{mha}^{(l)}$ and $g_{ffn}^{(l)}$ denote the gating scores for $l$-th layers of the gated fusion transformer. 
    The audio provides informative cues for accurate retrieval, where ``a man is talking'' in the query text is not visible (a). The irrelevant audio is filtered by the gated fusion transformer, leading to an accurate retrieval result (b).   
    }
    \label{fig: qual}
    \vspace{-4.5mm}
\end{figure*}

\noindent\textbf{Implementation Details:}
%audio 없는 instance는 zero input 들어가는거 꼭 넣어주기
We adopt the pre-trained CLIP models from OpenAI~\cite{clip} with two different sizes of image encoder, \ie, ViT-B/32 and ViT-B/16. Moreover, we adopt AST pre-trained on ImageNet~\cite{imagenet} and AudioSet~\cite{audioset} with DeiT~\cite{DeiT} backbone.
Note that we set the audio input as zero vector for the videos that do not include audio signals. 
The dimension $D$ of audio, frame, and text embeddings is set to 512. Our model is optimized using the Adam optimizer~\cite{Adamsolver} for five epochs with a batch size of 128 for all experiments.
The initial learning rate is set to $\expnum{1}{7}$ for the CLIP encoders and $\expnum{1}{4}$ for other modules, using a cosine warm-up strategy~\cite{warmup}, while AST is frozen. 
Following~\cite{clip4clip}, the number of frames $N$ is set to 12, and the max length of the text description is set to 32.
The fixed length of resampled audio embedding $M$ is set to 12. 
The number of layers of the gated fusion module $L$ is set to 4. We use the scaling parameter $\alpha$ in~\cref{eq:local_alignment} of 100. 
$\lambda$ in~\cref{eq:margin} is set to 0.2.
Except for $\delta$ in~\cref{eq:margin}, the same hyperparameter settings are used in both MSR-VTT and VATEX.
$\delta$ is set to 0.1 and 0.05 for MSR-VTT and VATEX, respectively.
\input{tabs/table2}

\subsection{Quantitative Results}
\label{sec:quan}
%Table~\ref{tab:main_results} presents the quantitative results of video-text retrieval on MSR-VTT 9k split~\cite{msrvtt}. 
% Our proposed approach demonstrates superior performance compared to existing methods, including both text-to-video and video-to-text retrieval tasks. 
% % We evaluate retrieval performance using recall metrics at ranks 1, 5, and 10 (R@1, R@5, R@10), which are widely adopted to measure the effectiveness of retrieval systems.
% For the CLIP ViT-B/32~\cite{clip} backbone, our method outperforms state-of-the-art models such as TEFAL~\cite{tefal} and UCoFiA~\cite{ucofia}, achieving R@1 of 50.2\% for text-to-video retrieval, surpassing TEFAL by 0.8\%. Similarly, our approach obtains a substantial gain in video-to-text retrieval, achieving R@1 of 49.7\%. 
% The improvement is consistent across higher recall metrics, highlighting the effectiveness of our audio-guided video representation framework.

% When evaluated with a large size backbone (\ie, CLIP ViT-B/16~\cite{clip}), our method further shows its robustness by achieving R@1 scores of 52.1\% and 51.2\% for text-to-video and video-to-text retrieval, respectively. 
% This performance surpasses other approaches, including UCoFiA and TEFAL, demonstrating the efficacy of incorporating audio modality alongside visual and textual information.
% The consistent improvements across different backbones and retrieval tasks underscore the benefits of our approach in bridging the modality gap and effectively fusing audio-visual information. 
% These quantitative results affirm the advantage of our method in achieving state-of-the-art retrieval performance.
We compare AVIGATE with previous video-text retrieval methods on the MSR-VTT 9k split~\cite{msrvtt} and VATEX~\cite{vatex} datasets, with results presented in Table~\ref{tab:main_results} and Table~\ref{tab:vatex}, respectively.
Each table shows the modalities used by the methods for video-text retrieval, indicated as visual (V), textual (T), and audio (A), with results reported separately for each CLIP ViT backbone size.

%As shown in the tables, our method outperforms previous methods.
%We demonstrate superior performance across all datasets and CLIP ViT backbone sizes in terms of R@1.
These tables demonstrate that AVIGATE outperforms all previous methods in R@1 across all datasets and CLIP ViT backbone sizes.
% Specifically, on MSR-VTT, AVIGATE using the CLIP ViT-B/32 backbone achieves improvements over TEFAL~\cite{tefal}, the previous state-of-the-art audio-based model, by 0.8\%p and 2.6\%p in R@1 for text-to-video and video-to-text retrieval tasks, respectively.
% Moreover, AVIGATE surpasses UATVR~\cite{uatvr} by a large margin, 1.8\%p in terms of R@1 for text-to-video retrieval on VATEX.
Specifically, on MSR-VTT, AVIGATE achieves improvements of 0.8\%p and 2.6\%p over TEFAL~\cite{tefal} (w/ audio SOTA) in text-to-video retrieval and video-to-text retrieval, respectively.
Ours also surpasses UATVR~\cite{uatvr} (w/o audio, but SOTA) by a large margin, 1.8\%p in R@1 on VATEX.
\iffalse
As shown in the tables, our method outperforms previous methods across all datasets and CLIP ViT backbone sizes.
We demonstrate superior performance not only in R@1 but also R@5, R@10 and Rsum, indicating consistently strong retrieval results.
%In particular, compared to TEFAL which incurs high computational costs to extract text-guided audio and visual features, we achieve superior performance while requiring lower computational costs by using only audio-guided visual features.
In particular, compared to TEFAL, which hinders the efficiency of the retrieval system by extracting text-guided audio and visual features, we achieve superior performance by using only audio-guided video representation, allowing for a more suitable retrieval process.
\fi
The improvements of AVIGATE become more distinctive when a larger backbone is used.
% For the larger ViT backbone, AVIGATE outperforms prior state-of-the-art methods~\cite{uatvr,ucofia} by a large margin in both R@1 and RSum on both MSR-VTT and VATEX.
Specifically, on MSR-VTT, AVIGATE achieves a 1.3\%p improvement in text-to-video retrieval and a 3.1\%p in video-to-text retrieval while achieving a 3.0\%p improvement in text-to-video retrieval on VATEX.
Furthermore, our method demonstrates significant improvements in RSum, with 6.6\%p improvements on MSR-VTT.
% These quantitative results demonstrate that our method  
The superior performance of AVIGATE is attributed to its ability to selectively integrate informative audio cues while dynamically adjusting the semantic alignment between video and text, leading to a more discriminative and generalizable cross-modal representation.
\subsection{Qualitative Results}
\label{sec:qual}
% To demonstrate the effectiveness of AVIGATE, %we present the Top-1 retrieved video results given a text query, along with gating scores from the gated fusion transformer.
% In Figure~\ref{fig: qual}, we present Top-1 retrieved video results for the given text query, including the paired audio signal and layer-wise gating scores.
Figure~\ref{fig: qual} illustrates the Top-1 retrieved video results from our method for the given text query, including the paired audio signal and layer-wise gating scores.
% In cases where the audio is uninformative, simple audio-video fusion without gating leads to retrieval failure.
% In contrast, our model assigns low gating scores to uninformative audio, effectively filtering out uninformative signals and retrieving the relevant video.
% Figure~\ref{fig: qual}(a) illustrates a scenario where the audio is informative.
% In this case, our model achieves successful retrieval with high gating scores that enable effective audio fusion.
% However, the baseline model that ignores audio information fails in retrieval.
\iffalse
For the query ``a man is talking about a sports car he is driving''~(Figure~\ref{fig: qual}(a)), our model retrieves the correct video, supported by the informative audio cues that match the content of the query. 
\fi
For the query in Figure~\ref{fig: qual}(a), our model retrieves the correct video, supported by the informative audio cues that match the content of the query. 
% In this example, the audio contains meaningful spoken descriptions, which are reflected in high gating scores ($g_{\text{mha}}^{(l)}$ and $g_{\text{ffn}}^{(l)}$) except $g_{\text{mha}}^{(0)}$, emphasizing the relevance of the auditory information. 
In this example, the audio provides valuable information, reflected by relatively high gating scores ($g_{\text{mha}}^{(l)}$ and $g_{\text{ffn}}^{(l)}$) except $g_{\text{mha}}^{(1)}$ across layers, emphasizing the contribution of the audio in the fusion.
\iffalse
Conversely, for the query ``a man with a very red nose''~(Figure~\ref{fig: qual}(b)), the successfully retrieved video includes background music that is irrelevant content. 
\fi
Conversely, for the query in Figure~\ref{fig: qual}(b), the successfully retrieved video includes background music that is irrelevant content.
The gating mechanism responds accordingly, assigning low gating scores to suppress the influence of irrelevant audio signals. 
This behavior shows that the gated fusion transformer successfully filters out irrelevant audio while using the multi-modal nature of videos only when the audio contributes positively. 
% It demonstrates that our gated fusion transformer can adaptively control the integration of audio embeddings, ensuring that only useful cues contribute to the final video representation. 


\subsection{Ablation Studies}
\label{sec:ablation}
%We evaluate the effectiveness of different components in AVIGATE through comprehensive experiments. 
%The default image encoder is CLIP ViT-B/32~\cite{clip}, and the text-to-video retrieval results are reported on the widely-used MSR-VTT dataset~\cite{msrvtt}.
We evaluate the effectiveness of the proposed components in AVIGATE through comprehensive experiments.
For the ablation study, we report text-to-video retrieval results on the MSR-VTT dataset~\cite{msrvtt} with CLIP ViT-B/32~\cite{clip}. %as the image encoder.

\noindent \textbf{Components of AVIGATE:}
In Table~\ref{tab:ablation_components}, we present the results of the ablation study on the main components of our model.
% A baseline model, which utilizes only video-text modalities without additional audio modality, achieves 45.4\%, 72.2\%, and 81.6\% in terms of R@1, R@5 and R@10, respectively.
We first build a baseline that includes only the CLIP encoders for video and text embeddings, which is learned by a conventional cross-modal contrastive loss.
%When the audio modality is added, we observe an overall performance improvement, indicating that audio contributes positively to text-to-video retrieval.
% \iffalse
Then, the baseline is extended by introducing a simplified fusion transformer without the gating mechanism from our gated fusion transformer to exploit audio modality (Baseline + Audio).
The extended baseline improves overall performance, particularly with a notable 1.7\%p improvement in R@1, demonstrating that audio contributes positively to text-to-video retrieval.
% \fi
\iffalse
Additionally, in the baseline model, we introduce a simplified fusion transformer without the gating mechanism from our gated fusion transformer to add the audio modality to the visual modality.
This integration leads to an overall performance improvement, indicating that audio contributes positively to text-to-video retrieval.
\fi
Subsequently, introducing our main components, including the gated fusion transformer and adaptive margin, consistently improves the extended baseline in all metrics when each component is applied individually.
This observation highlights the effectiveness of the gated fusion transformer, which dynamically adjusts the contribution of the audio, and the benefit of contrastive learning with adaptive margin.
The full configuration of our method achieves the best performance in R@1 at 50.2\% while demonstrating consistent improvements and highlighting the complementary synergy between the gated fusion transformer and the adaptive margin-based contrastive loss.
It is worth noting that employing a fixed margin ($m_{ij}$ in Eq.~\ref{eq:margin} is fixed as 0.1) with the gated fusion transformer achieves a moderate performance gain in R@1, but the most significant improvement is presented when the margin is adaptively employed.
% the superiority of our adaptive margin-based contrastive learning, with a 1.2\%p improvement in R@1 compared to using a fixed margin instead.

% \noindent \textbf{Layer Depth of Gated Fusion Transformer:}
% We present the impact of the number of layers of the gated fusion transformer ($L$) in Table~\ref{tab:ablation_hyp}(a)  and observe that the performance gradually improves up to $L$=4.%, where the best performance is achieved.
%best performance is achieved at $L$=4.
\input{tabs/table_ablation}
\input{tabs/table_hyp}
\noindent \textbf{Granularity of Alignment Scheme:}
We analyze alignment schemes in terms of granularity in Table~\ref{tab:ablation_hyp}, demonstrating that the global-local multi-grained alignment scheme improves performance across all metrics due to its ability to capture the overall semantic context and fine details.

% We explore the influence of the number of layers in the gated fusion transformer and the alignment scheme at global and local levels. 
% In Table~\ref{tab:ablation_hyp}(a), we examine various layer configurations of the gated fusion transformer ($L$) and observe that the best performance is achieved at $L$=4. 
% Lastly, we analyze alignment schemes in terms of granularity in Table~\ref{tab:ablation_hyp}(b), demonstrating that the global-local multi-grained alignment scheme achieves superior performance across all metrics due to its ability to capture both the overall semantic context and fine details.
%\bs{Need to define what is baseline, gate, and margin in the table.}



\subsection{Computational Cost Analysis}
\label{sec:complexity}
\input{tabs/table_complexity}
Let $\mathcal{T}$, $\mathcal{V}$, and $\mathcal{A}$ denote the number of text queries, videos, and audios, respectively, where $\mathcal{A} \leq \mathcal{V}$, as each audio is associated with a corresponding video but not all videos include an audio.
% To demonstrate the efficiency of our model during testing, we compare the computational complexity and latency of AVIGATE with previous methods~\cite{clip4clip,xpool,tefal}, as summarized in Table~\ref{tab:complexity}.
Table~\ref{tab:complexity} compares the computational complexity and latency of AVIGATE with previous methods~\cite{clip4clip,xpool,tefal} to demonstrate the efficiency of our model during testing.
% Specifically, we analyze the time complexity in terms of the required operations for text-to-video retrieval and evaluate the latency for computing similarity scores between pairs of video and text.
% Given $\mathcal{T}$ text queries and $\mathcal{V}$ videos including $\mathcal{A}$ audios, 
AVIGATE achieves an efficient retrieval process with a time complexity of $\mathcal{O}(\mathcal{A}+\mathcal{V} + \mathcal{T})$, while TEFAL introduces additional computational burdens with complexity of $\mathcal{O}(\mathcal{AT} + \mathcal{VT})$.
% We further evaluate the latency for text-to-video retrieval, which involves processing a single text query against a large set of video representations. 
We further evaluate the average latency involved in processing a single text query against a large set of pre-extracted video representations for text-to-video retrieval.
Specifically, we utilize the MSR-VTT-9k test split~\cite{msrvtt}, which comprises 1,000 video-text pairs, where the video representations are pre-extracted and stored, eliminating the need for on-the-fly computation during the retrieval process.
When a text query arrives, the system computes similarity scores between the text embedding and the entire set of video representations. 
% The total latency encompasses two primary components: the time required to extract the text query embedding and the time taken to calculate the similarity scores between the text embedding and all video representations.
The total latency encompasses the extraction of the text embedding and calculating similarity scores between the text embedding and all video representations.
AVIGATE is over 14 times faster than TEFAL and over 6 times faster than X-Pool, as they require cross-modal interaction processes repeatedly for all videos with each text query to generate their final representations, resulting in substantial latency overhead.
% since they necessitate additional cross-modal interaction processes for each text query to generate the final video representations, resulting in substantial latency overhead.
Meanwhile, ours incurs only a slight additional cost due to our multi-grained alignment compared to CLIP4Clip.
% Also, it is worth noting that AVIGATE surpasses TEFAL in terms of R@1 and RSum, as shown in Table~\ref{tab:complexity}.

==> Submission_backup_0304/_5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We have introduced a novel video-text retrieval framework, AVIGATE, that effectively leverages audio cues through a gated attention mechanism. By selectively filtering out uninformative audio signals, AVIGATE enhances the video representation, leading to a more comprehensive understanding of video content. 
Additionally, we proposed an adaptive margin-based contrastive loss to address the inherent positive-negative relationships between visual and textual modalities. 
%This loss function facilitates better alignment between video and text embeddings by dynamically adjusting margins according to intra-modal semantic dissimilarities.
This loss function facilitates a more discriminative and generalized cross-modal embedding space by dynamically adjusting margins according to intra-modal semantic dissimilarities. 
Extensive experiments on public benchmarks demonstrate that AVIGATE achieves state-of-the-art performance and ensures efficient retrieval.
% Our findings highlight the importance of incorporating audio in a selective manner and suggest promising directions for future research in multimodal information retrieval and video understanding.

\noindent\textbf{Acknowledgement.} This work was supported by the *** grant and the *** grant funded by (***-n\%, ****-m\%). 

==> Submission_backup_0304/_7_supple.tex <==





\section{More Architectural Details}
\label{supp_sec:archi}
To efficiently fuse audio embeddings with frame embeddings while reducing computational overhead, we introduce an audio resampler using a query-based transformer framework~\cite{perceiver,detr,flamingo} that utilizes a cross-attention mechanism with $M$ learnable query embeddings. 
Specifically, the audio input is fed into Audio Spectrogram Transformer (AST)~\cite{ast}, and the output is then passed to the audio resampler to reduce the number of audio embeddings to a fixed length of $M$ while preserving essential information.
As shown in Figure~\ref{fig:resampler}, the audio resampler comprises $K$ audio resampler blocks, each with multi-head self-attention (MHSA), multi-head cross-attention (MHA), and a feed-forward network (FFN).
We set $K$ as 4 for default. 

MHSA first allows the learnable query embeddings to interact and capture contextual relationships among themselves, refining their initial representations. This is followed by MHA, where the query embeddings attend to the output of AST, extracting audio embeddings with a fixed length of $M$.
The FFN then processes the audio embeddings to refine them.
This sequence of operations enables the audio resampler to reduce the number of audio embeddings efficiently while preserving critical information, facilitating seamless fusion with the frame embeddings in subsequent stages.
\begin{figure}[t!]
    % \vspace{-1mm}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/supp_resampler_v2.pdf}
    \caption{The overall architecture of audio resampler.}
    \label{fig:resampler}
    \vspace{-3mm}
\end{figure}

\bs{The MLP consists of two layers with dimensions $\mathbb{R}^{2D\times D/2}$ and $\mathbb{R}^{D/2 \times 1}$, using a QuickGELU as the non-linearity between them.}

\section{More Quantitative Results}
\label{supp_sec:quan}
\noindent\textbf{Effect of Post-Processing:}
% \bs{About post processing...}
Post-processing techniques have been widely adopted in video-text retrieval to enhance performance by refining similarity scores.
Previous methods~\cite{camoe,ts2,ucofia,uatvr,tefal} adopt the post-processing techniques, including Dual Softmax Loss (DSL)~\cite{camoe}, Querybank Norm (QB-Norm)~\cite{qbnorm}, and the Sinkhorn-Knopp algorithm (SK-Norm), for further improvements in retrieval accuracy.
We also explore the effect of the post-processing technique by adopting DSL that applies inverted softmax~\cite{inverted} during inference.
We report the retrieval performance of AVIGATE with and without post-processing in Table~\ref{tab:supp_postprocessing} compared with existing methods.
Our model, AVIGATE, consistently achieves superior performance across all evaluation metrics for both text-to-video and video-to-text retrieval tasks, outperforming all previous methods by significant margins. 
Specifically, for the CLIP ViT-B/32 backbone, AVIGATE with post-processing achieves R@1 of 53.9\% for text-to-video retrieval.
Furthermore, in video-to-text retrieval, AVIGATE with DSL achieves R@1 of 53.0\%. 
Similarly, for the CLIP ViT-B/16 backbone, AVIGATE achieves substantial gains over existing methods. 
When using post-processing, our method achieves R@1 of 56.3\% for text-to-video retrieval, representing a considerable 2.3\%p improvement over TS2-Net~\cite{ts2}. 
In video-to-text retrieval, AVIGATE also outperforms other methods with R@1 of 57.4\%.

\input{tabs/supp_table_post}
\input{tabs/supp_table_vatex}
\noindent\textbf{Entire Performance on VATEX:}
We present the complete video-text retrieval results on VATEX~\cite{vatex} in Table~\ref{tab:supp_vatex}, including both text-to-video and video-to-text retrieval.
\iffalse
Our method, AVIGATE, is evaluated with two variants of the CLIP ViT backbone (\ie, ViT-B/32 and ViT-B/16).
As shown in Table~\ref{tab:supp_vatex}, AVIGATE achieves notable results in text-to-video retrieval, with R@1 of 63.1\% and 67.5\% for ViT-B/32 and ViT-B/16, respectively. 
In the video-to-text retrieval task, AVIGATE also demonstrates impressive performance, achieving R@1 of 76.6\% and 80.7\% for ViT-B/32 and ViT-B/16, respectively. 
These results highlight the scalability of AVIGATE across different backbone sizes.
% In addition, we demonstrate the effect of post-processing, as detailed in Table~\ref{tab:supp_vatex}.
Furthermore, the use of the post-processing technique, DSL~\cite{camoe}, leads to a significant boost in retrieval accuracy.
% Specifically, RSum increases from 522.0 to 545.2 with ViT-B/32 and from 535.4 to 555.6 with ViT-B/16, indicating a substantial gain in overall retrieval accuracy.
\fi
The results are reported using two variants of the CLIP ViT backbone, CLIP ViT-B/32 and CLIP ViT-B/16.
Moreover, we assess the effect of the post-processing technique, DSL~\cite{camoe}, for further performance boosts.
With the CLIP ViT-B/32 backbone, AVIGATE achieves notable results in text-to-video retrieval, with R@1 of 63.1\% and 76.6\% for text-to-video retrieval and video-to-text retrieval, respectively.
When applying DSL, we observe significant improvements across all metrics.
Specifically, it improves AVIGATE by a large margin, 7.6\%p and 8.7\%p in R@1 for text-to-video retrieval and video-to-text retrieval, respectively.
When employing the larger backbone, CLIP ViT-B/16, our method demonstrates the scalability across different backbone sizes, achieving R@1 of 67.5\% for text-to-video retrieval and 80.7\% for video-to-text retrieval.
Moreover, the use of DSL consistently boosts the retrieval accuracy overall, with 20.2\%p improvements in RSum.


\section{Comparison to Recent Work}
\label{supp_sec:tmass}
\bs{(To be removed?)
T-MASS~\cite{tmass} presents a state-of-the-art performance in video-text retrieval, introducing a stochastic text modeling method.
Although we aimed to conduct a comprehensive evaluation that included comparisons with recent state-of-the-art methods, this was unfortunately not possible due to the unavailability of their official code repository\footnote[1]{\url{https://github.com/Jiamian-Wang/T-MASS-text-video-retrieval}}, which appears to have been removed from GitHub due to technical or unforeseen issues.
Without access to the implementation details or pretrained models, reproducing their results consistently and fairly was not feasible. Considering the critical importance of reproducibility, we opted to exclude T-MASS from our experiments rather than risk an inaccurate and incomplete evaluation.
}
% We appreciate their contributions to the field and would be glad to include such comparisons if the necessary resources become available in the future.


\section{More Ablation Studies}
\label{supp_sec:ablation}
We further conduct ablation studies using varying hyperparameters in AVIGATE.
Similar to the main paper, we report text-to-video retrieval results on the MSR-VTT dataset~\cite{msrvtt} with CLIP ViT-B/32. Table~\ref{tab:supp_ablation_hyp} presents the whole results of the ablation studies.

\noindent \textbf{Layer Depth of Gated Fusion Transformer:}
We present the impact of the number of layers of the gated fusion transformer ($L$) in Table~\ref{tab:supp_ablation_hyp}(a)  and observe that the performance gradually improves up to $L$=4, where the best performance is achieved.

\noindent \textbf{Hyperparameters $\lambda$ and $\delta$ in Eq.~(5):}
We investigate the impact of the scaling factor $\lambda$ and the maximum margin $\delta$ in Eq.~(5) of the manuscript.
It is worth noting that the adaptive margin in Eq.~(5) becomes 0 when $\lambda$ or $\delta$ are set to 0, leading the loss in Eq.~(6) to the conventional contrastive loss.
As shown in Table~\ref{tab:supp_ablation_hyp}(b), when $\lambda$ is set to 0.2, the model yields the best performance. 
Meanwhile, setting $\lambda$ to 0.1 results in a slight decrease in performance, indicating that a smaller scaling factor may not provide sufficient margin adjustment.  
However, increasing $\lambda$ to 0.3 does not lead to further improvements.
Similarly, Table~\ref{tab:supp_ablation_hyp}(c) presents the effect of varying the maximum margin $\delta$. 
We observe that the performance gradually improves up to $\delta = 0.1$.
Increasing $\delta$ beyond 0.1 degrades performance due to excessively large margins pushing negative pairs too far apart.

\noindent \textbf{Gate Mechanism Type:}
Our method employs a soft gate mechanism, which allows for continuous modulation of the contribution of audio during fusion.
To evaluate the effectiveness of the soft gate mechanism, we compare the soft gate with a hard gate mechanism, which assigns a gating score of 1 if it exceeds a predefined threshold and 0 otherwise.
As shown in Table~\ref{tab:supp_ablation_hyp}(d), using the hard gate underperforms our method.
% The performance degradation when using the hard gate is attributed to its binary decision-making.
Unlike using the hard gate mechanism, our method facilitates the effective use of relevant audio cues while minimizing the impact of irrelevant or noisy audio signals; it enables the model to leverage informative audio more precisely, thereby improving retrieval accuracy.

\input{tabs/supp_table_ablation}

\begin{figure*}[t!]
    \vspace{-1mm}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/Supple_Qual.pdf}
    \vspace{-2mm}
    \caption{ Top-1 text-to-video retrieval results of our method on MSR-VTT, where they are true matches.
    The audio provides informative cues for accurate retrieval, where ``a man is talking'' in the query text is not visible (a) and ``talk$\cdots$san diego'' in the query text is not visible but audible (b).
    However, neglecting these informative audio signals (\ie, w/o Audio) fails to retrieve true matches. 
    Meanwhile, The irrelevant audio is filtered by the gated fusion transformer, leading to an accurate retrieval result (c) and (d); without the gating mechanism (\ie, w/o Gate), it leads to retrieving false matches due to the irrelevant audio.    
    }
    \label{fig:supp_qual}
    \vspace{-3.5mm}
\end{figure*}
\section{More Qualitative Results}
\label{supp_sec:qual}
We further present additional qualitative results that illustrate the effectiveness of AVIGATE in leveraging audio information for text-to-video retrieval. 
Figure~\ref{fig:supp_qual} shows the Top-1 retrieved videos from our method, including the corresponding audio signals, to highlight how audio cues influence retrieval outcomes.

In Figure~\ref{fig:supp_qual}(a) and (b), we present a scenario where the audio provides valuable information that enables improving retrieval performance. 
AVIGATE, which incorporates audio through the gated fusion transformer, successfully retrieves the correct video corresponding to the text query. In contrast, the method without audio information (\ie, w/o Audio) fails to retrieve the true matches. This comparison highlights the benefit of utilizing informative audio cues.

Conversely, Figure~\ref{fig:supp_qual}(c) and (d) present another scenario where the audio input contains irrelevant information, such as background noise. AVIGATE effectively filters out the uninformative audio signals through the gating mechanism. The gating function assigns low gating scores, allowing the model to focus only on the visual cues. As a result, AVIGATE successfully retrieves the correct videos. In contrast, the method without the gating function (\ie, w/o Gate) is impacted by the noisy audio and fails to retrieve the true matches.

These qualitative results demonstrate that the gated fusion transformer successfully filters out irrelevant audio while leveraging valuable audio information when the audio contributes positively.

==> Submission_backup_0304/subtabs/supp_table_ablation.tex <==

\begin{table}[!t]
% \vspace{-5mm}
\setlength{\tabcolsep}{2pt}
\fontsize{8.2}{9}\selectfont
\centering
\scalebox{0.95}{
\begin{tabularx}{0.499\textwidth}
    {
      >{\centering\arraybackslash}p{0.13\textwidth}
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X
      }
     \toprule
    \multirow{1}{*}[-4.5mm]{\textbf{Ablated Setting}} & \multicolumn{3}{c}{\textbf{Text-to-Video Retrieval}} \\ [-0.3ex] \cmidrule(lr){2-4}  
    &  R@1 & R@5 & R@10   \\  [-0.4ex] \midrule
    \multicolumn{4}{l}{\textit{\textbf{(a) Layer depth of Gated Fusion Transformer: $L$}}} \\ [-0.3ex]\midrule
    $L$=1 & 49.0 & 74.0 & 82.6 \\
    $L$=2  & 49.8 & 74.0 & 83.0 \\
    \ccol$L$=4  &\ccol 50.2 &\ccol  74.3 & \ccol 83.2 \\
    $L$=6  & 49.5 & 74.2 & 82.6 \\    [-0.3ex]\midrule
    \multicolumn{4}{l}{\textit{\textbf{(b) Scaling factor in Eq.(5): $\lambda$}}} \\ [-0.3ex]\midrule
    $\lambda$=0.0 & 48.0 & 75.1 & 83.4 \\
    $\lambda$=0.1 & 49.4 & 74.8 & 83.8 \\
    \ccol$\lambda$=0.2  &\ccol 50.2 &\ccol  74.3 & \ccol 83.2 \\
    $\lambda$=0.3  & 50.0 & 74.4 & 83.2 \\    [-0.3ex]\midrule
    \multicolumn{4}{l}{\textit{\textbf{(c) Maximum margin in Eq.(5): $\delta$}}} \\ [-0.3ex]\midrule
    $\delta$=0.00 & 48.0 & 75.1 & 83.4 \\
    $\delta$=0.05 & 49.4 & 75.1 & 83.6 \\
    \ccol$\delta$=0.10  &\ccol 50.2 &\ccol  74.3 & \ccol 83.2 \\
    $\delta$=0.15 & 49.3 & 74.8 & 83.8 \\
    $\delta$=0.20  & 48.3 & 74.4 & 83.9 \\  [-0.3ex]\midrule
    \multicolumn{4}{l}{\textit{\textbf{(d) Gate mechanism type}}} \\ [-0.3ex]\midrule
    Hard Gate & 49.3 & 75.0 & 82.5 \\
    \ccol Soft Gate  &\ccol 50.2 &\ccol  74.3 & \ccol 83.2 \\
[-0.3ex]\bottomrule 
\end{tabularx}
}
\vspace{-1.5mm}
\caption{Ablation studies on hyperparameters. 
\colorbox{grey}{{gray}} corresponds to our default setting.
}
\label{tab:supp_ablation_hyp}
\vspace{-4mm}
\end{table}



==> Submission_backup_0304/subtabs/supp_table_post.tex <==
% \begin{table*}[!t]
% \fontsize{8}{9.2}\selectfont
% \centering
% \begin{tabularx}{0.98\textwidth}
%     {
%       p{0.18\textwidth}
%       >{\raggedright\arraybackslash}p{0.07\textwidth}
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X 
%       >{\centering\arraybackslash}X
%       }
%      \toprule
%     {\multirow{1}{*}[-4.5mm]{\textbf{Methods}}}& \multirow{1}{*}[-4.5mm]{\textbf{Modality}}&
%     \multicolumn{3}{c}{\textbf{Text-to-Video Retrieval}} & \multicolumn{3}{c}{\textbf{Video-to-Text Retrieval}} & \multirow{2}{*}{RSum} \\ [-0.3ex]  \cmidrule(lr){3-5}  
%     \cmidrule(lr){6-8} & & R@1 & R@5 & R@10 &  R@1 & R@5 & R@10 & \\  [-0.4ex] \midrule
%     \multicolumn{9}{l}{\textit{\textbf{CLIP ViT-B/32}}} \\ [-0.3ex]\midrule
%     CAMoE~\cite{camoe} & V+T& 44.6 & 72.6 & 81.8 & 45.1 & 72.4 & 83.1 & 399.6 \\
%     ~~+DSL& V+T & 47.3  & 74.2 & 84.5 & 49.1 & 74.3 & 84.3 & 413.7 \\
%     TS2-Net~\cite{ts2} & V+T & 47.0 & 74.5 & {83.8} & 45.3 & 74.1 & 83.7 & 408.4 \\
%     ~~+DSL & V+T & 51.1 & 76.9 & 85.6 & - & - & - & - \\
%     UATVR~\cite{uatvr} & V+T & 47.5 & 73.9 & 83.5 & 46.9 & 73.8 & {83.8} & 409.4 \\
%     ~~+DSL & V+T & 49.8 & 76.1 & 85.5 & 51.1 & 74.8 & {85.1} & 422.4 \\
%     UCoFiA~\cite{ucofia}  & V+T &  48.2 & 73.3 & 82.3 & - & - & - & - \\
%     ~~+SK norm  & V+T &  {49.4} & 72.1 & 83.5 & {47.1} & 74.3 & 83.0 & 409.4 \\
%     % TEFAL~\cite{tefal} & A+V+T & {49.4} & 75.9 & 83.9 & {47.1} & {75.1} & 84.9 & 416.3 \\
%     \ccol  AVIGATE (Ours) & \ccol A+V+T &\ccol  {50.2} & \ccol {74.3}  &\ccol  83.2 &\ccol {49.7} &  \ccol  {75.3}   & \ccol 83.7 & \ccol {416.4}    \\
%     \ccol  ~~+DSL & \ccol A+V+T &\ccol  \textbf{53.9} & \ccol \textbf{77.0}  &\ccol  \textbf{86.0} &\ccol \textbf{53.0} &  \ccol  \textbf{78.2}   & \ccol \textbf{85.4} & \ccol \textbf{433.5}    \\    
%     \midrule
%     \multicolumn{9}{l}{\textit{\textbf{CLIP ViT-B/16}}} \\ [-0.4ex] \midrule
%     % X-Pool~\cite{xpool} & V+T & 48.2 & 73.7 & 82.6 & 46.4 & 73.9 & 84.1 & 408.9 \\
%     TS2-Net~\cite{ts2} & V+T & 49.4 & 75.6 & 85.3 & 46.6 & 75.9 & 84.9 & 417.7 \\
%     ~~+DSL & V+T & 54.0 & 79.3 & 87.4 & - & - & - & - \\
%     TEFAL~\cite{tefal} & A+V+T & 49.9 & 76.2 & 84.4  & - & - & - & - \\
%     ~~+DSL+QB-Norm & A+V+T & 52.0 & 76.6 & 86.1  & - & - & - & - \\
%     UATVR~\cite{uatvr} & V+T & {50.8} & {76.3} & 85.5 & 48.1 & 76.3 & {85.4} & 422.4 \\ 
%     ~~+DSL & V+T & {53.5} & {79.5} & 88.1 & 54.5 & 79.1 & \textbf{87.9} & 442.6 \\ 
%     \ccol  AVIGATE (Ours) & \ccol A+V+T &\ccol  {52.1} & \ccol {76.4} &\ccol  {85.2} &\ccol {51.2} &  \ccol  {77.9}   & \ccol {86.2} & \ccol {429.0}    \\
%     \ccol  ~~+DSL & \ccol A+V+T &\ccol  \textbf{56.3} & \ccol \textbf{80.8} &\ccol  \textbf{88.1} &\ccol \textbf{57.4} &  \ccol  \textbf{80.2}   & \ccol {87.4} & \ccol \textbf{450.2}    \\
% \bottomrule 
% \end{tabularx}
% \vspace{-1.5mm}
% \caption{Text-to-video and video-to-text retrieval results on the MSR-VTT 9k split. 
% Post-processing techniques such as DSL~\cite{camoe}, QB-Norm~\cite{qbnorm}, and SK norm are used for further performance boosting.
% }
% \label{tab:main_results}
% \vspace{-3mm}
% \end{table*}

\begin{table*}[!t]
\fontsize{8}{9.2}\selectfont
\centering
\begin{tabularx}{0.98\textwidth}
    {
      p{0.153\textwidth}
      >{\raggedright\arraybackslash}p{0.07\textwidth}
      >{\raggedright\arraybackslash}p{0.075\textwidth}
      >{\raggedright\arraybackslash}p{0.075\textwidth}
      >{\raggedright\arraybackslash}p{0.075\textwidth}
      >{\raggedright\arraybackslash}p{0.075\textwidth}
      >{\raggedright\arraybackslash}p{0.075\textwidth}
      >{\raggedright\arraybackslash}p{0.075\textwidth}
      >{\raggedright\arraybackslash}X
      }
     \toprule
    {\multirow{1}{*}[-4.5mm]{\textbf{Methods}}}& \multirow{1}{*}[-4.5mm]{\textbf{Modality}}&
    \multicolumn{3}{c}{\textbf{Text-to-Video Retrieval}} & \multicolumn{3}{c}{\textbf{Video-to-Text Retrieval}} & \multicolumn{1}{c}{\multirow{2}{*}{RSum}} \\ [-0.3ex]  \cmidrule(lr){3-5}  
    \cmidrule(lr){6-8} & & R@1 & R@5 & R@10 &  R@1 & R@5 & R@10 & \\  [-0.4ex] \midrule
    \multicolumn{9}{l}{\textit{\textbf{CLIP ViT-B/32}}} \\ [-0.3ex]\midrule
    CAMoE~\cite{camoe} & V+T& 44.6 & 72.6 & 81.8 & 45.1 & 72.4 & 83.1 & 399.6 \\
    ~~+DSL& V+T & 47.3 \textcolor{grn}{(+2.7)} & 74.2 \textcolor{grn}{(+1.6)} & 84.5 \textcolor{grn}{(+2.7)} & 49.1 \textcolor{grn}{(+4.0)} & 74.3 \textcolor{grn}{(+1.9)} & 84.3 \textcolor{grn}{(+1.2)} & 413.7 \textcolor{grn}{(+14.1)} \\
    TS2-Net~\cite{ts2} & V+T & 47.0 & 74.5 & {83.8} & 45.3 & 74.1 & 83.7 & 408.4 \\
    ~~+DSL & V+T & 51.1 \textcolor{grn}{(+4.1)} & 76.9 \textcolor{grn}{(+2.4)} & 85.6 \textcolor{grn}{(+1.8)} & - & - & - & - \\
    UATVR~\cite{uatvr} & V+T & 47.5 & 73.9 & 83.5 & 46.9 & 73.8 & {83.8} & 409.4 \\
    ~~+DSL & V+T & 49.8 \textcolor{grn}{(+2.3)} & 76.1 \textcolor{grn}{(+2.2)} & 85.5 \textcolor{grn}{(+2.0)} & 51.1 \textcolor{grn}{(+4.2)} & 74.8 \textcolor{grn}{(+1.0)} & 85.1 \textcolor{grn}{(+1.3)} & 422.4 \textcolor{grn}{(+13.0)} \\
    UCoFiA~\cite{ucofia}  & V+T &  48.2 & 73.3 & 82.3 & - & - & - & - \\
    ~~+SK norm  & V+T &  49.4 \textcolor{grn}{(+1.2)} & 72.1 \textcolor{red}{(-0.9)} & 83.5 \textcolor{grn}{(+1.2)} & {47.1} & 74.3 & 83.0 & 409.4 \\

    % TEFAL~\cite{tefal} & A+V+T & {49.4} & 75.9 & 83.9 & {47.1} & {75.1} & 84.9 & 416.3 \\
    \ccol  AVIGATE (Ours) & \ccol A+V+T &\ccol  {50.2} & \ccol {74.3}  &\ccol  83.2 &\ccol {49.7} &  \ccol  {75.3}   & \ccol 83.7 & \ccol {416.4}    \\
    \ccol  ~~+DSL & \ccol A+V+T &\ccol  \textbf{53.9} \textcolor{grn}{(+3.7)} & \ccol \textbf{77.0} \textcolor{grn}{(+2.7)}  &\ccol  \textbf{86.0} \textcolor{grn}{(+2.8)} &\ccol \textbf{53.0} \textcolor{grn}{(+3.3)} &  \ccol  \textbf{78.2} \textcolor{grn}{(+2.9)}   & \ccol \textbf{85.4} \textcolor{grn}{(+1.7)} & \ccol \textbf{433.5} \textcolor{grn}{(+16.9)}     \\    
    \midrule
    \multicolumn{9}{l}{\textit{\textbf{CLIP ViT-B/16}}} \\ [-0.4ex] \midrule
    % X-Pool~\cite{xpool} & V+T & 48.2 & 73.7 & 82.6 & 46.4 & 73.9 & 84.1 & 408.9 \\
    TS2-Net~\cite{ts2} & V+T & 49.4 & 75.6 & 85.3 & 46.6 & 75.9 & 84.9 & 417.7 \\
    ~~+DSL & V+T & 54.0 \textcolor{grn}{(+4.6)} & 79.3 \textcolor{grn}{(+3.7)} & 87.4 \textcolor{grn}{(+2.1)} & - & - & - & - \\
    TEFAL~\cite{tefal} & A+V+T & 49.9 & 76.2 & 84.4  & - & - & - & - \\
    ~~+DSL+QB-Norm & A+V+T & 52.0 \textcolor{grn}{(+2.1)} & 76.6 \textcolor{grn}{(+0.4)} & 86.1 \textcolor{grn}{(+1.7)}  & - & - & - & - \\
    UATVR~\cite{uatvr} & V+T & {50.8} & {76.3} & 85.5 & 48.1 & 76.3 & {85.4} & 422.4 \\ 
    ~~+DSL & V+T & {53.5} \textcolor{grn}{(+2.7)} & {79.5} \textcolor{grn}{(+3.2)} & 88.1 \textcolor{grn}{(+2.7)} & 54.5 \textcolor{grn}{(+6.4)} & 79.1 \textcolor{grn}{(+2.8)} & \textbf{87.9} \textcolor{grn}{(+2.5)} & 442.6 \textcolor{grn}{(+20.2)} \\ 
    \ccol  AVIGATE (Ours) & \ccol A+V+T &\ccol  {52.1} & \ccol {76.4} &\ccol  {85.2} &\ccol {51.2} &  \ccol  {77.9}   & \ccol {86.2} & \ccol {429.0}    \\
    \ccol  ~~+DSL & \ccol A+V+T &\ccol  \textbf{56.3} \textcolor{grn}{(+4.2)} & \ccol \textbf{80.8} \textcolor{grn}{(+4.4)} &\ccol  \textbf{88.1} \textcolor{grn}{(+2.9)} &\ccol \textbf{57.4} \textcolor{grn}{(+6.2)} &  \ccol  \textbf{80.2} \textcolor{grn}{(+2.3)}   & \ccol {87.4} \textcolor{grn}{(+1.2)} & \ccol \textbf{450.2} \textcolor{grn}{(+21.2)}    \\
[-0.3ex]\bottomrule 
\end{tabularx}
\vspace{-1.5mm}
\caption{Text-to-video and video-to-text retrieval results on the MSR-VTT 9k split. 
The post-processing techniques such as DSL~\cite{camoe}, QB-Norm~\cite{qbnorm}, and SK norm are used for further performance boosting.
}
\label{tab:supp_postprocessing}
\vspace{-3mm}
\end{table*}



==> Submission_backup_0304/subtabs/supp_table_vatex.tex <==
\begin{table*}[!t]
\fontsize{8}{9.2}\selectfont
\centering
\begin{tabularx}{0.98\textwidth}
    {
      p{0.153\textwidth}
      >{\raggedright\arraybackslash}p{0.07\textwidth}
      >{\raggedright\arraybackslash}p{0.075\textwidth}
      >{\raggedright\arraybackslash}p{0.075\textwidth}
      >{\raggedright\arraybackslash}p{0.075\textwidth}
      >{\raggedright\arraybackslash}p{0.075\textwidth}
      >{\raggedright\arraybackslash}p{0.075\textwidth}
      >{\raggedright\arraybackslash}p{0.075\textwidth}
      >{\raggedright\arraybackslash}X
      }
     \toprule
    {\multirow{1}{*}[-4.5mm]{\textbf{Methods}}}& \multirow{1}{*}[-4.5mm]{\textbf{Modality}}&
    \multicolumn{3}{c}{\textbf{Text-to-Video Retrieval}} & \multicolumn{3}{c}{\textbf{Video-to-Text Retrieval}} & \multicolumn{1}{c}{\multirow{2}{*}{RSum}} \\ [-0.3ex]  \cmidrule(lr){3-5}  
    \cmidrule(lr){6-8} & & R@1 & R@5 & R@10 &  R@1 & R@5 & R@10 & \\  [-0.4ex] \midrule
    \multicolumn{9}{l}{\textit{\textbf{CLIP ViT-B/32}}} \\ [-0.3ex]\midrule
      AVIGATE (Ours) &  A+V+T &  {63.1} &  {90.7}  &  95.5 & 76.6 &    97.3   &  98.8 &  522.0    \\
      ~~+DSL &  A+V+T &  \textbf{70.7} \textcolor{grn}{(+7.6)} &  \textbf{93.4} \textcolor{grn}{(+2.7)} &  \textbf{95.5} \textcolor{grn}{(+1.4)} &  \textbf{85.3} \textcolor{grn}{(+8.7)} &  \textbf{99.1} \textcolor{grn}{(+1.8)} &  \textbf{99.8} \textcolor{grn}{(+1.0)} &  \textbf{545.2} \textcolor{grn}{(+23.2)} \\
    \midrule
    \multicolumn{9}{l}{\textit{\textbf{CLIP ViT-B/16}}} \\ [-0.4ex] \midrule

    AVIGATE (Ours) &  A+V+T &  67.5 &  93.2 &  96.7 & 80.7 &    97.8   &  99.5 &  535.4    \\
      ~~+DSL &  A+V+T &  \textbf{74.6} \textcolor{grn}{(+7.1)} &  \textbf{95.3} \textcolor{grn}{(+2.1)} &  \textbf{97.8} \textcolor{grn}{(+1.1)} &  \textbf{88.7} \textcolor{grn}{(+8.0)} &  \textbf{99.3} \textcolor{grn}{(+1.5)} &  \textbf{99.9} \textcolor{grn}{(+0.3)} &  \textbf{555.6} \textcolor{grn}{(+20.2)}          \\
\bottomrule 
\end{tabularx}
\vspace{-1.5mm}
\caption{Text-to-video and video-to-text retrieval results on VATEX. 
The post-processing technique, DSL~\cite{camoe}, is used for further performance boosting.
}
\label{tab:supp_vatex}
\vspace{-3mm}
\end{table*}


==> Submission_backup_0304/tabs/table1.tex <==

% \begin{table*}[!t]
% % \vspace{-5mm}
% \setlength{\tabcolsep}{2.5pt}
% \fontsize{9}{10}\selectfont
% \centering
% \begin{tabularx}{1.0\textwidth}
%     {
%       p{0.18\textwidth}
%       >{\raggedright\arraybackslash}p{0.07\textwidth}
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X 
%       % >{\centering\arraybackslash}X
%       }
%      \toprule
%     {\multirow{1}{*}[-4.5mm]{\textbf{Methods}}}& \multirow{1}{*}[-4.5mm]{\textbf{Modality}}&
%     \multicolumn{3}{c}{\textbf{Text-to-Video Retrieval}} & \multicolumn{3}{c}{\textbf{Video-to-Text Retrieval}} \\ [-0.3ex]  \cmidrule(lr){3-5}  
%     \cmidrule(lr){6-8} & & R@1 & R@5 & R@10 &  R@1 & R@5 & R@10  \\  [-0.4ex] \midrule
%     \multicolumn{8}{l}{\textit{\textbf{CLIP ViT-B/32}}} \\ [-0.3ex]\midrule
%     CLIP4Clip$_{meanP}$~\cite{clip4clip} & V+T &43.1 & 70.4 & 80.8 & 43.1 & 70.5 & 81.2 \\
%     CLIP4Clip$_{seqTransf}$~\cite{clip4clip}& V+T & 44.5 & 71.4 & 81.6 & 42.7 & 70.9 & 80.6 \\
%     CAMoE$^\dagger$~\cite{camoe} & V+T& 44.6 & 72.6 & 81.8 & 45.1 & 72.4 & 83.1 \\
%     ECLIPSE~\cite{eclipse} & A+V+T & 44.9 & 71.3 & 81.6 & 44.7 & 71.9 & 82.8 \\
%     X-CLIP~\cite{xclip} & V+T & 46.1  & 73.0 & 83.1 & 46.8 & 73.3 & 84.0 \\
%     X-Pool~\cite{xpool} & V+T & 46.9 & 72.8 & 82.2 & 44.4 & 73.3 & 84.0 \\
%     TS2-Net~\cite{ts2} & V+T & 47.0 & 74.5 & {83.8} & 45.3 & 74.1 & 83.7 \\
%     UATVR~\cite{uatvr} & V+T & 47.5 & 73.9 & 83.5 & 46.9 & 73.8 & {83.8} \\
%     ProST~\cite{prost} & V+T & 48.2 & 74.6 & 83.4 & 46.3 & 74.2 & 83.2 \\
%     UCoFiA$^\dagger$~\cite{ucofia}  & V+T &  {49.4} & 72.1 & 83.5 & {47.1} & 74.3 & 83.0 \\
%     TEFAL~\cite{tefal} & A+V+T & {49.4} & \textbf{75.9} & \textbf{83.9} & {47.1} & {75.1} & \textbf{84.9} \\
%     \ccol  AVIGATE (Ours) & \ccol A+V+T &\ccol  \textbf{50.2} & \ccol {74.3}  &\ccol  83.2 &\ccol \textbf{49.7 }&  \ccol  \textbf{75.3}   & \ccol 83.7    \\
%     % \ccol  Ours + DSL & \ccol A+V+T &\ccol  51.8 & 76.3 \ccol &\ccol  85.3 &\ccol 49.0 &  \ccol  70.9   & \ccol 79.2    \\     
%     \midrule
%     \multicolumn{8}{l}{\textit{\textbf{CLIP ViT-B/16}}} \\ [-0.4ex] \midrule
%     X-Pool~\cite{xpool} & V+T & 48.2 & 73.7 & 82.6 & 46.4 & 73.9 & 84.1 \\
%     TS2-Net~\cite{ts2} & V+T & 49.4 & 75.6 & 85.3 & 46.6 & 75.9 & 84.9 \\
%     ProST~\cite{prost} & V+T & 49.5 & 75.0 & 84.0 & 48.0 & 75.9 & 85.2 \\
%     UCoFiA$^\dagger$~\cite{ucofia}  & V+T &  49.8 & 74.6 & 83.5 & {49.1} & {77.0} & 83.8 \\
%     TEFAL~\cite{tefal} & A+V+T & 49.9 & 76.2 & 84.4  & - & - & -\\
%     UATVR~\cite{uatvr} & V+T & {50.8} & {76.3} & \textbf{85.5} & 48.1 & 76.3 & {85.4} \\ 
%     \ccol  AVIGATE (Ours) & \ccol A+V+T &\ccol  \textbf{52.1} & \ccol \textbf{76.4 } &\ccol  {85.2} &\ccol \textbf{51.2} &  \ccol  \textbf{77.9}   & \ccol \textbf{86.2}    \\
%     % \ccol  Ours + DSL & \ccol A+V+T &\ccol  53.8 & 80.1 \ccol &\ccol  87.1 &\ccol 53.4 &  \ccol  75.2   & \ccol 82.8    \\ \midrule
     
% \bottomrule 
% \end{tabularx}
% \vspace{-2.5mm}
% \caption{Text-to-video and video-to-text retrieval results on MSR-VTT 9k split. \textbf{Bold} denotes the best performance. $^\dagger$ denotes the use of post-processing techniques.
% }
% \label{tab:main_results}
% \vspace{-4mm}
% \end{table*}


\begin{table*}[!t]
% \vspace{-5mm}
% \setlength{\tabcolsep}{2.5pt}
\fontsize{8}{9.2}\selectfont
\centering
\begin{tabularx}{0.98\textwidth}
    {
      p{0.18\textwidth}
      >{\raggedright\arraybackslash}p{0.07\textwidth}
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X 
      >{\centering\arraybackslash}X
      }
     \toprule
    {\multirow{1}{*}[-4.5mm]{\textbf{Methods}}}& \multirow{1}{*}[-4.5mm]{\textbf{Modality}}&
    \multicolumn{3}{c}{\textbf{Text-to-Video Retrieval}} & \multicolumn{3}{c}{\textbf{Video-to-Text Retrieval}} & \multirow{2}{*}{RSum} \\ [-0.3ex]  \cmidrule(lr){3-5}  
    \cmidrule(lr){6-8} & & R@1 & R@5 & R@10 &  R@1 & R@5 & R@10 & \\  [-0.4ex] \midrule
    \multicolumn{9}{l}{\textit{\textbf{CLIP ViT-B/32}}} \\ [-0.3ex]\midrule
    CLIP4Clip$_{meanP}$~\cite{clip4clip} & V+T &43.1 & 70.4 & 80.8 & 43.1 & 70.5 & 81.2 & 389.1 \\
    CLIP4Clip$_{seqTransf}$~\cite{clip4clip}& V+T & 44.5 & 71.4 & 81.6 & 42.7 & 70.9 & 80.6 & 391.7 \\
    % CAMoE$^\dagger$~\cite{camoe} & V+T& 44.6 & 72.6 & 81.8 & 45.1 & 72.4 & 83.1 & 399.6 \\
    ECLIPSE~\cite{eclipse} & A+V+T & 44.9 & 71.3 & 81.6 & 44.7 & 71.9 & 82.8 & 397.2 \\
    X-CLIP~\cite{xclip} & V+T & 46.1  & 73.0 & 83.1 & 46.8 & 73.3 & 84.0 & 406.3 \\
    X-Pool~\cite{xpool} & V+T & 46.9 & 72.8 & 82.2 & 44.4 & 73.3 & 84.0 & 403.6 \\
    TS2-Net~\cite{ts2} & V+T & 47.0 & 74.5 & {83.8} & 45.3 & 74.1 & 83.7 & 408.4 \\
    UATVR~\cite{uatvr} & V+T & 47.5 & 73.9 & 83.5 & 46.9 & 73.8 & {83.8} & 409.4 \\
    ProST~\cite{prost} & V+T & 48.2 & 74.6 & 83.4 & 46.3 & 74.2 & 83.2 & 409.9 \\
    UCoFiA$^\dagger$~\cite{ucofia}  & V+T &  {49.4} & 72.1 & 83.5 & {47.1} & 74.3 & 83.0 & 409.4 \\
    TEFAL~\cite{tefal} & A+V+T & {49.4} & \textbf{75.9} & \textbf{83.9} & {47.1} & {75.1} & \textbf{84.9} & 416.3 \\
    \ccol  AVIGATE (Ours) & \ccol A+V+T &\ccol  \textbf{50.2} & \ccol {74.3}  &\ccol  83.2 &\ccol \textbf{49.7} &  \ccol  \textbf{75.3}   & \ccol 83.7 & \ccol \textbf{416.4}    \\
    \midrule
    \multicolumn{9}{l}{\textit{\textbf{CLIP ViT-B/16}}} \\ [-0.4ex] \midrule
    X-Pool~\cite{xpool} & V+T & 48.2 & 73.7 & 82.6 & 46.4 & 73.9 & 84.1 & 408.9 \\
    TS2-Net~\cite{ts2} & V+T & 49.4 & 75.6 & 85.3 & 46.6 & 75.9 & 84.9 & 417.7 \\
    ProST~\cite{prost} & V+T & 49.5 & 75.0 & 84.0 & 48.0 & 75.9 & 85.2 & 417.6 \\
    UCoFiA$^\dagger$~\cite{ucofia}  & V+T &  49.8 & 74.6 & 83.5 & {49.1} & {77.0} & 83.8 & 417.8 \\
    TEFAL~\cite{tefal} & A+V+T & 49.9 & 76.2 & 84.4  & - & - & - & - \\
    UATVR~\cite{uatvr} & V+T & {50.8} & {76.3} & \textbf{85.5} & 48.1 & 76.3 & {85.4} & 422.4 \\ 
    \ccol  AVIGATE (Ours) & \ccol A+V+T &\ccol  \textbf{52.1} & \ccol \textbf{76.4} &\ccol  {85.2} &\ccol \textbf{51.2} &  \ccol  \textbf{77.9}   & \ccol \textbf{86.2} & \ccol \textbf{429.0}    \\
\bottomrule 
\end{tabularx}
\vspace{-1.5mm}
\caption{Text-to-video and video-to-text retrieval results on the MSR-VTT 9k split. 
% \textbf{Bold} denotes the best performance.
$^\dagger$ denotes the use of post-processing techniques.
}
\label{tab:main_results}
\vspace{-3mm}
\end{table*}

==> Submission_backup_0304/tabs/table2.tex <==

\begin{table}[!t]
% \vspace{-5mm}
% \setlength{\tabcolsep}{2.5pt}
\vspace{2mm}
\centering
\fontsize{8.2}{9.5}\selectfont
\scalebox{0.95}{
\begin{tabularx}{0.499\textwidth}
    {
      p{0.13\textwidth}
      >{\raggedright\arraybackslash}p{0.07\textwidth}
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X
      }
     \toprule
    {\multirow{1}{*}[-4.5mm]{\textbf{Methods}}}& \multirow{1}{*}[-4.5mm]{\textbf{Modality}}&
    \multicolumn{3}{c}{\textbf{Text-to-Video Retrieval}} \\ [-0.3ex]  \cmidrule(lr){3-5}  
     & & R@1 & R@5 & R@10   \\  [-0.4ex] \midrule
    \multicolumn{5}{l}{\textit{\textbf{CLIP ViT-B/32}}} \\ [-0.3ex]\midrule
    % CLIP4Clip$_{seqTransf}$~\cite{clip4clip} & V+T & 55.9 & 89.2 & 95.0 \\
    % CLIP2Video~\cite{clip2video} & V+T & 57.3 & 90.0 & {95.5} \\
    ECLIPSE~\cite{eclipse} & A+V+T & 57.8 & 88.4 & 94.3 \\
    TS2-Net~\cite{ts2} & V+T & 59.1 & 90.0 & 95.2 \\
    X-Pool~\cite{xpool} & V+T & 60.0 & 90.0 & 95.0 \\
    ProST~\cite{prost} & V+T & 60.6 & 90.5 & 95.4 \\ 
    TEFAL~\cite{tefal} & A+V+T & 61.0 & 90.0 & 95.0 \\
    UCoFiA$^\dagger$~\cite{ucofia} & V+T & 61.1 & 90.5 & - \\
    UATVR~\cite{uatvr} & V+T & {61.3} & \textbf{91.0} & \textbf{95.6} \\
    \ccol  AVIGATE (Ours) & \ccol A+V+T &\ccol  \textbf{63.1} & \ccol {90.7 } &\ccol  {95.5} \\
    \midrule
    \multicolumn{5}{l}{\textit{\textbf{CLIP ViT-B/16}}} \\ [-0.4ex] \midrule
    X-Pool~\cite{xpool} & V+T & 62.6 & 91.7 & 96.0 \\
    ProST~\cite{prost} & V+T & 64.0 & 92.2 & 96.3 \\
    UATVR~\cite{uatvr} & V+T & {64.5} & {92.6} & \textbf{96.8} \\
    \ccol  AVIGATE (Ours) & \ccol A+V+T &\ccol  \textbf{67.5} & \ccol \textbf{93.2 } &\ccol  {96.7} \\
    % \ccol  Ours + DSL & \ccol A+V+T &\ccol  53.8 & 80.1 \ccol &\ccol  87.1 &\ccol 53.4 &  \ccol  75.2   & \ccol 82.8    \\ \midrule
     
\bottomrule 
\end{tabularx}
}
\vspace{-1.5mm}
\caption{Text-to-video retrieval results on VATEX. 
% \textbf{Bold} denotes the best accuracy. 
$^\dagger$ denotes the use of post-processing techniques. 
}
\label{tab:vatex}
\vspace{-4.2mm}
\end{table}


% \begin{table}[!t]
% % \vspace{-5mm}
% \setlength{\tabcolsep}{2.5pt}
% \fontsize{8.5}{9}\selectfont
% \centering
% \begin{tabularx}{0.49\textwidth}
%     {
%       p{0.13\textwidth}
%       >{\raggedright\arraybackslash}p{0.07\textwidth}
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       }
%      \toprule
%     {\multirow{1}{*}[-4.5mm]{\textbf{Methods}}}& \multirow{1}{*}[-4.5mm]{\textbf{Modality}}&
%     \multicolumn{3}{c}{\textbf{Text-to-Video Retrieval}} &\multirow{2}{*}{RSum}\\ [-0.3ex]  \cmidrule(lr){3-5}  
%      & & R@1 & R@5 & R@10 &   \\  [-0.4ex] \midrule
%     \multicolumn{6}{l}{\textit{\textbf{CLIP ViT-B/32}}} \\ [-0.3ex]\midrule
%     CLIP2Video~\cite{clip2video} & V+T & 57.3 & 90.0 & {95.5} & 242.8 \\
%     ECLIPSE~\cite{eclipse} & A+V+T & 57.8 & 88.4 & 94.3 & 240.5 \\
%     TS2-Net~\cite{ts2} & V+T & 59.1 & 90.0 & 95.2 & 244.3 \\
%     X-Pool~\cite{xpool} & V+T & 60.0 & 90.0 & 95.0 & 245.0 \\
%     ProST~\cite{prost} & V+T & 60.6 & 90.5 & 95.4 & 246.5 \\ 
%     TEFAL~\cite{tefal} & A+V+T & 61.0 & 90.0 & 95.0 & 246.0 \\
%     UCoFiA$^\dagger$~\cite{ucofia} & V+T & 61.1 & 90.5 & - & - \\
%     UATVR~\cite{uatvr} & V+T & {61.3} & \textbf{91.0} & \textbf{95.6} & 247.9 \\
%     \ccol  AVIGATE (Ours) & \ccol A+V+T &\ccol  \textbf{63.1} & \ccol {90.7 } &\ccol  {95.5} & \ccol \textbf{249.3} \\
%     \midrule
%     \multicolumn{6}{l}{\textit{\textbf{CLIP ViT-B/16}}} \\ [-0.4ex] \midrule
%     X-Pool~\cite{xpool} & V+T & 62.6 & 91.7 & 96.0 & 250.3 \\
%     ProST~\cite{prost} & V+T & 64.0 & 92.2 & 96.3 & 252.5 \\
%     UATVR~\cite{uatvr} & V+T & {64.5} & {92.6} & \textbf{96.8} & 253.9 \\
%     \ccol  AVIGATE (Ours) & \ccol A+V+T &\ccol  \textbf{67.5} & \ccol \textbf{93.2 } &\ccol  {96.7} & \ccol \textbf{257.4} \\
     
% \bottomrule 
% \end{tabularx}
% \vspace{-2.5mm}
% \caption{Text-to-video retrieval results on VATEX. \textbf{Bold} denotes the best accuracy. $^\dagger$ denotes the use of post-processing techniques. 
% }
% \label{tab:vatex}
% \vspace{-4mm}
% \end{table}

==> Submission_backup_0304/tabs/table_ablation.tex <==
% \begin{table}[!t]
% % \vspace{-5mm}
% \setlength{\tabcolsep}{2.5pt}
% \fontsize{9}{10}\selectfont
% \centering
% \begin{tabularx}{0.49\textwidth}
%     {
%       p{0.15\textwidth}
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}X
%       }
%      \toprule
%     {\multirow{1}{*}[-4.5mm]{\textbf{Methods}}}& \multirow{1}{*}[-4.5mm]{\textbf{Gate}}& \multirow{1}{*}[-4.5mm]{\textbf{Margin}}&
%     \multicolumn{3}{c}{\textbf{Text-to-Video Retrieval}} \\ [-0.3ex]  \cmidrule(lr){4-6}  
%      & & & R@1 & R@5 & R@10   \\  [-0.4ex] \midrule
%     % \multicolumn{6}{l}{\textit{\textbf{CLIP ViT-B/32}}} \\ [-0.3ex]\midrule
%     Baseline & \xmark & \xmark & 45.4 & 72.2 & 81.6 \\
%     ~~+ Audio & \xmark & \xmark & 47.1& 73.4 & 81.9 \\ \midrule
%     Gated Fusion & \cmark & \xmark & 48.0& 75.1 & 83.4\\
%     Adaptive Margin & \xmark & \cmark & 48.9 & 74.8& 83.7\\
%     %$\mathcal{L}$ in~\cref{eq:Margin_loss} & \xmark & \cmark & 48.9 & 74.8& 83.7\\ 
%     Fixed Margin & \cmark & \cmark& 49.0 & 74.1 & 83.5\\ 
%     \ccol  AVIGATE (Ours) & \ccol \cmark &\ccol  \cmark & \ccol 50.2 &\ccol  74.3 & \ccol 83.2  \\

% \bottomrule 
% \end{tabularx}
% \vspace{-2.5mm}
% \caption{Ablation studies on key components of our method. The experiments are conducted on the MSR-VTT 9k split with CLIP ViT-B/32.  
% }
% \label{tab:ablation_components}
% \vspace{-4mm}
% \end{table}

\begin{table}[!t]
% \vspace{-5mm}
\setlength{\tabcolsep}{4pt}
\fontsize{8.2}{9.5}\selectfont
\centering
\scalebox{0.95}{
\begin{tabularx}{0.5\textwidth}
    {
      p{0.12\textwidth}
      >{\centering\arraybackslash}p{0.04\textwidth}
      >{\centering\arraybackslash}p{0.04\textwidth}
      >{\centering\arraybackslash}p{0.063\textwidth}
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X
      }
     \toprule
    {\multirow{1}{*}[-4.7mm]{\textbf{Methods}}}& \multirow{1}{*}[-4.7mm]{\textbf{Gate}}&
    \multicolumn{2}{c}{\textbf{Margin}} &
    \multicolumn{3}{c}{\textbf{Text-to-Video Retrieval}} \\ [-0.3ex] \cmidrule(lr){3-4} \cmidrule(lr){5-7}  
     & & \textbf{Fixed} & \textbf{Adaptive} & R@1 & R@5 & R@10   \\  [-0.4ex] \midrule
    % \multicolumn{6}{l}{\textit{\textbf{CLIP ViT-B/32}}} \\ [-0.3ex]\midrule
    Baseline & \xmark & \xmark & \xmark & 45.4 & 72.2 & 81.6 \\
    ~~+ Audio & \xmark & \xmark & \xmark & 47.1& 73.4 & 81.9 \\ \midrule
    Adaptive Margin & \xmark & \xmark & \cmark & 48.9 & 74.8& 83.7\\
    Gated Fusion & \cmark & \xmark & \xmark & 48.0& 75.1 & 83.4\\
    %$\mathcal{L}$ in~\cref{eq:Margin_loss} & \xmark & \cmark & 48.9 & 74.8& 83.7\\ 
    ~~+ Fixed Margin & \cmark & \cmark & \xmark& 49.0 & 74.1 & 83.5\\ 
    \ccol  AVIGATE (Ours) & \ccol \cmark &\ccol \xmark&\ccol  \cmark & \ccol 50.2 &\ccol  74.3 & \ccol 83.2  \\

\bottomrule 
\end{tabularx}
}
\vspace{-1.5mm}
\caption{Ablation studies on key components of our method. %The experiments are conducted on the MSR-VTT 9k split with CLIP ViT-B/32.
}
\label{tab:ablation_components}
\vspace{-1.0mm}
\end{table}

==> Submission_backup_0304/tabs/table_complexity.tex <==


% \begin{table}[!t]
% % \vspace{-5mm}
% \setlength{\tabcolsep}{2.5pt}
% \fontsize{9}{10}\selectfont
% \centering
% \begin{tabularx}{0.49\textwidth}
%     {
%       p{0.128\textwidth}
%       >{\centering\arraybackslash}X
%       >{\centering\arraybackslash}p{0.04\textwidth}
%       >{\centering\arraybackslash}p{0.04\textwidth}
%       >{\centering\arraybackslash}p{0.05\textwidth}
%       >{\centering\arraybackslash}p{0.04\textwidth}
%       }
%      \toprule
%     {\multirow{1}{*}[-4.5mm]{\textbf{Methods}}}& \multirow{1}{*}[-0.5mm]{\textbf{Time}}&
%     \multicolumn{2}{c}{\textbf{Text-to-Video}} & \multicolumn{2}{c}{\textbf{Latency (ms)}$\downarrow$}  \\ [-0.3ex] \cmidrule(lr){3-4} \cmidrule(lr){5-6}   
%      & \multirow{1}{*}[0.5mm]{\textbf{Complexity}}& R@1 & R@5 & Total & $t_\text{ex}$  \\  [-0.4ex] \midrule
%     \multicolumn{6}{l}{\textit{\textbf{Modality: Video and Text}}} \\ [-0.3ex]\midrule
%     CLIP4Clip~\cite{clip4clip} & $\mathcal{O}$($\mathcal{V}+\mathcal{T}$) & 44.5 & 71.4 & 9.76 &9.74 \\
%     X-Pool~\cite{xpool} & $\mathcal{O}$($\mathcal{V}\mathcal{T}$)& 46.9 & 72.8 & 66.31 & 9.74 \\ [-0.3ex]\midrule
%     \multicolumn{6}{l}{\textit{\textbf{Modality: Audio, Video and Text}}} \\ [-0.3ex]\midrule
%     TEFAL~\cite{tefal} &$\mathcal{O}$($\mathcal{A}\mathcal{T} +\mathcal{V}\mathcal{T}$) & 49.4 & 75.9  &140.57 &9.74 \\
%     AVIGATE (Ours)& $\mathcal{O}$($\mathcal{A}\mathcal{V}+\mathcal{T}$) & 50.2 & 74.3 & 9.90 &9.74 \\
%     \bottomrule 
% \end{tabularx}
% \vspace{-2.5mm}
% \caption{Analysis of the efficiency of our method compared to the previous arts. $t_\text{ex}$ denotes the time required to extract the text query embedding. Note that $t_\text{ex}$ for all methods are the same since they use the same text encoder without any extra modules.}
% \label{tab:complexity}
% \vspace{-4mm}
% \end{table}



\begin{table}[!t]
% \vspace{-5mm}
\setlength{\tabcolsep}{2pt}
\fontsize{8.1}{9.5}\selectfont
\centering
\scalebox{0.95}{
\begin{tabularx}{0.499\textwidth}
    {
      p{0.09\textwidth}
      >{\centering\arraybackslash}p{0.12\textwidth}
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}p{0.05\textwidth}
      >{\centering\arraybackslash}p{0.05\textwidth}
      >{\centering\arraybackslash}p{0.05\textwidth}
      }
     \toprule
    {\multirow{1}{*}[-4.5mm]{\textbf{Methods}}}& \multirow{1}{*}[-0.5mm]{\textbf{Time}}&
    \multicolumn{2}{c}{\textbf{Performance}} & \multicolumn{3}{c}{\textbf{Latency (ms)}$\downarrow$}  \\ [-0.3ex] \cmidrule(lr){3-4} \cmidrule(lr){5-7}   
     & \multirow{1}{*}[0.5mm]{\textbf{Complexity}}& R@1 & RSum & $t_\text{sim}$ & $t_\text{ex}$ & Total  \\  [-0.4ex] \midrule
    \multicolumn{7}{l}{\textit{\textbf{Modality: Video and Text}}} \\ [-0.3ex]\midrule
    CLIP4Clip~\cite{clip4clip} & $\mathcal{O}$($\mathcal{V}+\mathcal{T}$) & 44.5 & 391.7 & 0.02 & 9.74 & 9.76 \\
    X-Pool~\cite{xpool} & $\mathcal{O}$($\mathcal{V}\mathcal{T}$)& 46.9 & 403.6  & 56.57 & 9.74 & 66.31 \\ [-0.3ex]\midrule
    \multicolumn{7}{l}{\textit{\textbf{Modality: Audio, Video and Text}}} \\ [-0.3ex]\midrule
    TEFAL~\cite{tefal} &$\mathcal{O}$($\mathcal{A}\mathcal{T} +\mathcal{V}\mathcal{T}$) & 49.4 & 416.3  &130.83 & 9.74 &140.57 \\
    AVIGATE & $\mathcal{O}$($\mathcal{A}+\mathcal{V}+\mathcal{T}$) &\textbf{ 50.2} & \textbf{416.4 }& 0.16 &9.74 &9.90 \\
    \bottomrule 
\end{tabularx}
}
\vspace{-1.0mm}
\caption{Analysis of the efficiency of our method compared to the previous arts. 
$t_\textrm{sim}$ and $t_\textrm{ex}$ denote the latency of the similarity calculation and the query embedding extraction, respectively.
% $t_\textrm{ex}$ denotes the latency of the text query embedding extraction. 
Note that $t_\text{ex}$ for all methods are the same since they use the same text encoder. %without any extra modules.
The latency is calculated by a single RTX3090 card.}
\label{tab:complexity}
\vspace{-3.5mm}
\end{table}

==> Submission_backup_0304/tabs/table_hyp.tex <==

\begin{table}[!t]
% \vspace{-5mm}
\setlength{\tabcolsep}{2pt}
\fontsize{8.2}{9}\selectfont
\centering
\scalebox{0.95}{
\begin{tabularx}{0.499\textwidth}
    {
      >{\centering\arraybackslash}p{0.13\textwidth}
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X
      >{\centering\arraybackslash}X
      }
     \toprule
    \multirow{1}{*}[-4.5mm]{\textbf{Ablated Setting}} & \multicolumn{3}{c}{\textbf{Text-to-Video Retrieval}} \\ [-0.3ex] \cmidrule(lr){2-4}  
    &  R@1 & R@5 & R@10   \\  [-0.4ex] \midrule
    % \multicolumn{4}{l}{\textit{\textbf{(a) Layer depth of Gated Fusion Transformer: $L$}}} \\ [-0.3ex]\midrule
    % $L$=1 & 49.0 & 74.0 & 82.6 \\
    % $L$=2  & 49.8 & 74.0 & 83.0 \\
    % \ccol$L$=4  &\ccol 50.2 &\ccol  74.3 & \ccol 83.2 \\
    % $L$=6  & 49.5 & 74.2 & 82.6 \\    [-0.3ex]\midrule
    \multicolumn{4}{l}{\textit{\textbf{Granularity of alignment scheme}}} \\ [-0.3ex]\midrule
    Global only & 46.1 & 73.4 & 82.4 \\
    Local only & 48.5 & 73.7 & 82.8 \\
    \ccol Global-Local   & \ccol 50.2 &\ccol  74.3 & \ccol 83.2  \\

\bottomrule 
\end{tabularx}
}
\vspace{-1.5mm}
\caption{Ablation studies on alignment scheme. 
% \colorbox{grey}{{gray}} corresponds to our default setting.
}
\label{tab:ablation_hyp}
\vspace{-4mm}
\end{table}
